F-Fidelity: A Robust Framework for Faithfulness Evaluation of Explainable AI

Recent research has developed a number of eXplainable AI (XAI) techniques, such as gradient-based approaches, input perturbation-base methods, and black-box explanation methods. While these XAI techniques can extract meaningful insights from deep learning models, how to properly evaluate them remains an open problem. The most widely used approach is to perturb or even remove what the XAI method considers to be the most important features in an input and observe the changes in the output prediction. This approach, although straightforward, suffers the Out-of-Distribution (OOD) problem as the perturbed samples may no longer follow the original data distribution. A recent method RemOve And Retrain (ROAR) solves the OOD issue by retraining the model with perturbed samples guided by explanations. However, using the model retrained based on XAI methods to evaluate these explainers may cause information leakage and thus lead to unfair comparisons. We propose Fine-tuned Fidelity (F-Fidelity), a robust evaluation framework for XAI, which utilizes i) an explanation-agnostic fine-tuning strategy, thus mitigating the information leakage issue, and ii) a random masking operation that ensures that the removal step does not generate an OOD input. We also design controlled experiments with state-of-the-art (SOTA) explainers and their degraded version to verify the correctness of our framework. We conduct experiments on multiple data modalities, such as images, time series, and natural language. The results demonstrate that F-Fidelity significantly improves upon prior evaluation metrics in recovering the ground-truth ranking of the explainers. Furthermore, we show both theoretically and empirically that, given a faithful explainer, F-Fidelity metric can be used to compute the sparsity of influential input components, i.e., to extract the true explanation size.

==> experiments/Boiler/lstm_correlation_detail.tex <==
\begin{table*}[h]
    \centering
    \caption{Local Spearman rank correlation results on Boiler dataset with LSTM as the model to be explained.`-' means not available due to the different explanations having the same rank.}
    \label{tab:exp:PAM:LSTM:local:combined}
    \scalebox{0.6}{
     \begin{tabular}{c|cccc|cccc|cccc}
        \toprule
        & \multicolumn{4}{c|}{MoRF vs GT} & \multicolumn{4}{c|}{LeRF vs GT} & \multicolumn{4}{c}{MoRF vs LeRF} \\
        Sparsity & Fidelity & ROAR & R-Fidelity & F-Fidelity & Fidelity & ROAR & R-Fidelity & F-Fidelity & Fidelity & ROAR & R-Fidelity & F-Fidelity \\
        \midrule   
5\% & \ms{-0.95}{0.02} & \ms{\textbf{-0.97}}{0.03} & \ms{\textbf{-0.97}}{0.03} & \ms{\textbf{-0.97}}{0.07} & - & - & \ms{-0.03}{0.36} & \ms{\textbf{0.95}}{0.04} & - & - & \ms{0.07}{0.27} & \ms{-0.90}{0.15}\\
10\% & \ms{-0.96}{0.03} & \ms{-0.98}{0.03} & \ms{\textbf{-1.00}}{0.00} & \ms{-0.99}{0.02} & - & - & \ms{0.74}{0.23} & \ms{\textbf{1.00}}{0.00} & - & - & \ms{-0.74}{0.23} & \ms{\textbf{-0.99}}{0.02}\\
15\% & \ms{-0.91}{0.04} & \ms{-0.99}{0.01} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & - & - & \ms{0.92}{0.04} & \ms{\textbf{1.00}}{0.00} & - & - & \ms{-0.92}{0.04} & \ms{\textbf{-1.00}}{0.00}\\
20\% & \ms{-0.78}{0.10} & \ms{-0.93}{0.04} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & - & - & \ms{0.95}{0.03} & \ms{\textbf{1.00}}{0.00} & - & - & \ms{-0.95}{0.03} & \ms{\textbf{-1.00}}{0.00}\\
25\% & - & \ms{-0.73}{0.09} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & - & - & \ms{0.94}{0.04} & \ms{\textbf{1.00}}{0.00} & - & - & \ms{-0.94}{0.04} & \ms{\textbf{-1.00}}{0.00}\\

30\% & - & \ms{-0.69}{0.07} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & - & - & \ms{0.99}{0.02} & \ms{\textbf{1.00}}{0.00} & - & - & \ms{-0.99}{0.02} & \ms{\textbf{-1.00}}{0.00}\\
35\% & - & \ms{-0.69}{0.08} & \ms{\textbf{-1.00}}{0.00} & \ms{-0.99}{0.02} & - & - & \ms{\textbf{1.00}}{0.00} & \ms{0.97}{0.03} & - & - & \ms{\textbf{-1.00}}{0.00} & \ms{-0.98}{0.03}\\
40\% & - & - & \ms{\textbf{-1.00}}{0.00} & \ms{-0.97}{0.03} & - & - & \ms{\textbf{1.00}}{0.00} & \ms{0.97}{0.03} & - & - & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00}\\
45\% & - & - & \ms{\textbf{-0.99}}{0.02} & \ms{-0.97}{0.03} & \ms{0.69}{0.08} & \ms{0.86}{0.04} & \ms{\textbf{1.00}}{0.00} & \ms{0.97}{0.03} & - & - & \ms{-0.99}{0.02} & \ms{\textbf{-1.00}}{0.00}\\
50\% & - & - & \ms{\textbf{-0.98}}{0.03} & \ms{-0.93}{0.06} & \ms{0.81}{0.07} & \ms{0.88}{0.05} & \ms{\textbf{0.99}}{0.02} & \ms{0.94}{0.06} & - & - & \ms{-0.97}{0.03} & \ms{\textbf{-0.99}}{0.02}\\
55\% & - & - & \ms{\textbf{-0.98}}{0.03} & \ms{-0.90}{0.06} & \ms{0.86}{0.04} & \ms{0.88}{0.05} & \ms{\textbf{0.95}}{0.02} & \ms{0.92}{0.05} & - & - & \ms{-0.98}{0.03} & \ms{\textbf{-0.99}}{0.02}\\

60\% & - & - & \ms{-0.86}{0.07} & \ms{-0.84}{0.06} & \ms{0.86}{0.04} & \ms{\textbf{0.89}}{0.05} & \ms{0.85}{0.05} & \ms{0.84}{0.06} & - & - & \ms{-0.94}{0.06} & \ms{\textbf{-1.00}}{0.00}\\
65\% & - & - & \ms{\textbf{-0.83}}{0.13} & \ms{-0.78}{0.07} & \ms{\textbf{0.86}}{0.04} & \ms{0.81}{0.13} & \ms{0.78}{0.02} & \ms{0.78}{0.07} & - & - & \ms{-0.92}{0.05} & \ms{\textbf{-0.98}}{0.03}\\
70\% & - & - & \ms{\textbf{-0.74}}{0.13} & \ms{-0.67}{0.06} & \ms{\textbf{0.86}}{0.04} & \ms{0.72}{0.11} & \ms{0.66}{0.09} & \ms{0.70}{0.08} & - & - & \ms{-0.85}{0.12} & \ms{\textbf{-0.97}}{0.03}\\
75\% & - & - & \ms{-0.47}{0.14} & \ms{-0.65}{0.02} & \ms{\textbf{0.78}}{0.13} & \ms{0.52}{0.06} & \ms{0.55}{0.06} & \ms{0.62}{0.03} & - & - & \ms{-0.82}{0.12} & \ms{\textbf{-0.98}}{0.03}\\
80\% & - & - & \ms{-0.47}{0.7} & \ms{-0.47}{0.10} & \ms{\textbf{0.61}}{0.09} & \ms{0.49}{0.03} & \ms{0.49}{0.00} & \ms{\textbf{0.61}}{0.02} & - & - & \ms{-0.87}{0.10} & \ms{\textbf{-0.97}}{0.03}\\
85\% & - & - & \ms{-0.26}{0.31} & \ms{-0.38}{0.08} & \ms{0.38}{0.12} & \ms{0.31}{0.12} & \ms{0.23}{0.03} & \ms{\textbf{0.42}}{0.16} & - & - & \ms{-0.77}{0.17} & \ms{\textbf{-0.91}}{0.09}\\

90\% & \ms{0.00}{0.00} & - & \ms{0.06}{0.21} & \ms{-0.19}{0.08} & \ms{0.13}{0.10} & \ms{0.12}{0.09} & \ms{0.06}{0.07} & \ms{\textbf{0.22}}{0.07} & - & - & \ms{-0.57}{0.20} & \ms{\textbf{-0.97}}{0.03}\\
95\% & \ms{0.00}{0.00} & - & \ms{\textbf{-0.43}}{0.18} & \ms{-0.05}{0.09} & \ms{0.04}{0.10} & \ms{0.07}{0.07} & \ms{0.07}{0.07} & \ms{0.11}{0.09} & - & - & \ms{-0.26}{0.17} & \ms{-0.89}{0.09}\\
\midrule
Avg. Rank & 2.95 & 2.73 & \textbf{1.21} & 1.52 & 2.59 & 2.74 & 2.21 & \textbf{1.68} & 2.95 & 2.95 & 1.89 & \textbf{1.05}\\
        \bottomrule
    \end{tabular}
    }
\end{table*}






        


% \begin{table*}[h]
%     \centering
%         \caption{"MoRF VS GT" Local Spearman rank correlation results on Boiler dataset with LSTM as the model to be explained.'N/A' means not available due to the different explanations having the same rank.}
%     \label{tab:exp:PAM:LSTM:local:morf_rank}
%     \scalebox{0.75}{
%      \begin{tabular}{cccccccc}
%         \toprule
%         &
%         \multicolumn{2}{c}{Fidelity} &
%         \multicolumn{1}{c}{ROAR} &
%         \multicolumn{2}{c}{R-Fidelity} & 
%         \multicolumn{2}{c}{F-Fidelity} \\
%         \cmidrule(r){2-3} \cmidrule(r){4-4} \cmidrule(r){5-6} \cmidrule(r){7-8}
%         Sparsity &  origin  & fine-tune  & retrain  & origin  & fine-tune & origin  & fine-tune  \\
%         % Model & Correlation & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
%          \midrule   
%         % & \multicolumn{4}{c}{Local Spearman Correlation $\downarrow$} \\ 
%         % \hline
%         % \multirow{3}{\rotatebox[origin=c]{90}{ViT}}  \ms{\textbf{1.00}}{0.00}
%         $5\%$&  \ms{-0.95}{0.02} &  \ms{-0.96}{0.07} &  \ms{\textbf{-0.97}}{0.03} &  \ms{\textbf{-0.97}}{0.03} &  \ms{\textbf{-0.97}}{0.07} &  \ms{\textbf{-0.97}}{0.03} &  \ms{\textbf{-0.97}}{0.07} \\
%         10\% &  \ms{-0.96}{0.03} &  \ms{-0.99}{0.02} &  \ms{-0.98}{0.03} &  \ms{\textbf{-1.00}}{0.00} &  \ms{-0.99}{0.02} &  \ms{\textbf{-1.00}}{0.00} &  \ms{-0.98}{0.02}   \\
%         15\% &  \ms{-0.91}{0.04} &  \ms{\textbf{-1.00}}{0.00} &  \ms{-0.99}{0.01} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}   \\
%         20\% &  \ms{-0.78}{0.10} &  \ms{\textbf{-1.00}}{0.00} &  \ms{-0.93}{0.04} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}   \\
%         25\% &  \ms{N/A}{N/A} &  \ms{-0.98}{0.03} &  \ms{-0.73}{0.09} &  \ms{\textbf{-1.00}}{0.00}    &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}   \\
        
%         30\% &  \ms{N/A}{N/A} &  \ms{-0.99}{0.00} &  \ms{-0.69}{0.07} &  \ms{\textbf{-1.00}}{0.00}    &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}   \\
%         35\% &  \ms{N/A}{N/A} &  \ms{-0.92}{0.06} &  \ms{-0.69}{0.08} &  \ms{\textbf{-1.00}}{0.00}    &  \ms{-0.99}{0.02} &  \ms{\textbf{-1.00}}{0.00} &  \ms{-0.98}{0.03}   \\
%         40\% &  \ms{N/A}{N/A} &  \ms{-0.91}{0.04} &  \ms{N/A}{N/A} &  \ms{\textbf{-1.00}}{0.00}      &  \ms{-0.97}{0.03} &  \ms{\textbf{-1.00}}{0.00} &  \ms{-0.94}{0.06}  \\
%         45\% &  \ms{N/A}{N/A} &  \ms{-0.88}{0.05} &  \ms{N/A}{N/A} &  \ms{\textbf{-0.99}}{0.02}      &  \ms{-0.97}{0.03} &  \ms{\textbf{-0.99}}{0.02} &  \ms{-0.97}{0.03}   \\
%         50\% &  \ms{N/A}{N/A} &  \ms{-0.76}{0.09} &  \ms{N/A}{N/A} &  \ms{\textbf{-0.98}}{0.03}      &  \ms{-0.93}{0.06} &  \ms{-0.95}{0.02} &  \ms{-0.94}{0.06}  \\
%         55\% &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{\textbf{-0.98}}{0.03}         &  \ms{-0.90}{0.06} &  \ms{-0.93}{0.06} &  \ms{-0.92}{0.08}  \\
        
%         60\% &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{-0.86}{0.07}        &  \ms{-0.84}{0.06} &  \ms{\textbf{-0.89}}{0.07} &  \ms{\textbf{-0.89}}{0.06}  \\
%         65\% &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{\textbf{-0.83}}{0.13}        &  \ms{-0.78}{0.07} &  \ms{-0.79}{0.03} &  \ms{-0.77}{0.13}   \\
%         70\% &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{\textbf{-0.74}}{0.13}        &  \ms{-0.67}{0.06} &  \ms{-0.73}{0.10} &  \ms{-0.69}{0.09}   \\
%         75\% &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{-0.47}{0.14}        &  \ms{-0.65}{0.02} &  \ms{-0.54}{0.10} &  \ms{\textbf{-0.66}}{0.15}   \\
%         80\% &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{-0.47}{0.7}         &  \ms{-0.47}{0.10} &  \ms{-0.42}{0.14} &  \ms{\textbf{-0.59}}{0.08}   \\
%         85\% &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{-0.26}{0.31}        &  \ms{-0.38}{0.08} &  \ms{\textbf{-0.44}}{0.15} &  \ms{-0.39}{0.11}   \\
        
%         90\% &  \ms{0.00}{0.00} &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{0.06}{0.21}       &  \ms{-0.19}{0.08} &  \ms{-0.23}{0.15} &  \ms{\textbf{-0.32}}{0.17}   \\
%         95\% &  \ms{0.00}{0.00} &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{\textbf{-0.43}}{0.18}      &  \ms{-0.05}{0.09} &  \ms{-0.06}{0.10} &  \ms{-0.19}{0.20}   \\
%         \midrule   
%         Avg. Rank & 5.84 & 4.53 & 5.32 & 1.68 & 2.68 & \textbf{1.63} & 2.21\\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table*}

% \begin{table*}[h]
%     \centering
%         \caption{"LeRF VS GT" Local Spearman rank correlation results on Boiler dataset with LSTM as the model to be explained.'N/A' means not available due to the different explanations having the same rank.}
%     \label{tab:exp:PAM:LSTM:local:lerf_rank}
%     \scalebox{0.75}{
%      \begin{tabular}{ccccccccccc}
%         \toprule
%         &
%         \multicolumn{2}{c}{Fidelity} &
%         \multicolumn{1}{c}{ROAR} &
%         \multicolumn{2}{c}{R-Fidelity} & 
%         \multicolumn{2}{c}{F-Fidelity} \\
%         \cmidrule(r){2-3} \cmidrule(r){4-4} \cmidrule(r){5-6} \cmidrule(r){7-8}
%         Sparsity &  origin  & fine-tune  & retrain  & origin  & fine-tune & origin  & fine-tune  \\
%         % Model & Correlation & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
%          \midrule   
%         % & \multicolumn{4}{c}{Local Spearman Correlation $\downarrow$} \\ 
%         % \hline
%         % \multirow{3}{\rotatebox[origin=c]{90}{ViT}}  \ms{\textbf{1.00}}{0.00}
%         $5\%$&  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{-0.03}{0.36}   &  \ms{\textbf{0.95}}{0.04} &  \ms{0.87}{0.01} &  \ms{0.92}{0.05} \\
%         10\% &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{0.74}{0.23}    &  \ms{\textbf{1.00}}{0.00} &  \ms{0.98}{0.03} &  \ms{0.98}{0.03}   \\
%         15\% &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{0.92}{0.04}    &  \ms{\textbf{1.00}}{0.00} &  \ms{0.99}{0.02} &  \ms{\textbf{1.00}}{0.00}   \\
%         20\% &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{0.95}{0.03}    &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}   \\
%         25\% &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{0.94}{0.04}    &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}   \\
        
%         30\% &  \ms{N/A}{N/A} &  \ms{0.86}{0.04} &  \ms{N/A}{N/A} &  \ms{0.99}{0.02} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}   \\
%         35\% &  \ms{N/A}{N/A} &  \ms{0.95}{0.01} &  \ms{N/A}{N/A} &  \ms{\textbf{1.00}}{0.00} &  \ms{0.97}{0.03} &  \ms{\textbf{1.00}}{0.00} &  \ms{0.95}{0.04}   \\
%         40\% &  \ms{N/A}{N/A} &  \ms{0.94}{0.06} &  \ms{N/A}{N/A} &  \ms{\textbf{1.00}}{0.00} &  \ms{0.97}{0.03} &  \ms{0.99}{0.02} &  \ms{0.91}{0.03}  \\
%         45\% &  \ms{0.69}{0.08} &  \ms{0.93}{0.07} &  \ms{0.86}{0.04} &  \ms{\textbf{1.00}}{0.00} &  \ms{0.97}{0.03} &  \ms{0.99}{0.02} &  \ms{0.86}{0.09}   \\
%         50\% &  \ms{0.81}{0.07} &  \ms{0.94}{0.06} &  \ms{0.88}{0.05} &  \ms{\textbf{0.99}}{0.02} &  \ms{0.94}{0.06} &  \ms{0.98}{0.03} &  \ms{0.84}{0.11}  \\
%         55\% &  \ms{0.86}{0.04} &  \ms{0.91}{0.07} &  \ms{0.88}{0.05} &  \ms{\textbf{0.95}}{0.02} &  \ms{0.92}{0.05} &  \ms{0.90}{0.08} &  \ms{0.91}{0.08}  \\
        
%         60\% &  \ms{0.86}{0.04} &  \ms{0.87}{0.06} &  \ms{\textbf{0.89}}{0.05} &  \ms{0.85}{0.05} &  \ms{0.84}{0.06} &  \ms{0.83}{0.00} &  \ms{0.86}{0.11}  \\
%         65\% &  \ms{\textbf{0.86}}{0.04} &  \ms{0.73}{0.11} &  \ms{0.81}{0.13} &  \ms{0.78}{0.02} &  \ms{0.78}{0.07} &  \ms{0.79}{0.03} &  \ms{0.78}{0.09}   \\
%         70\% &  \ms{\textbf{0.86}}{0.04} &  \ms{0.67}{0.08} &  \ms{0.72}{0.11} &  \ms{0.66}{0.09} &  \ms{0.70}{0.08} &  \ms{0.62}{0.03} &  \ms{0.76}{0.10}   \\
%         75\% &  \ms{\textbf{0.78}}{0.13} &  \ms{0.58}{0.09} &  \ms{0.52}{0.06} &  \ms{0.55}{0.06} &  \ms{0.62}{0.03} &  \ms{0.58}{0.05} &  \ms{0.66}{0.06}   \\
%         80\% &  \ms{\textbf{0.61}}{0.09} &  \ms{0.55}{0.07} &  \ms{0.49}{0.03} &  \ms{0.49}{0.00} &  \ms{\textbf{0.61}}{0.02} &  \ms{0.51}{0.05} &  \ms{\textbf{0.61}}{0.02}   \\
%         85\% &  \ms{0.38}{0.12} &  \ms{0.31}{0.07} &  \ms{0.31}{0.12} &  \ms{0.23}{0.03} &  \ms{\textbf{0.42}}{0.16} &  \ms{0.22}{0.03} &  \ms{\textbf{0.42}}{0.16}   \\
        
%         90\% &  \ms{0.13}{0.10} &  \ms{0.17}{0.09} &  \ms{0.12}{0.09} &  \ms{0.06}{0.07} &  \ms{\textbf{0.22}}{0.07} &  \ms{0.06}{0.07} &  \ms{0.21}{0.07}   \\
%         95\% &  \ms{0.04}{0.10} &  \ms{0.08}{0.05} &  \ms{0.07}{0.07} &  \ms{0.07}{0.07} &  \ms{0.11}{0.09} &  \ms{0.06}{0.07} &  \ms{\textbf{0.15}}{0.07}   \\
%         \midrule   
%         Avg. Rank & 4.47 & 4.21 & 4.79 & 3.79 & \textbf{2.21} & 3.58 & 2.47\\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table*}


% \begin{table*}[h]
%     \centering
%         \caption{"MoRF VS LeRF" Local Spearman rank correlation results on Boiler dataset with LSTM as the model to be explained.'N/A' means not available due to the different explanations having the same rank.}
%     \label{tab:exp:PAM:LSTM:local:morf_lerf}
%     \scalebox{0.75}{
%      \begin{tabular}{cccccccc}
%         \toprule
%         &
%         \multicolumn{2}{c}{Fidelity} &
%         \multicolumn{1}{c}{ROAR} &
%         \multicolumn{2}{c}{R-Fidelity} & 
%         \multicolumn{2}{c}{F-Fidelity} \\
%         \cmidrule(r){2-3} \cmidrule(r){4-4} \cmidrule(r){5-6} \cmidrule(r){7-8}
%         Sparsity &  origin  & fine-tune  & retrain  & origin  & fine-tune & origin  & fine-tune  \\
%         % Model & Correlation & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
%          \midrule   
%         % & \multicolumn{4}{c}{Local Spearman Correlation $\downarrow$} \\ 
%         % \hline
%         % \multirow{3}{\rotatebox[origin=c]{90}{ViT}}  \ms{\textbf{1.00}}{0.00}
%         $5\%$&  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{0.07}{0.27} &  \ms{-0.90}{0.15} &  \ms{-0.90}{0.08} &  \ms{\textbf{-0.95}}{0.02} \\
%         10\% &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{-0.74}{0.23} &  \ms{\textbf{-0.99}}{0.02} &  \ms{-0.97}{0.03} &  \ms{\textbf{-0.99}}{0.02}   \\
%         15\% &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{-0.92}{0.04} &  \ms{\textbf{-1.00}}{0.00} &  \ms{-0.99}{0.02} &  \ms{\textbf{-1.00}}{0.00}   \\
%         20\% &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{-0.95}{0.03} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}   \\
%         25\% &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{-0.94}{0.04} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}   \\
        
%         30\% &  \ms{N/A}{N/A} &  \ms{-0.84}{0.04} &  \ms{N/A}{N/A} &  \ms{-0.99}{0.02} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}   \\
%         35\% &  \ms{N/A}{N/A} &  \ms{-0.85}{0.12} &  \ms{N/A}{N/A} &  \ms{\textbf{-1.00}}{0.00} &  \ms{-0.98}{0.03} &  \ms{\textbf{-1.00}}{0.00} &  \ms{-0.98}{0.03}   \\
%         40\% &  \ms{N/A}{N/A} &  \ms{-0.83}{0.15} &  \ms{N/A}{N/A} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{-0.99}{0.02} &  \ms{-0.92}{0.03}  \\
%         45\% &  \ms{N/A}{N/A} &  \ms{-0.86}{0.06} &  \ms{N/A}{N/A} &  \ms{-0.99}{0.02} &  \ms{\textbf{-1.00}}{0.00} &  \ms{-0.98}{0.03} &  \ms{-0.87}{0.07}   \\
%         50\% &  \ms{N/A}{N/A} &  \ms{-0.75}{0.15} &  \ms{N/A}{N/A} &  \ms{-0.97}{0.03} &  \ms{\textbf{-0.99}}{0.02} &  \ms{-0.98}{0.03} &  \ms{-0.87}{0.07}  \\
%         55\% &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{-0.98}{0.03} &  \ms{\textbf{-0.99}}{0.02} &  \ms{-0.97}{0.07} &  \ms{-0.95}{0.04}  \\
        
%         60\% &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{-0.94}{0.06} &  \ms{\textbf{-1.00}}{0.00} &  \ms{-0.95}{0.07} &  \ms{-0.95}{0.07}  \\
%         65\% &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{-0.92}{0.05} &  \ms{\textbf{-0.98}}{0.03} &  \ms{\textbf{-0.98}}{0.03} &  \ms{-0.91}{0.09}   \\
%         70\% &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{-0.85}{0.12} &  \ms{\textbf{-0.97}}{0.03} &  \ms{\textbf{-0.97}}{0.03} &  \ms{-0.92}{0.03}   \\
%         75\% &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{-0.82}{0.12} &  \ms{\textbf{-0.98}}{0.03} &  \ms{-0.94}{0.06} &  \ms{-0.97}{0.03}   \\
%         80\% &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{-0.87}{0.10} &  \ms{\textbf{-0.97}}{0.03} &  \ms{-0.95}{0.04} &  \ms{\textbf{-0.97}}{0.03}   \\
%         85\% &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{-0.77}{0.17} &  \ms{\textbf{-0.91}}{0.09} &  \ms{\textbf{-0.91}}{0.08} &  \ms{-0.89}{0.08}   \\
        
%         90\% &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{-0.57}{0.20} &  \ms{\textbf{-0.97}}{0.03} &  \ms{-0.91}{0.11} &  \ms{-0.90}{0.08}   \\
%         95\% &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{N/A}{N/A} &  \ms{-0.26}{0.17} &  \ms{-0.89}{0.09} &  \ms{\textbf{-0.94}}{0.04} &  \ms{-0.91}{0.07}   \\
%         \midrule   
%         Avg. Rank & 5.26 & 5.00 & 5.26 & 3.37 & \textbf{1.26} & 1.95 & 2.37 \\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table*}



==> experiments/Boiler/spearman_correlation_global.tex <==
\begin{table*}[h]
    \centering
        \caption{Global Spearman rank correlation results on Boiler dataset which compares the average fidelity of different explanation size between $5\%$ to $95\%$. The best performance is marked as bold. For R-Fidelity and F-Fidelity, $\alpha^+=\alpha^-=0.5$. In F-Fidelity, $\beta=0.1$. In this table, w/ means the fine-tuned model as the model to be explained, while w/o means the original one.}
    \label{tab:exp:boiler:global:correlation}
    \scalebox{0.75}{
     \begin{tabular}{ccccccccccc}
        \toprule
        \multirow{2}{*}{Model} &
        \multirow{2}{*}{Correlation} &
        \multicolumn{2}{c}{Fidelity} &
        \multicolumn{1}{c}{ROAR} &
        \multicolumn{2}{c}{R-Fidelity} & 
        \multicolumn{2}{c}{F-Fidelity} \\
        \cmidrule(r){3-4} \cmidrule(r){5-5} \cmidrule(r){6-7} \cmidrule(r){8-9} 
        & &  origin  & fine-tune   & retrain  & origin  & fine-tune   & origin  & fine-tune  \\
        % Model & Correlation & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
         \midrule   
        % & \multicolumn{4}{c}{Local Spearman Correlation $\downarrow$} \\ 
        % \hline
        \multirow{3}{*}{\rotatebox[origin=c]{90}{LSTM}}
        % \multirow{3}{\rotatebox[origin=c]{90}{Res.}} \ms{-0.68}{0.08}
        & MoRF VS GT $\downarrow$   &\ms{-0.98}{0.03} &\ms{-1.00}{0.00} &\ms{-0.99}{0.2}  &\ms{-1.00}{0.00} &\ms{-0.94}{0.06} &\ms{-1.00}{0.00} &\ms{-1.00}{0.00}\\
        & LeRF VS GT $\uparrow$     &\ms{0.22}{0.03}  &\ms{0.65}{0.06} &\ms{0.36}{0.11}   &\ms{0.53}{0.06}  &\ms{0.93}{0.06}  &\ms{0.78}{0.02}  &\ms{0.86}{0.07}\\
        & MoRF VS LeRF $\downarrow$ &\ms{-0.27}{0.08} &\ms{-0.65}{0.06} &\ms{-0.38}{0.14} &\ms{-0.53}{0.06} &\ms{-0.99}{0.02} &\ms{-0.78}{0.02} & \ms{-0.86}{0.07}\\
        \hline
        \multirow{3}{*}{\rotatebox[origin=c]{90}{Trans.}}
        % \multirow{3}{\rotatebox[origin=c]{90}{ViT}}  \ms{\textbf{1.00}}{0.00}
        & MoRF VS GT $\downarrow$ & \ms{-0.84}{0.04} & \ms{-0.91}{0.07} & \ms{-0.71}{0.22}& \ms{-0.96}{0.05} & \ms{-0.90}{0.10}& \ms{-0.91}{0.08}& \ms{-0.66}{0.21}\\
        & LeRF VS GT $\uparrow$ & \ms{0.81}{0.12}    & \ms{0.91}{0.05}  & \ms{0.75}{0.14}& \ms{0.90}{0.08}   & \ms{0.87}{0.09} & \ms{0.91}{0.05}& \ms{-0.69}{0.19}\\
        & MoRF VS LeRF $\downarrow$ & \ms{-0.67}{0.19}& \ms{-0.86}{0.08}& \ms{-0.61}{0.30}& \ms{-0.86}{0.06} & \ms{-0.86}{0.05}& \ms{-0.87}{0.14}&\ms{-0.38}{0.48}\\
        
        \bottomrule
    \end{tabular}
    }
\end{table*}



==> experiments/Boiler/spearman_correlation_local.tex <==
\begin{table*}[h]
    \centering
        \caption{Local Spearman rank correlation results on PAM dataset. We report the total number of top-1 ranks at each sparsity between $5\%$ to $95\%$. The best performance is marked as bold. Other settings are the same as Table~\ref{tab:exp:pam:global:correlation}}
    \label{tab:exp:boiler:local:correlation_rank}
    \scalebox{0.75}{
     \begin{tabular}{cccccccccc}
        \toprule
        \multirow{2}{*}{Model} &
        \multirow{2}{*}{Top-1 Ranks } &
        \multicolumn{2}{c}{Fidelity} &
        \multicolumn{2}{c}{ROAR} &
        \multicolumn{2}{c}{R-Fidelity} & 
        \multicolumn{2}{c}{F-Fidelity} \\
        \cmidrule(r){3-4} \cmidrule(r){5-6} \cmidrule(r){7-8} \cmidrule(r){9-10} 
        & &  w/o  & w/  & w/o  & w/  & w/o  & w/  & w/o  & w/  \\
        % Model & Correlation & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
         \midrule   
        % & \multicolumn{4}{c}{Local Spearman Correlation $\downarrow$} \\ 
        % \hline
        \multirow{3}{*}{\rotatebox[origin=c]{90}{LSTM}}
        % \multirow{3}{\rotatebox[origin=c]{90}{Res.}} 
        & MoRF VS GT  & \\
        & LeRF VS GT & \\
        & MoRF VS LeRF & \\
        \hline
        \multirow{3}{*}{\rotatebox[origin=c]{90}{Trans.}}
        % \multirow{3}{\rotatebox[origin=c]{90}{ViT}}  \ms{\textbf{1.00}}{0.00}
        & MoRF VS GT  &  \\
        & LeRF VS GT  & \\
        & MoRF VS LeRF & \\
        \bottomrule
    \end{tabular}
    }
\end{table*}



==> experiments/Boiler/transformer_correlation_detail.tex <==
\begin{table*}[h]
    \centering
        \caption{"MoRF VS GT" Local Spearman rank correlation results on Boiler dataset with Transformer as the model to be explained.}
    \label{tab:exp:PAM:tansformer:local:morf_rank}
    \scalebox{0.75}{
     \begin{tabular}{cccccccc}
        \toprule
        &
        \multicolumn{2}{c}{Fidelity} &
        \multicolumn{1}{c}{ROAR} &
        \multicolumn{2}{c}{R-Fidelity} & 
        \multicolumn{2}{c}{F-Fidelity} \\
        \cmidrule(r){2-3} \cmidrule(r){4-4} \cmidrule(r){5-6} \cmidrule(r){7-8}
        Sparsity &  origin  & fine-tune  & retrain  & origin  & fine-tune & origin  & fine-tune  \\
        % Model & Correlation & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
         \midrule   
        % & \multicolumn{4}{c}{Local Spearman Correlation $\downarrow$} \\ 
        % \hline
        % \multirow{3}{\rotatebox[origin=c]{90}{ViT}}  \ms{\textbf{1.00}}{0.00}
        $5\%$&  \ms{-0.85}{0.06} &  \ms{-0.79}{0.28}&  \ms{-0.46}{0.30}&  \ms{-0.89}{0.04}&  \ms{-0.70}{0.22} &  \ms{-0.81}{0.18}&  \ms{-0.43}{0.21}\\
        10\% &  \ms{-0.93}{0.08} &  \ms{-0.90}{0.07}&  \ms{-0.45}{0.20}&  \ms{-0.95}{0.04}&  \ms{-0.78}{0.19}&  \ms{-0.91}{0.07}&  \ms{-0.75}{0.16}\\
        15\% &  \ms{-1.00}{0.00}&  \ms{-0.94}{0.06}&  \ms{-0.78}{0.18}&  \ms{-0.98}{0.05}&  \ms{-0.91}{0.08}&  \ms{-0.97}{0.03}&  \ms{-0.81}{0.11}\\
        20\% &  \ms{-1.00}{0.01}&  \ms{-0.97}{0.03}&  \ms{-0.94}{0.06}&  \ms{-1.00}{0.00}&  \ms{-0.93}{0.06}&  \ms{-0.98}{0.03}&  \ms{-0.91}{0.05}\\
        25\% &  \ms{-0.80}{0.11}&  \ms{-1.00}{0.00}&  \ms{-0.97}{0.03}&  \ms{-1.00}{0.00}&  \ms{-0.95}{0.02}&  \ms{-0.99}{0.02}&  \ms{-0.91}{0.05}\\
        
        30\% &  \ms{-0.74}{0.17}&  \ms{-0.97}{0.04}&  \ms{-0.94}{0.00}&  \ms{-1.00}{0.00}&  \ms{-0.98}{0.03}&  \ms{-0.98}{0.03}&  \ms{-0.91}{0.05}\\
        35\% &  \ms{-0.52}{0.25}&  \ms{-0.98}{0.03}&  \ms{-0.84}{0.10}&  \ms{-1.00}{0.00}&  \ms{-0.98}{0.03}&  \ms{-0.99}{0.02}&  \ms{-0.87}{0.09}\\
        40\% &  \ms{-0.10}{0.24}&  \ms{-0.89}{0.08}&  \ms{-0.48}{0.24}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-0.98}{0.03}&  \ms{-0.86}{0.09}\\
        45\% &  \ms{0.01}{0.29}&  \ms{-0.88}{0.09}&  \ms{-0.10}{0.36}&  \ms{-0.98}{0.03}&  \ms{-0.97}{0.05}&  \ms{-0.99}{0.02}&  \ms{-0.85}{0.08}\\
        50\% &  \ms{0.01}{0.29}&  \ms{-0.86}{0.10}&  \ms{0.04}{0.31}&  \ms{-0.95}{0.04}&  \ms{-0.97}{0.05}&  \ms{-0.92}{0.08}&  \ms{-0.81}{0.15}\\
        55\% &  \ms{0.01}{0.29}&  \ms{-0.82}{0.08}&  \ms{0.16}{0.23}&  \ms{-0.94}{0.05}&  \ms{-0.97}{0.05}&  \ms{-0.92}{0.08}&  \ms{-0.66}{0.24}\\
        
        60\% &  \ms{0.01}{0.29}&  \ms{-0.76}{0.13}&  \ms{0.30}{0.20}&  \ms{-0.92}{0.06}&  \ms{-0.95}{0.06}&  \ms{-0.91}{0.08}&  \ms{-0.54}{0.19}\\
        65\% &  \ms{0.01}{0.29}&  \ms{-0.49}{0.17}&  \ms{0.32}{0.19}&  \ms{-0.87}{0.07}&  \ms{-0.84}{0.13}&  \ms{-0.78}{0.10}&  \ms{-0.43}{0.16}\\
        70\% &  \ms{0.01}{0.29}&  \ms{-0.40}{0.30}&  \ms{0.30}{0.20}&  \ms{-0.76}{0.15}&  \ms{-0.71}{0.24}&  \ms{-0.63}{0.15}&  \ms{0.02}{0.15}\\
        75\% &  \ms{0.01}{0.29}&  \ms{-0.36}{0.29}&  \ms{0.30}{0.20}&  \ms{-0.53}{0.29}&  \ms{-0.62}{0.33}&  \ms{-0.55}{0.23}&  \ms{0.37}{0.25}\\
        80\% &  \ms{0.01}{0.29}&  \ms{-0.28}{0.37}&  \ms{0.29}{0.19}&  \ms{-0.37}{0.38}&  \ms{-0.51}{0.26}&  \ms{-0.52}{0.21}&  \ms{0.41}{0.16}\\
        85\% &  \ms{0.01}{0.29}&  \ms{-0.28}{0.37}&  \ms{0.31}{0.18}&  \ms{-0.15}{0.46}&  \ms{-0.37}{0.31}&  \ms{-0.44}{0.27}&  \ms{0.54}{0.24}\\
        
        90\% &  \ms{0.01}{0.29}&  \ms{-0.28}{0.37}&  \ms{0.39}{0.24}&  \ms{0.06}{0.47}&  \ms{-0.19}{0.24}&  \ms{-0.27}{0.37}&  \ms{0.51}{0.21}\\
        95\% &  \ms{0.01}{0.29}&  \ms{-0.28}{0.37}&  \ms{0.52}{0.08}&  \ms{0.14}{0.33}&  \ms{-0.19}{0.25}&  \ms{-0.09}{0.49}&  \ms{0.57}{0.16}\\
        \midrule   
        Avg. Rank \\
        \bottomrule
    \end{tabular}
    }
\end{table*}

\begin{table*}[h]
    \centering
        \caption{"LeRF VS GT" Local Spearman rank correlation results on Boiler dataset with Transformer as the model to be explained.}
    \label{tab:exp:PAM:tansformer:local:lerf_rank}
    \scalebox{0.75}{
     \begin{tabular}{cccccccccc}
        \toprule
        &
        \multicolumn{2}{c}{Fidelity} &
        \multicolumn{1}{c}{ROAR} &
        \multicolumn{2}{c}{R-Fidelity} & 
        \multicolumn{2}{c}{F-Fidelity} \\
        \cmidrule(r){2-3} \cmidrule(r){4-4} \cmidrule(r){5-6} \cmidrule(r){7-8}
        Sparsity &  origin  & fine-tune  & retrain  & origin  & fine-tune & origin  & fine-tune  \\
        % Model & Correlation & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
         \midrule   
        % & \multicolumn{4}{c}{Local Spearman Correlation $\downarrow$} \\ 
        % \hline
        % \multirow{3}{\rotatebox[origin=c]{90}{ViT}}  \ms{\textbf{1.00}}{0.00}
        $5\%$& \ms{0.43}{0.34}& \ms{0.38}{0.22} & \ms{-0.49}{0.29} & \ms{0.10}{0.47}& \ms{0.76}{0.15} & \ms{0.79}{0.08} & \ms{0.04}{0.46} \\
        10\% & \ms{0.43}{0.34}& \ms{0.38}{0.22} & \ms{-0.48}{0.25} & \ms{0.45}{0.36}& \ms{0.97}{0.03} & \ms{0.84}{0.09} & \ms{0.28}{0.41} \\
        15\% & \ms{0.43}{0.34}& \ms{0.43}{0.27} & \ms{-0.47}{0.25} & \ms{0.78}{0.12}& \ms{0.97}{0.03}  & \ms{0.89}{0.08} & \ms{0.45}{0.35} \\
        20\% & \ms{0.43}{0.34}& \ms{0.56}{0.25} & \ms{-0.47}{0.25}& \ms{0.85}{0.08}& \ms{0.98}{0.03}  & \ms{0.92}{0.06} & \ms{0.44}{0.31} \\
        25\% & \ms{0.43}{0.34}& \ms{0.85}{0.10} & \ms{-0.48}{0.25}& \ms{0.92}{0.08}& \ms{0.97}{0.05}  & \ms{0.93}{0.02} & \ms{0.65}{0.19} \\
        
        30\% & \ms{0.43}{0.34}& \ms{0.97}{0.03} & \ms{-0.45}{0.24}& \ms{0.93}{0.06}& \ms{0.97}{0.03} & \ms{0.98}{0.03} & \ms{0.74}{0.12} \\
        35\% & \ms{0.69}{0.22}& \ms{0.98}{0.03} & \ms{-0.12}{0.21}& \ms{0.99}{0.02}& \ms{0.98}{0.03}& \ms{1.00}{0.00} & \ms{0.81}{0.14} \\
        40\% & \ms{0.79}{0.13}& \ms{0.97}{0.03} & \ms{0.73}{0.16}& \ms{0.99}{0.02}& \ms{0.98}{0.03}& \ms{1.00}{0.00} & \ms{0.84}{0.08} \\
        45\% & \ms{0.94}{0.03}& \ms{0.99}{0.02} & \ms{0.82}{0.11}& \ms{1.00}{0.00}& \ms{0.99}{0.03}& \ms{1.00}{0.00} & \ms{0.94}{0.00} \\
        50\% &  \ms{0.97}{0.30}& \ms{0.99}{0.02}& \ms{0.97}{0.04}& \ms{0.98}{0.03} & \ms{0.95}{0.04}& \ms{1.00}{0.00} & \ms{0.92}{0.08} \\
        55\% & \ms{0.99}{0.02} & \ms{0.96}{0.05}& \ms{0.93}{0.06}& \ms{0.94}{0.06}& \ms{0.95}{0.02}& \ms{0.98}{0.03} & \ms{0.95}{0.02} \\
        
        60\% & \ms{1.00}{0.00} & \ms{0.95}{0.04}& \ms{0.89}{0.06}& \ms{0.94}{0.06}& \ms{0.94}{0.00}& \ms{0.99}{0.02} & \ms{0.94}{0.06} \\
        65\% & \ms{0.95}{0.02} & \ms{0.82}{0.12}& \ms{0.91}{0.09}& \ms{0.91}{0.07}& \ms{0.87}{0.14}& \ms{0.93}{0.07} & \ms{0.95}{0.07} \\
        70\% & \ms{0.85}{0.05} & \ms{0.82}{0.09}& \ms{0.81}{0.13}& \ms{0.86}{0.10}& \ms{0.87}{0.14}& \ms{0.97}{0.03} & \ms{0.93}{0.06} \\
        75\% & \ms{0.81}{0.02} & \ms{0.69}{0.13}& \ms{0.57}{0.13}& \ms{0.73}{0.13}& \ms{0.82}{0.14}& \ms{0.86}{0.13} & \ms{0.90}{0.06} \\
        80\% & \ms{0.58}{0.13} & \ms{0.71}{0.14}& \ms{0.45}{0.02}& \ms{0.67}{0.12}& \ms{0.69}{0.18}& \ms{0.73}{0.14} & \ms{0.71}{0.28} \\
        85\% & \ms{0.42}{0.10} & \ms{0.43}{0.28}& \ms{0.21}{0.20}& \ms{0.55}{0.19}& \ms{0.60}{0.22}& \ms{0.72}{0.11} & \ms{0.55}{0.20} \\
        
        90\% & \ms{0.22}{0.18} & \ms{0.40}{0.29}& \ms{0.05}{0.13}& \ms{0.45}{0.26}& \ms{0.52}{0.20}& \ms{0.34}{0.20} & \ms{0.26}{0.26} \\
        95\% &  \ms{0.42}{0.11}& \ms{0.41}{0.29}& \ms{-0.26}{0.36}& \ms{0.41}{0.30}& \ms{0.44}{0.23}& \ms{0.39}{0.20} & \ms{0.27}{0.29} \\
        \midrule   
        Avg. Rank \\
        \bottomrule
    \end{tabular}
    }
\end{table*}


\begin{table*}[h]
    \centering
        \caption{"MoRF VS LeRF" Local Spearman rank correlation results on Boiler dataset with Transformer as the model to be explained.}
    \label{tab:exp:PAM:tansformer:local:morf_lerf}
    \scalebox{0.75}{
     \begin{tabular}{cccccccc}
        \toprule
        &
        \multicolumn{2}{c}{Fidelity} &
        \multicolumn{1}{c}{ROAR} &
        \multicolumn{2}{c}{R-Fidelity} & 
        \multicolumn{2}{c}{F-Fidelity} \\
        \cmidrule(r){2-3} \cmidrule(r){4-4} \cmidrule(r){5-6} \cmidrule(r){7-8}
        Sparsity &  origin  & fine-tune  & retrain  & origin  & fine-tune & origin  & fine-tune  \\
        % Model & Correlation & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
         \midrule   
        % & \multicolumn{4}{c}{Local Spearman Correlation $\downarrow$} \\ 
        % \hline
        % \multirow{3}{\rotatebox[origin=c]{90}{ViT}}  \ms{\textbf{1.00}}{0.00}
        $5\%$& \ms{-0.25}{0.40} & \ms{-0.27}{0.18}& \ms{0.37}{0.27}& \ms{0.01}{0.42} & \ms{-0.61}{0.22} & \ms{-0.69}{0.19} & \ms{-0.12}{0.44}\\
        10\% & \ms{-0.40}{0.41} & \ms{-0.30}{0.27}& \ms{0.24}{0.24}& \ms{-0.41}{0.30}& \ms{-0.81}{0.19}& \ms{-0.82}{0.23}& \ms{-0.17}{0.51}\\
        15\% &  \ms{-0.43}{0.34}& \ms{-0.41}{0.30}& \ms{0.42}{0.23}& \ms{-0.73}{0.13}& \ms{-0.90}{0.08}& \ms{-0.89}{0.15}& \ms{-0.31}{0.32}\\
        20\% & \ms{-0.43}{0.34} & \ms{-0.55}{0.25}& \ms{0.49}{0.17}& \ms{-0.85}{0.08}& \ms{-0.93}{0.06}& \ms{-0.92}{0.06}& \ms{-0.41}{0.30}\\
        25\% &  \ms{-0.33}{0.34}& \ms{-0.85}{0.10}& \ms{0.48}{0.25}& \ms{-0.92}{0.08}& \ms{-0.97}{0.02}& \ms{-0.92}{0.03}& \ms{-0.58}{0.22}\\
        
        30\% & \ms{-0.32}{0.25} & \ms{-0.95}{0.04}& \ms{0.24}{0.30}& \ms{-0.93}{0.06}& \ms{-0.99}{0.03}& \ms{-0.98}{0.03}& \ms{-0.67}{0.20}\\
        35\% &  \ms{-0.31}{0.09}& \ms{-0.97}{0.03}& \ms{-0.07}{0.16}& \ms{-0.99}{0.02}& \ms{-0.98}{0.03}& \ms{-0.99}{0.02}& \ms{-0.65}{0.24}\\
        40\% &  \ms{-0.01}{0.40}& \ms{-0.89}{0.06}& \ms{-0.14}{0.32}& \ms{-0.99}{0.02}& \ms{-0.98}{0.03}& \ms{-0.98}{0.03}& \ms{-0.61}{0.30}\\
        45\% &  \ms{0.02}{0.33}& \ms{-0.89}{0.08}& \ms{0.12}{0.42}& \ms{-0.98}{0.03}& \ms{-0.95}{0.04}& \ms{-0.99}{0.02}& \ms{-0.81}{0.15}\\
        50\% &  \ms{0.07}{0.29}& \ms{-0.85}{0.08}& \ms{0.17}{0.32}& \ms{-0.93}{0.04}& \ms{-0.92}{0.05}& \ms{-0.92}{0.08}& \ms{-0.68}{0.22}\\
        55\% &  \ms{0.03}{0.32}& \ms{-0.79}{0.11}& \ms{0.21}{0.24}& \ms{-0.91}{0.05}& \ms{-0.92}{0.03}& \ms{-0.90}{0.08}& \ms{-0.59}{0.28}\\
        
        60\% &  \ms{0.01}{0.29}& \ms{-0.77}{0.12}& \ms{0.32}{0.13}& \ms{-0.87}{0.06}& \ms{-0.94}{0.00}& \ms{-0.90}{0.08}& \ms{-0.45}{0.32}\\
        65\% &  \ms{-0.15}{0.24}& \ms{-0.37}{0.28}& \ms{0.33}{0.18}& \ms{-0.87}{0.07}& \ms{-0.81}{0.17}& \ms{-0.79}{0.11}& \ms{-0.30}{0.26}\\
        70\% &  \ms{-0.05}{0.35}& \ms{-0.24}{0.24}& \ms{0.31}{0.12}& \ms{-0.81}{0.09}& \ms{-0.78}{0.14}& \ms{-0.67}{0.23}& \ms{0.11}{0.27}\\
        75\% &  \ms{-0.08}{0.28}& \ms{-0.22}{0.41}& \ms{0.22}{0.17}& \ms{-0.46}{0.16}& \ms{-0.73}{0.16}& \ms{-0.66}{0.33}& \ms{0.39}{0.37}\\
        80\% &  \ms{0.11}{0.51}& \ms{0.11}{0.47}& \ms{0.29}{0.11}& \ms{-0.34}{0.27}& \ms{-0.54}{0.11}& \ms{-0.65}{0.23}& \ms{0.34}{0.43}\\
        85\% &  \ms{0.11}{0.58}& \ms{-0.09}{0.49}& \ms{0.48}{0.24}& \ms{-0.18}{0.31}& \ms{-0.60}{0.14}& \ms{-0.43}{0.31}& \ms{0.31}{0.33}\\
        
        90\% &  \ms{-0.13}{0.30}& \ms{-0.01}{0.49}& \ms{0.42}{0.33}& \ms{0.10}{0.13}& \ms{-0.29}{0.19}& \ms{-0.38}{0.22}& \ms{0.25}{0.31}\\
        95\% &  \ms{0.16}{0.16}& \ms{0.16}{0.50}& \ms{0.12}{0.38}& \ms{0.23}{0.33}& \ms{-0.37}{0.18}& \ms{-0.11}{0.41}& \ms{0.33}{0.24}\\
        \midrule   
        Avg. Rank \\
        \bottomrule
    \end{tabular}
    }
\end{table*}



==> experiments/Boiler/transformer_fid_images.tex <==
\begin{table*}[h]
    \centering
        \caption{Fidelity results on Boiler dataset with Transformer as the model to be explained. }
    \label{tab:exp:pam:transformere:fid}
    \scalebox{1.0}{
     \begin{tabular}{ccccc}
        \toprule
         & \multicolumn{2}{c}{$Fid^+$} & \multicolumn{2}{c}{$Fid^-$} \\ 
        \cmidrule(r){2-3} \cmidrule(r){4-5} 
        Methods &  origin  & fine-tune/retrain  & origin & fine-tune/retrain\\ 
        
        \midrule 
        \rotatebox[origin=c]{90}{Fidelity}
        &
        \begin{minipage}[b]{0.20\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/Boiler/transformer/image_ori_transformer_split_ori_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.20\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/Boiler/transformer/image_finetune_transformer-finetune_split_ori_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.20\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/Boiler/transformer/image_ori_transformer_split_ori_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.20\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/Boiler/transformer/image_finetune_transformer-finetune_split_ori_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        \\

        \rotatebox[origin=c]{90}{ROAR}
        &
        \begin{minipage}[b]{0.20\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/Boiler/transformer/image_ori_transformer_split_ori_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.20\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/Boiler/transformer/image_ori_transformer_split_roar_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.20\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/Boiler/transformer/image_ori_transformer_split_ori_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.20\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/Boiler/transformer/image_ori_transformer_split_roar_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        \\
    
        \rotatebox[origin=c]{90}{R-Fidelity}
        &
        \begin{minipage}[b]{0.20\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/Boiler/transformer/image_ori_transformer_split_rfid_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.20\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/Boiler/transformer/image_finetune_transformer-finetune_split_rfid_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.20\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/Boiler/transformer/image_ori_transformer_split_rfid_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.20\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/Boiler/transformer/image_finetune_transformer-finetune_split_rfid_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        \\

        \rotatebox[origin=c]{90}{F-Fidelity}
        &
        \begin{minipage}[b]{0.20\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/Boiler/transformer/image_ori_transformer_split_ffid_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.20\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/Boiler/transformer/image_finetune_transformer-finetune_split_ffid_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.20\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/Boiler/transformer/image_ori_transformer_split_ffid_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.20\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/Boiler/transformer/image_finetune_transformer-finetune_split_ffid_interv0.2_gradcam_leRF.png}}
	  \end{minipage} \\
        
        \bottomrule
        
    \end{tabular}
    }
\end{table*}


==> experiments/BoolQ/spearman_correlation.tex <==
\begin{table*}[h]
    \centering
        \caption{Spearman rank correlation and rank results on BoolQ dataset with LSTM and Transformer. }
    \label{tab:exp:boolq:correlation}
    \scalebox{0.9}{
     \begin{tabular}{ccccc|ccc}
        \toprule
        \multirow{2}{*}{} &
        \multirow{2}{*}{Correlation} &
        \multicolumn{3}{c}{LSTM} &
        \multicolumn{3}{c}{Transformer} \\
        \cmidrule(r){3-5} \cmidrule(r){6-8}
        & & 
        Fidelity &
        R-Fidelity & 
        F-Fidelity & 
        Fidelity &
        R-Fidelity & 
        F-Fidelity\\
         \midrule   
        \multirow{3}{*}{\rotatebox[origin=c]{90}{\shortstack{Macro \\ Corr.}}}
        & MoRF vs GT $\downarrow$   & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        & LeRF vs GT $\uparrow$     & \ms{\textbf{1.00}}{0.00}   & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}   & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} \\
        & MoRF vs LeRF $\downarrow$ & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00}\\
        \midrule
        \multirow{3}{*}{\rotatebox[origin=c]{90}{\shortstack{Micro \\ Corr.}}}
        & MoRF vs GT  $\downarrow$  & \ms{\textbf{-1.00}}{0.01} & \ms{\textbf{-1.00}}{0.01} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.01} & \ms{\textbf{-1.00}}{0.01} & \ms{\textbf{-1.00}}{0.00}\\
        & LeRF vs GT  $\uparrow$    & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}   & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}\\
        & MoRF vs LeRF $\downarrow$ & \ms{\textbf{-1.00}}{0.01} & \ms{\textbf{-1.00}}{0.01} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00}\\
        \midrule
        \multirow{3}{*}{\rotatebox[origin=c]{90}{\shortstack{Micro \\ Rank}}}
        & MoRF vs GT $\downarrow$  & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
        & LeRF vs GT  $\downarrow$ & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
        & MoRF vs LeRF $\downarrow$& \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
        \bottomrule
    \end{tabular}
    }
\end{table*}

==> experiments/PAM/lstm_correlation_detail.tex <==
\begin{table*}[h]
    \centering
    \caption{Micro Spearman rank correlation results on PAM dataset with LSTM as the model to be explained.}
    \label{tab:exp:PAM:LSTM:local:local:combined}
    \scalebox{0.6}{
     \begin{tabular}{c|cccc|cccc|cccc}
        \toprule
        & \multicolumn{4}{c|}{MoRF vs GT} & \multicolumn{4}{c|}{LeRF vs GT} & \multicolumn{4}{c}{MoRF vs LeRF} \\
        Sparsity & Fidelity & ROAR & R-Fidelity & F-Fidelity & Fidelity & ROAR & R-Fidelity & F-Fidelity & Fidelity & ROAR & R-Fidelity & F-Fidelity \\
        \midrule   
5\% & \ms{-0.99}{0.02} & \ms{-0.94}{0.05} & \ms{\textbf{-1.00}}{0.00} & \ms{-0.99}{0.00} & \ms{0.99}{0.02} & \ms{0.91}{0.05} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.98}{0.03} & \ms{-0.88}{0.07} & \ms{\textbf{-1.00}}{0.00} & \ms{-0.99}{0.02}\\
10\% & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.01} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{0.88}{0.07} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{-0.88}{0.07} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00}\\
15\% & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{0.94}{0.07} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{-0.94}{0.07} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00}\\
20\% & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.01} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.01} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00}\\
25\% & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.01} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00}\\
30\% & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{0.98}{0.03} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{-0.98}{0.03} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00}\\
35\% & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.01} & \ms{0.79}{0.08} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{-1.00}}{0.01} & \ms{-0.79}{0.08} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00}\\
40\% & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{0.92}{0.06} & \ms{0.57}{0.23} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.92}{0.06} & \ms{-0.57}{0.23} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00}\\
45\% & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{0.55}{0.12} & \ms{0.21}{0.31} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.55}{0.12} & \ms{-0.21}{0.31} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00}\\
50\% & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{0.26}{0.00} & \ms{0.71}{0.08} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.26}{0.00} & \ms{-0.71}{0.08} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00}\\
55\% & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{-0.02}{0.13} & \ms{0.67}{0.16} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{0.02}{0.13} & \ms{-0.67}{0.16} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00}\\
60\% & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{0.12}{0.16} & \ms{0.63}{0.17} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.12}{0.16} & \ms{-0.63}{0.17} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00}\\
65\% & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{0.24}{0.18} & \ms{0.92}{0.08} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.24}{0.18} & \ms{-0.92}{0.08} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00}\\
70\% & \ms{-0.99}{0.02} & \ms{-0.99}{0.02} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{0.72}{0.04} & \ms{0.43}{0.33} & \ms{\textbf{1.00}}{0.02} & \ms{\textbf{1.00}}{0.00} & \ms{-0.75}{0.05} & \ms{-0.42}{0.33} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00}\\
75\% & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{0.89}{0.03} & \ms{0.86}{0.16} & \ms{0.99}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.89}{0.03} & \ms{-0.86}{0.16} & \ms{-0.99}{0.02} & \ms{\textbf{-1.00}}{0.00}\\
80\% & \ms{-0.94}{0.06} & \ms{-0.99}{0.01} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{0.78}{0.11} & \ms{0.88}{0.09} & \ms{\textbf{1.00}}{0.02} & \ms{\textbf{1.00}}{0.00} & \ms{-0.70}{0.19} & \ms{-0.87}{0.11} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00}\\
85\% & \ms{-0.97}{0.02} & \ms{-0.99}{0.01} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{0.96}{0.05} & \ms{0.97}{0.02} & \ms{0.99}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.93}{0.06} & \ms{-0.97}{0.03} & \ms{-0.99}{0.02} & \ms{\textbf{-1.00}}{0.00}\\
90\% & \ms{-0.65}{0.22} & \ms{-0.87}{0.06} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{0.72}{0.16} & \ms{0.91}{0.09} & \ms{\textbf{1.00}}{0.00} & \ms{0.99}{0.02} & \ms{-0.76}{0.22} & \ms{-0.79}{0.11} & \ms{\textbf{-1.00}}{0.00} & \ms{-0.99}{0.02}\\
95\% & \ms{0.75}{0.23} & \ms{-0.62}{0.30} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{0.85}{0.06} & \ms{0.91}{0.08} & \ms{0.98}{0.02} & \ms{0.99}{0.02} & \ms{0.69}{0.19} & \ms{-0.57}{0.34} & \ms{-0.98}{0.03} & \ms{\textbf{-0.99}}{0.02}\\
        \midrule   
Avg. Rank & 1.53 & 1.37 & \textbf{1.00} & 1.05 & 2.32 & 2.37 & 1.16 & \textbf{1.05} & 2.37 & 2.42 & 1.16 & \textbf{1.11} \\
        \bottomrule
    \end{tabular}
    }
\end{table*}


% \begin{table*}[h]
%     \centering
%         \caption{"MoRF VS GT" Local Spearman rank correlation results on PAM dataset with LSTM as the model to be explained.}
%     \label{tab:exp:PAM:LSTM:local:morf_rank}
%     \scalebox{0.75}{
%      \begin{tabular}{cccccccc}
%         \toprule
%         &
%         \multicolumn{2}{c}{Fidelity} &
%         \multicolumn{1}{c}{ROAR} &
%         \multicolumn{2}{c}{R-Fidelity} & 
%         \multicolumn{2}{c}{F-Fidelity} \\
%         \cmidrule(r){2-3} \cmidrule(r){4-4} \cmidrule(r){5-6} \cmidrule(r){7-8}
%         Sparsity &  origin  & fine-tune & retrain & origin  & fine-tune  & origin  & fine-tune  \\
%         % Model & Correlation & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
%          \midrule   
%         % & \multicolumn{4}{c}{Local Spearman Correlation $\downarrow$} \\ 
%         % \hline
%         % \multirow{3}{\rotatebox[origin=c]{90}{ViT}}  \ms{\textbf{1.00}}{0.00}
%         5\%&  \ms{-0.99}{0.02}&  \ms{-0.99}{0.02}&  \ms{-0.94}{0.05}&  \ms{\textbf{-1.00}}{0.00}&  \ms{-0.99}{0.00}&  \ms{\textbf{-1.00}}{0.00} &  \ms{-0.99}{0.02}\\
%         10\% &  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.01}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         15\% &  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         20\% &  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         25\% &  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
        
%         30\% &  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         35\% &  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         40\% &  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         45\% &  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         50\% &  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         55\% &  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
        
%         60\% &  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         65\% &  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         70\% &  \ms{-0.99}{0.02}&  \ms{\textbf{-1.00}}{0.00}&  \ms{-0.99}{0.02}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         75\% &  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00} &  \ms{-0.99}{0.02}\\
%         80\% &  \ms{-0.94}{0.06}&  \ms{-0.99}{0.02}&  \ms{-0.99}{0.01}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{-0.99}{0.02} &  \ms{\textbf{-1.00}}{0.00}\\
%         85\% &  \ms{-0.97}{0.02}&  \ms{-0.99}{0.02}&  \ms{-0.99}{0.01}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
        
%         90\% &  \ms{-0.65}{0.22}&  \ms{-0.91}{0.08}&  \ms{-0.87}{0.06}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         95\% &  \ms{0.75}{0.23}&  \ms{-0.80}{0.12}&  \ms{-0.62}{0.30}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{-0.99}{0.02} &  \ms{-0.87}{0.09}\\
%         \midrule   
%         Avg. Rank & 2.63 & 1.89 & 2.47 & 1.00 & \textbf{1.11} & 1.26 & 1.58\\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table*}

% \begin{table*}[h]
%     \centering
%         \caption{"LeRF VS GT" Local Spearman rank correlation results on PAM dataset with LSTM as the model to be explained.}
%     \label{tab:exp:PAM:LSTM:local:lerf_rank}
%     \scalebox{0.75}{
%      \begin{tabular}{cccccccccc}
%         \toprule
%         &
%         \multicolumn{2}{c}{Fidelity} &
%         \multicolumn{1}{c}{ROAR} &
%         \multicolumn{2}{c}{R-Fidelity} & 
%         \multicolumn{2}{c}{F-Fidelity} \\
%         \cmidrule(r){2-3} \cmidrule(r){4-4} \cmidrule(r){5-6} \cmidrule(r){7-8}
%         Sparsity &  origin  & fine-tune & retrain & origin  & fine-tune  & origin  & fine-tune  \\
%         % Model & Correlation & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
%          \midrule   
%         % & \multicolumn{4}{c}{Local Spearman Correlation $\downarrow$} \\ 
%         % \hline
%         % \multirow{3}{\rotatebox[origin=c]{90}{ViT}}  \ms{\textbf{1.00}}{0.00}
        
%         $5\%$&  \ms{0.99}{0.02}&  \ms{0.68}{0.15}&  \ms{0.91}{0.05}&  \ms{\textbf{1.00}}{0.00}&  \ms{\textbf{1.00}}{0.00}&  \ms{0.99}{0.02} &  \ms{0.94}{0.06} \\
%         10\% &  \ms{\textbf{1.00}}{0.00}&  \ms{0.95}{0.02}&  \ms{0.88}{0.07}&  \ms{\textbf{1.00}}{0.00}&  \ms{\textbf{1.00}}{0.00}&  \ms{0.99}{0.02} &  \ms{0.93}{0.04}\\
%         15\% &  \ms{\textbf{1.00}}{0.00}&  \ms{0.99}{0.02}&  \ms{0.94}{0.07}&  \ms{\textbf{1.00}}{0.00}&  \ms{\textbf{1.00}}{0.00}&  \ms{\textbf{1.00}}{0.00} &  \ms{0.99}{0.02}\\
%         20\% &  \ms{\textbf{1.00}}{0.00}&  \ms{\textbf{1.00}}{0.00}&  \ms{\textbf{1.00}}{0.01}&  \ms{\textbf{1.00}}{0.00}&  \ms{\textbf{1.00}}{0.00}&  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         25\% &  \ms{\textbf{1.00}}{0.01}&  \ms{0.99}{0.02}&  \ms{\textbf{1.00}}{0.00}&  \ms{\textbf{1.00}}{0.00}&  \ms{\textbf{1.00}}{0.00}&  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
        
%         30\% &  \ms{\textbf{1.00}}{0.00}&  \ms{0.96}{0.02}&  \ms{0.98}{0.03}&  \ms{\textbf{1.00}}{0.00}&  \ms{\textbf{1.00}}{0.00}&  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         35\% &  \ms{\textbf{1.00}}{0.01}&  \ms{0.97}{0.04}&  \ms{0.79}{0.08}&  \ms{\textbf{1.00}}{0.00}&  \ms{\textbf{1.00}}{0.00}&  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         40\% &  \ms{0.92}{0.06}&  \ms{\textbf{1.00}}{0.00}&  \ms{0.57}{0.23}&  \ms{\textbf{1.00}}{0.00}&  \ms{\textbf{1.00}}{0.00}&  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         45\% &  \ms{0.55}{0.12}&  \ms{0.86}{0.08}&  \ms{0.21}{0.31}&  \ms{\textbf{1.00}}{0.00}&  \ms{\textbf{1.00}}{0.00}&  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         50\% &  \ms{0.26}{0.00}&  \ms{0.77}{0.15}&  \ms{0.71}{0.08}&  \ms{\textbf{1.00}}{0.00}&  \ms{\textbf{1.00}}{0.00}&  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         55\% &  \ms{-0.02}{0.13}&  \ms{0.89}{0.05}&  \ms{0.67}{0.16}&  \ms{\textbf{1.00}}{0.00}&  \ms{\textbf{1.00}}{0.00}&  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
        
%         60\% &  \ms{0.12}{0.16}&  \ms{0.95}{0.06}&  \ms{0.63}{0.17}&  \ms{\textbf{1.00}}{0.00}&  \ms{\textbf{1.00}}{0.00}&  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         65\% &  \ms{0.24}{0.18}&  \ms{0.98}{0.03}&  \ms{0.92}{0.08}&  \ms{\textbf{1.00}}{0.00}&  \ms{\textbf{1.00}}{0.00}&  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         70\% &  \ms{0.72}{0.04}&  \ms{0.94}{0.06}&  \ms{0.43}{0.33}&  \ms{\textbf{1.00}}{0.02}&  \ms{\textbf{1.00}}{0.00}&  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         75\% &  \ms{0.89}{0.03}&  \ms{0.92}{0.07}&  \ms{0.86}{0.16}&  \ms{0.99}{0.00}&  \ms{\textbf{1.00}}{0.00}&  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         80\% &  \ms{0.78}{0.11}&  \ms{0.85}{0.08}&  \ms{0.88}{0.09}&  \ms{\textbf{1.00}}{0.02}&  \ms{\textbf{1.00}}{0.00}&  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         85\% &  \ms{0.96}{0.05}&  \ms{0.99}{0.01}&  \ms{0.97}{0.02}&  \ms{0.99}{0.00}&  \ms{\textbf{1.00}}{0.00}&  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
        
%         90\% &  \ms{0.72}{0.16}&  \ms{0.95}{0.05}&  \ms{0.91}{0.09}&  \ms{\textbf{1.00}}{0.00}&  \ms{0.99}{0.02}&  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         95\% &  \ms{0.85}{0.06}&  \ms{0.96}{0.02}&  \ms{0.91}{0.08}&  \ms{0.98}{0.02}&  \ms{0.99}{0.02}&  \ms{0.97}{0.05} &  \ms{\textbf{1.00}}{0.00}\\
%         \midrule   
%         Avg. Rank & 4.68 & 4.95 & 5.79 & 1.42 & \textbf{1.21} & 1.42 & 1.68\\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table*}


% \begin{table*}[h]
%     \centering
%         \caption{"MoRF VS LeRF" Local Spearman rank correlation results on PAM dataset with LSTM as the model to be explained.}
%     \label{tab:exp:PAM:LSTM:local:morf_lerf}
%     \scalebox{0.75}{
%      \begin{tabular}{cccccccc}
%         \toprule
%         &
%         \multicolumn{2}{c}{Fidelity} &
%         \multicolumn{1}{c}{ROAR} &
%         \multicolumn{2}{c}{R-Fidelity} & 
%         \multicolumn{2}{c}{F-Fidelity} \\
%         \cmidrule(r){2-3} \cmidrule(r){4-4} \cmidrule(r){5-6} \cmidrule(r){7-8}
%         Sparsity &  origin  & fine-tune & retrain & origin  & fine-tune  & origin  & fine-tune  \\
%         % Model & Correlation & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
%          \midrule   
%         % & \multicolumn{4}{c}{Local Spearman Correlation $\downarrow$} \\ 
%         % \hline
%         % \multirow{3}{\rotatebox[origin=c]{90}{ViT}}  \ms{\textbf{1.00}}{0.00}
%         $5\%$&  \ms{-0.98}{0.03}&  \ms{-0.65}{0.12}&  \ms{-0.88}{0.07}&  \ms{\textbf{-1.00}}{0.00}&  \ms{-0.99}{0.02}&  \ms{-0.99}{0.02}&  \ms{-0.93}{0.07} \\
%         10\% &  \ms{\textbf{-1.00}}{0.00}&  \ms{-0.95}{0.02}&  \ms{-0.88}{0.07}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{-0.99}{0.02}&  \ms{-0.93}{0.04}\\
%         15\% &  \ms{\textbf{-1.00}}{0.00}&  \ms{-0.98}{0.02}&  \ms{-0.94}{0.07}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{-0.99}{0.02}\\
%         20\% &  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.01}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}\\
%         25\% &  \ms{\textbf{-1.00}}{0.00}&  \ms{-0.99}{0.02}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}\\
        
%         30\% &  \ms{\textbf{-1.00}}{0.00}&  \ms{-0.96}{0.02}&  \ms{-0.98}{0.03}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}\\
%         35\% &  \ms{\textbf{-1.00}}{0.01}&  \ms{-0.97}{0.04}&  \ms{-0.79}{0.08}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}\\
%         40\% &  \ms{-0.92}{0.06}&  \ms{\textbf{-1.00}}{0.00}&  \ms{-0.57}{0.23}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}\\
%         45\% &  \ms{-0.55}{0.12}&  \ms{-0.86}{0.08}&  \ms{-0.21}{0.31}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}\\
%         50\% &  \ms{-0.26}{0.00}&  \ms{-0.77}{0.15}&  \ms{-0.71}{0.08}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}\\
%         55\% &  \ms{0.02}{0.13}&  \ms{-0.89}{0.05}&  \ms{-0.67}{0.16} &  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}\\
        
%         60\% &  \ms{-0.12}{0.16}&  \ms{-0.95}{0.06}&  \ms{-0.63}{0.17}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}\\
%         65\% &  \ms{-0.24}{0.18}&  \ms{-0.98}{0.0.}&  \ms{-0.92}{0.08}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}\\
%         70\% &  \ms{-0.75}{0.05}&  \ms{-0.94}{0.06}&  \ms{-0.42}{0.33}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}\\
%         75\% &  \ms{-0.89}{0.03}&  \ms{-0.92}{0.07}&  \ms{-0.86}{0.16}&  \ms{-0.99}{0.02}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{-0.99}{0.02}\\
%         80\% &  \ms{-0.70}{0.19}&  \ms{-0.87}{0.09}&  \ms{-0.87}{0.11}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{-0.99}{0.02}&  \ms{\textbf{-1.00}}{0.00}\\
%         85\% &  \ms{-0.93}{0.06}&  \ms{-0.98}{0.03}&  \ms{-0.97}{0.03}&  \ms{-0.99}{0.02}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}\\
        
%         90\% &  \ms{-0.76}{0.22}&  \ms{-0.86}{0.12}&  \ms{-0.79}{0.11}&  \ms{\textbf{-1.00}}{0.00}&  \ms{-0.99}{0.02}&  \ms{\textbf{-1.00}}{0.00}&  \ms{\textbf{-1.00}}{0.00}\\
%         95\% &  \ms{0.69}{0.19}&  \ms{-0.75}{0.14}&  \ms{-0.57}{0.34} &  \ms{-0.98}{0.03}&  \ms{\textbf{-0.99}}{0.02}&  \ms{-0.95}{0.04}&  \ms{-0.87}{0.09}\\
%         \midrule   
%         Avg. Rank & 4.74 & 5.00 & 5.68 & 1.32 & \textbf{1.21} & 1.47 & 2.00\\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table*}



==> experiments/PAM/spearman_correlation_local.tex <==
\begin{table*}[h]
    \centering
        \caption{Local Spearman rank correlation results on PAM dataset. We report the total number of top-1 ranks at each sparsity between $5\%$ to $95\%$. The best performance is marked as bold. Other settings are the same as Table~\ref{tab:exp:pam:global:correlation}}
    \label{tab:exp:cfar:local:correlation_rank}
    \scalebox{0.75}{
     \begin{tabular}{cccccccccc}
        \toprule
        \multirow{2}{*}{Model} &
        \multirow{2}{*}{Top-1 Ranks } &
        \multicolumn{2}{c}{Fidelity} &
        \multicolumn{2}{c}{ROAR} &
        \multicolumn{2}{c}{R-Fidelity} & 
        \multicolumn{2}{c}{F-Fidelity} \\
        \cmidrule(r){3-4} \cmidrule(r){5-6} \cmidrule(r){7-8} \cmidrule(r){9-10} 
        & &  w/o  & w/  & w/o  & w/  & w/o  & w/  & w/o  & w/  \\
        % Model & Correlation & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
         \midrule   
        % & \multicolumn{4}{c}{Local Spearman Correlation $\downarrow$} \\ 
        % \hline
        \multirow{3}{*}{\rotatebox[origin=c]{90}{LSTM}}
        % \multirow{3}{\rotatebox[origin=c]{90}{Res.}} 
        & MoRF VS GT  & \\
        & LeRF VS GT & \\
        & MoRF VS LeRF & \\
        \hline
        \multirow{3}{*}{\rotatebox[origin=c]{90}{Trans.}}
        % \multirow{3}{\rotatebox[origin=c]{90}{ViT}}  \ms{\textbf{1.00}}{0.00}
        & MoRF VS GT  &  \\
        & LeRF VS GT  & \\
        & MoRF VS LeRF & \\
        \bottomrule
    \end{tabular}
    }
\end{table*}



==> experiments/PAM/transformer_correlation_detail.tex <==
\begin{table*}[h]
    \centering
        \caption{"MoRF VS GT" Local Spearman rank correlation results on PAM dataset with Transformer as the model to be explained.}
    \label{tab:exp:PAM:transformer:local:morf_rank}
    \scalebox{0.75}{
     \begin{tabular}{ccccccccc}
        \toprule
        &
        \multicolumn{2}{c}{Fidelity} &
        \multicolumn{1}{c}{ROAR} &
        \multicolumn{2}{c}{R-Fidelity} & 
        \multicolumn{2}{c}{F-Fidelity} \\
        \cmidrule(r){2-3} \cmidrule(r){4-4} \cmidrule(r){5-6} \cmidrule(r){7-8}
        Sparsity &  origin  & fine-tune & retrain & origin  & fine-tune  & origin  & fine-tune  \\
        % Model & Correlation & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
         \midrule   
        % & \multicolumn{4}{c}{Local Spearman Correlation $\downarrow$} \\ 
        % \hline
        % \multirow{3}{\rotatebox[origin=c]{90}{ViT}}  \ms{\textbf{1.00}}{0.00}
        $5\%$&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-0.98}{0.03}&  \ms{-1.00}{0.00}&  \ms{-0.98}{0.02}&  \ms{0.00}{0.00} \\
        10\% &  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-0.98}{0.03}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{0.00}{0.00}\\
        15\% &  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{0.00}{0.00}\\
        20\% &  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{0.00}{0.00}\\
        25\% &  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{0.00}{0.00}\\
        
        30\% &  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-0.99}{0.02}&  \ms{0.00}{0.00}\\
        35\% &  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-0.98}{0.03}&  \ms{0.00}{0.00}\\
        40\% &  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-0.93}{0.08}&  \ms{0.00}{0.00}\\
        45\% &  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-0.94}{0.06}&  \ms{0.00}{0.00}\\
        50\% &  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-0.92}{0.08}&  \ms{0.00}{0.00}\\
        55\% &  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-0.92}{0.08}&  \ms{0.00}{0.00}\\
        
        60\% &  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-0.92}{0.08}&  \ms{0.00}{0.00}\\
        65\% &  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-0.91}{0.08}&  \ms{0.00}{0.00}\\
        70\% &  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-0.99}{0.01}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-0.86}{0.08}&  \ms{0.00}{0.00}\\
        75\% &  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.01}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-0.84}{0.14}&  \ms{0.00}{0.00}\\
        80\% &  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-0.98}{0.02}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-0.79}{0.12}&  \ms{0.00}{0.00}\\
        85\% &  \ms{-1.00}{0.00}&  \ms{-1.00}{0.01}&  \ms{-0.95}{0.04}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-0.73}{0.16}&  \ms{0.00}{0.00}\\
        
        90\% &  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-0.94}{0.07}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-0.67}{0.12}&  \ms{0.00}{0.00}\\
        95\% &  \ms{-1.00}{0.00}&  \ms{-0.99}{0.02}&  \ms{-0.90}{0.13}&  \ms{-0.99}{0.02}&  \ms{-1.00}{0.00}&  \ms{-0.53}{0.13}&  \ms{0.00}{0.00}\\
        \midrule   
        Avg. Rank & \\
        \bottomrule
    \end{tabular}
    }
\end{table*}

\begin{table*}[h]
    \centering
        \caption{"LeRF VS GT" Local Spearman rank correlation results on PAM dataset with Transformer as the model to be explained.}
    \label{tab:exp:PAM:transformer:local:lerf_rank}
    \scalebox{0.75}{
     \begin{tabular}{ccccccccc}
        \toprule
        &
        \multicolumn{2}{c}{Fidelity} &
        \multicolumn{1}{c}{ROAR} &
        \multicolumn{2}{c}{R-Fidelity} & 
        \multicolumn{2}{c}{F-Fidelity} \\
        \cmidrule(r){2-3} \cmidrule(r){4-4} \cmidrule(r){5-6} \cmidrule(r){7-8}
        Sparsity &  origin  & fine-tune & retrain & origin  & fine-tune  & origin  & fine-tune  \\
        % Model & Correlation & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
         \midrule   
        % & \multicolumn{4}{c}{Local Spearman Correlation $\downarrow$} \\ 
        % \hline
        % \multirow{3}{\rotatebox[origin=c]{90}{ViT}}  \ms{\textbf{1.00}}{0.00}
        $5\%$&  \ms{1.00}{0.00}&  \ms{1.00}{0.00}&  \ms{1.00}{0.00}&  \ms{1.00}{0.00}&  \ms{0.98}{0.03}&  \ms{0.45}{0.36}&  \ms{0.00}{0.00} \\
        10\% &  \ms{1.00}{0.00}&  \ms{1.00}{0.00}&  \ms{1.00}{0.00}&  \ms{1.00}{0.00}&  \ms{0.99}{0.02}&  \ms{0.67}{0.25}&  \ms{0.00}{0.00}\\
        15\% &  \ms{1.00}{0.01}&  \ms{1.00}{0.00}&  \ms{1.00}{0.00}&  \ms{1.00}{0.00}&  \ms{0.94}{0.06}&  \ms{0.73}{0.27}&  \ms{0.00}{0.00}\\
        20\% &  \ms{0.96}{0.02}&  \ms{1.00}{0.00}&  \ms{1.00}{0.00}&  \ms{1.00}{0.00}&  \ms{0.98}{0.03}&  \ms{0.84}{0.11}&  \ms{0.00}{0.00}\\
        25\% &  \ms{0.95}{0.02}&  \ms{0.97}{0.03}&  \ms{1.00}{0.00}&  \ms{1.00}{0.00}&  \ms{0.95}{0.07}&  \ms{0.84}{0.13}&  \ms{0.00}{0.00}\\
        
        30\% &  \ms{0.95}{0.04}&  \ms{0.97}{0.04}&  \ms{1.00}{0.00}&  \ms{1.00}{0.00}&  \ms{0.95}{0.07}&  \ms{0.87}{0.09}&  \ms{0.00}{0.00}\\
        35\% &  \ms{0.95}{0.03}&  \ms{0.97}{0.03}&  \ms{1.00}{0.00}&  \ms{0.99}{0.02}&  \ms{0.95}{0.07}&  \ms{0.86}{0.11}&  \ms{0.00}{0.00}\\
        40\% &  \ms{0.96}{0.02}&  \ms{0.87}{0.07}&  \ms{1.00}{0.00}&  \ms{1.00}{0.01}&  \ms{0.95}{0.07}&  \ms{0.87}{0.12}&  \ms{0.00}{0.00}\\
        45\% &  \ms{0.94}{0.04}&  \ms{0.92}{0.04}&  \ms{1.00}{0.00}&  \ms{1.00}{0.00}&  \ms{0.95}{0.07}&  \ms{0.87}{0.12}&  \ms{0.00}{0.00}\\
        50\% &  \ms{0.93}{0.07}&  \ms{0.94}{0.04}&  \ms{1.00}{0.00}&  \ms{0.98}{0.03}&  \ms{0.98}{0.03}&  \ms{0.87}{0.09}&  \ms{0.00}{0.00}\\
        55\% &  \ms{0.90}{0.09}&  \ms{0.92}{0.03}&  \ms{1.00}{0.00}&  \ms{0.98}{0.03}&  \ms{0.97}{0.03}&  \ms{0.92}{0.07}&  \ms{0.00}{0.00}\\
        
        60\% &  \ms{0.91}{0.14}&  \ms{0.91}{0.02}&  \ms{1.00}{0.00}&  \ms{0.98}{0.03}&  \ms{0.94}{0.06}&  \ms{0.91}{0.08}&  \ms{0.00}{0.00}\\
        65\% &  \ms{0.94}{0.04}&  \ms{0.95}{0.03}&  \ms{1.00}{0.00}&  \ms{0.98}{0.03}&  \ms{0.98}{0.03}&  \ms{0.94}{0.05}&  \ms{0.00}{0.00}\\
        70\% &  \ms{0.96}{0.06}&  \ms{0.95}{0.05}&  \ms{1.00}{0.00}&  \ms{0.99}{0.02}&  \ms{0.98}{0.03}&  \ms{0.97}{0.03}&  \ms{0.00}{0.00}\\
        75\% &  \ms{0.93}{0.06}&  \ms{0.96}{0.03}&  \ms{0.98}{0.02}&  \ms{0.98}{0.03}&  \ms{0.99}{0.02}&  \ms{0.95}{0.06}&  \ms{0.00}{0.00}\\
        80\% &  \ms{0.84}{0.11}&  \ms{0.94}{0.03}&  \ms{1.00}{0.01}&  \ms{0.97}{0.03}&  \ms{0.98}{0.03}&  \ms{0.97}{0.03}&  \ms{0.00}{0.00}\\
        85\% &  \ms{0.76}{0.11}&  \ms{0.97}{0.03}&  \ms{0.94}{0.06}&  \ms{0.98}{0.03}&  \ms{0.95}{0.07}&  \ms{0.97}{0.05}&  \ms{0.00}{0.00}\\
        
        90\% &  \ms{0.74}{0.13}&  \ms{0.97}{0.03}&  \ms{0.87}{0.09}&  \ms{0.98}{0.03}&  \ms{0.98}{0.03}&  \ms{0.95}{0.04}&  \ms{0.00}{0.00}\\
        95\% &  \ms{0.92}{0.09}&  \ms{0.95}{0.04}&  \ms{0.78}{0.10}&  \ms{0.97}{0.03}&  \ms{0.98}{0.03}&  \ms{0.92}{0.09}&  \ms{0.00}{0.00}\\
        \midrule   
        Avg. Rank &\\
        \bottomrule
    \end{tabular}
    }
\end{table*}


\begin{table*}[h]
    \centering
        \caption{"MoRF VS LeRF" Local Spearman rank correlation results on PAM dataset with Transformer as the model to be explained.}
    \label{tab:exp:PAM:transformer:local:morf_lerf}
    \scalebox{0.75}{
     \begin{tabular}{ccccccccc}
        \toprule
        &
        \multicolumn{2}{c}{Fidelity} &
        \multicolumn{1}{c}{ROAR} &
        \multicolumn{2}{c}{R-Fidelity} & 
        \multicolumn{2}{c}{F-Fidelity} \\
        \cmidrule(r){2-3} \cmidrule(r){4-4} \cmidrule(r){5-6} \cmidrule(r){7-8}
        Sparsity &  origin  & fine-tune & retrain & origin  & fine-tune  & origin  & fine-tune  \\
        % Model & Correlation & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
         \midrule   
        % & \multicolumn{4}{c}{Local Spearman Correlation $\downarrow$} \\ 
        % \hline
        % \multirow{3}{\rotatebox[origin=c]{90}{ViT}}  \ms{\textbf{1.00}}{0.00}
        $5\%$&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-0.98}{0.03}&  \ms{-0.97}{0.03}&  \ms{-0.50}{0.36}&  \ms{-0.76}{0.29} \\
        10\% &  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-0.98}{0.03}&  \ms{-0.99}{0.02}&  \ms{-0.67}{0.25}&  \ms{-0.86}{0.06}\\
        15\% &  \ms{-1.00}{0.01}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-0.94}{0.06}&  \ms{-0.73}{0.27}&  \ms{-0.91}{0.07}\\
        20\% &  \ms{-0.96}{0.02}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-0.98}{0.02}&  \ms{-0.84}{0.11}&  \ms{-0.93}{0.08}\\
        25\% &  \ms{-0.95}{0.02}&  \ms{-0.97}{0.03}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-0.95}{0.07}&  \ms{-0.84}{0.13}&  \ms{-0.92}{0.08}\\
        
        30\% &  \ms{-0.95}{0.04}&  \ms{-0.97}{0.04}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-0.95}{0.07}&  \ms{-0.90}{0.08}&  \ms{-0.91}{0.08}\\
        35\% &  \ms{-0.95}{0.03}&  \ms{-0.97}{0.03}&  \ms{-1.00}{0.00}&  \ms{-0.99}{0.02}&  \ms{-0.95}{0.07}&  \ms{-0.90}{0.09}&  \ms{-0.87}{0.09}\\
        40\% &  \ms{-0.96}{0.00}&  \ms{-0.87}{0.07}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.01}&  \ms{-0.95}{0.07}&  \ms{-0.84}{0.13}&  \ms{-0.82}{0.14}\\
        45\% &  \ms{-0.94}{0.04}&  \ms{-0.92}{0.04}&  \ms{-1.00}{0.00}&  \ms{-1.00}{0.00}&  \ms{-0.95}{0.07}&  \ms{-0.90}{0.10}&  \ms{-0.83}{0.10}\\
        50\% &  \ms{-0.93}{0.07}&  \ms{-0.94}{0.04}&  \ms{-1.00}{0.00}&  \ms{-0.98}{0.03}&  \ms{-0.98}{0.03}&  \ms{-0.82}{0.12}&  \ms{-0.84}{0.10}\\
        55\% &  \ms{-0.90}{0.09}&  \ms{-0.92}{0.03}&  \ms{-1.00}{0.00}&  \ms{-0.98}{0.03}&  \ms{-0.97}{0.03}&  \ms{-0.86}{0.13}&  \ms{-0.66}{0.26}\\
        
        60\% &  \ms{-0.91}{0.14}&  \ms{-0.91}{0.02}&  \ms{-1.00}{0.00}&  \ms{-0.98}{0.03}&  \ms{-0.94}{0.06}&  \ms{-0.81}{0.13}&  \ms{-0.54}{0.24}\\
        65\% &  \ms{-0.94}{0.04}&  \ms{-0.95}{0.03}&  \ms{-1.00}{0.00}&  \ms{-0.98}{0.03}&  \ms{-0.98}{0.03}&  \ms{-0.87}{0.14}&  \ms{-0.63}{0.13}\\
        70\% &  \ms{-0.96}{0.06}&  \ms{-0.95}{0.05}&  \ms{-0.99}{0.01}&  \ms{-0.99}{0.02}&  \ms{-0.98}{0.03}&  \ms{-0.83}{0.15}&  \ms{-0.59}{0.12}\\
        75\% &  \ms{-0.93}{0.06}&  \ms{-0.96}{0.03}&  \ms{-0.98}{0.02}&  \ms{-0.98}{0.03}&  \ms{-0.99}{0.02}&  \ms{-0.81}{0.20}&  \ms{-0.59}{0.12}\\
        80\% &  \ms{-0.84}{0.11}&  \ms{-0.94}{0.03}&  \ms{-0.87}{0.02}&  \ms{-0.97}{0.03}&  \ms{-0.98}{0.03}&  \ms{-0.81}{0.22}&  \ms{-0.50}{0.07}\\
        85\% &  \ms{-0.76}{0.11}&  \ms{-0.96}{0.04}&  \ms{-0.90}{0.09}&  \ms{-0.98}{0.03}&  \ms{-0.95}{0.07}&  \ms{-0.69}{0.24}&  \ms{-0.44}{0.12}\\
        
        90\% &  \ms{-0.74}{0.13}&  \ms{-0.97}{0.03}&  \ms{-0.80}{0.10}&  \ms{-0.98}{0.03}&  \ms{-0.98}{0.03}&  \ms{-0.66}{0.23}&  \ms{-0.23}{0.22}\\
        95\% &  \ms{-0.92}{0.09}&  \ms{-0.94}{0.05}&  \ms{-0.70}{0.18}&  \ms{-0.95}{0.02}&  \ms{-0.98}{0.03}&  \ms{-0.54}{0.20}&  \ms{0.11}{0.27}\\
        \midrule   
        Avg. Rank & \\
        \bottomrule
    \end{tabular}
    }
\end{table*}



==> experiments/PAM/transformer_fid_images.tex <==
\begin{table*}[h]
    \centering
        \caption{Fidelity results on PAM dataset with Transformer as the model to be explained. }
    \label{tab:exp:pam:transformer:fid}
    \scalebox{1.0}{
     \begin{tabular}{ccccc}
        \toprule
         & \multicolumn{2}{c}{$Fid^+$} & \multicolumn{2}{c}{$Fid^-$} \\ 
        \cmidrule(r){2-3} \cmidrule(r){4-5}
        Methods &  origin  & fine-tune/retrain  & origin & fine-tune/retrain\\ 
        
        \midrule 
        \rotatebox[origin=c]{90}{Fidelity}
        &
        \begin{minipage}[b]{0.20\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/PAM/transformer/image_ori_transformer_split_ori_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.20\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/PAM/transformer/image_finetune_transformer-finetune_split_ori_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.20\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/PAM/transformer/image_ori_transformer_split_ori_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.20\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/PAM/transformer/image_finetune_transformer-finetune_split_ori_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        \\

        
        \rotatebox[origin=c]{90}{ROAR}
        &
        \begin{minipage}[b]{0.20\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/PAM/transformer/image_ori_transformer_split_ori_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.20\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/PAM/transformer/image_ori_transformer_split_roar_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.20\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/PAM/transformer/image_ori_transformer_split_ori_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.20\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/PAM/transformer/image_ori_transformer_split_ori_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        \\

        \rotatebox[origin=c]{90}{R-Fidelity}
        &
        \begin{minipage}[b]{0.20\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/PAM/transformer/image_ori_transformer_split_rfid_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.20\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/PAM/transformer/image_finetune_transformer-finetune_split_rfid_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.20\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/PAM/transformer/image_ori_transformer_split_rfid_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.20\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/PAM/transformer/image_finetune_transformer-finetune_split_rfid_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        \\

        \rotatebox[origin=c]{90}{F-Fidelity}
        &
        \begin{minipage}[b]{0.20\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/PAM/transformer/image_ori_transformer_split_ffid_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.20\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/PAM/transformer/image_finetune_transformer-finetune_split_ffid_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.20\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/PAM/transformer/image_ori_transformer_split_ffid_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.20\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/PAM/transformer/image_finetune_transformer-finetune_split_ffid_interv0.2_gradcam_leRF.png}}
	  \end{minipage} \\
        
        \bottomrule
        
    \end{tabular}
    }
\end{table*}


==> experiments/SST2/spearman_correlation.tex <==
\begin{table*}[h]
    \centering
        \caption{Spearman rank correlation and rank results on SST2 dataset with LSTM and Transformer. }
    \label{tab:exp:sst2:correlation}
    \scalebox{0.9}{
     \begin{tabular}{ccccc|ccc}
        \toprule
        \multirow{2}{*}{} &
        \multirow{2}{*}{Correlation} &
        \multicolumn{3}{c}{LSTM} &
        \multicolumn{3}{c}{Transformer} \\
        \cmidrule(r){3-5} \cmidrule(r){6-8}
        & & 
        Fidelity &
        R-Fidelity & 
        F-Fidelity & 
        Fidelity &
        R-Fidelity & 
        F-Fidelity\\
         \midrule   
        \multirow{3}{*}{\rotatebox[origin=c]{90}{\shortstack{Macro \\ Corr.}}}
        & MoRF vs GT $\downarrow$   & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00}  & \ms{-0.94}{0.00} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
        & LeRF vs GT $\uparrow$     & \ms{\textbf{1.00}}{0.00}   & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}   & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
        & MoRF vs LeRF $\downarrow$ & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00}  & \ms{-0.94}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00}\\
        \midrule
        \multirow{3}{*}{\rotatebox[origin=c]{90}{\shortstack{Micro \\ Corr.}}}
        & MoRF vs GT  $\downarrow$  & \ms{\textbf{-1.00}}{0.01} & \ms{\textbf{-1.00}}{0.01} & \ms{{-0.99}}{0.03} & \ms{-0.93}{0.07} & \ms{-0.97}{0.05} & \ms{\textbf{-1.00}}{0.01} \\
        & LeRF vs GT  $\uparrow$    & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{{1.00}}{0.01}  & \ms{0.98}{0.04} & \ms{\textbf{0.99}}{0.02} & \ms{\textbf{0.99}}{0.03}\\
        & MoRF vs LeRF $\downarrow$ & \ms{\textbf{-1.00}}{0.01} & \ms{\textbf{-1.00}}{0.01} & \ms{{-0.99}}{0.02} & \ms{-0.92}{0.09} & \ms{-0.97}{0.05} & \ms{\textbf{-0.99}}{0.02}\\
        \midrule
        \multirow{3}{*}{\rotatebox[origin=c]{90}{\shortstack{Micro \\ Rank}}}
        & MoRF vs GT $\downarrow$  & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} & \ms{{1.05}}{0.22}           & \ms{2.05}{0.89} & \ms{1.32}{0.46} & \ms{\textbf{1.05}}{0.22}\\
        & LeRF vs GT  $\downarrow$ & \ms{\textbf{1.05}}{0.22}     & \ms{\textbf{1.05}}{0.22} & \ms{\textbf{1.05}}{0.22}   & \ms{\textbf{1.16}}{0.49} & \ms{1.26}{0.55}  & \ms{\textbf{1.16}}{0.36}\\
        & MoRF vs LeRF $\downarrow$& \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{{1.11}}{0.31}         & \ms{2.05}{0.97}  & \ms{1.32}{0.46} & \ms{\textbf{1.11}}{0.45}\\
        \bottomrule
    \end{tabular}
    }
\end{table*}



==> experiments/ablation/ablation_figure_beta.tex <==
\begin{figure}[h]
 \centering
 \subfigure[Local Spearman Correlation]{\includegraphics[width=2.0in]{experiments/ablation/beta/image_finetune_size0.20_threshold_local_spearman_coeffe.png}\label{fig:ablation:sampling:local}}\hspace{0em}
 \subfigure[Global Spearman Correlation]{\includegraphics[width=2.0in]{experiments/ablation/beta/image_finetune_size0.20_threshold_global_spearman_coeffe.png}\label{fig:ablation:sampling:global}}
 \caption{Ablation study on hyperparameter $\beta$ in Eq.~\ref{eq:f-fid}, with $S=50, \alpha_1=\alpha_2=0.5$. We compared 5 settings on global Spearman correlation and 3 settings on local Spearman correlation.}
 \label{fig:ablation:beta}
\end{figure}


==> experiments/ablation/ablation_figure_sampling.tex <==
% \begin{figure}[htb]
%   \begin{minipage}[b]{.48\linewidth}
%   \centerline{\includegraphics[width=4cm]{experiments/ablation/image_finetune_size0.20_numsampling_local_spearman_coeffe.png}}
% %  \vspace{1.5cm}
%   \end{minipage}
% \hfill
%   \begin{minipage}[b]{0.48\linewidth}
%   \centerline{\includegraphics[width=4cm]{experiments/ablation/image_finetune_size0.20_numsampling_global_spearman_coeffe.png}}
% %  \vspace{1.5cm}
%   \end{minipage}
% \caption{Ablation study on sampling number $S$, }
% \label{fig:res}
% \end{figure}



\begin{figure}[h]
 \centering
 \subfigure[Local Spearman Correlation]{\includegraphics[width=2.0in]{experiments/ablation/sampling/image_finetune_size0.20_numsampling_local_spearman_coeffe.png}\label{fig:ablation:sampling:local}}\hspace{0em}
 \subfigure[Global Spearman Correlation]{\includegraphics[width=2.0in]{experiments/ablation/sampling/image_finetune_size0.20_numsampling_global_spearman_coeffe.png}\label{fig:ablation:sampling:global}}
 \caption{Ablation study on sampling number $S$, with $\beta=0.1, \alpha_1=\alpha_2=0.5$. We compared 9 settings on global Spearman correlation and 3 settings on local Spearman correlation.}
 \label{fig:ablation:sampling}
\end{figure}

==> experiments/ablation/modules.tex <==
\begin{table*}[h]
    \centering
    \caption{Ablation study on F-Fidelity. The results are based on LSTM architecture and IG explainer on dataset Boiler.}
    \label{tab:exp:ablation:modules}
    \scalebox{0.85}{
    \begin{tabular}{c|c|cccc}
        \toprule
        Metric & Type & Fidelity & W/o bound & W/o fine tune & F-Fidelity \\
        \midrule
        \multirow{2}{*}{MoRF vs GT $\downarrow$} & Macro & \ms{-0.98}{0.03} & \ms{-1.00}{0.00} & \ms{-1.00}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        & Micro & N/A & N/A & \ms{-0.79}{0.29} & \ms{\textbf{-0.80}}{0.25} \\
        \midrule
        \multirow{2}{*}{LeRF vs GT $\uparrow$} & Macro & \ms{0.22}{0.03} & \ms{0.65}{0.06} & \ms{0.78}{0.02} & \ms{\textbf{0.86}}{0.07} \\
        & Micro & N/A & N/A & \ms{0.76}{0.32} & \ms{\textbf{0.78}}{0.25} \\
        \midrule
        \multirow{2}{*}{MoRF vs LeRF $\downarrow$} & Macro & \ms{-0.27}{0.08} & \ms{-0.65}{0.06} & \ms{-0.78}{0.02} & \ms{\textbf{-0.86}}{0.07} \\
        & Micro & N/A & N/A & \ms{\textbf{-0.96}}{0.03} & \ms{-0.94}{0.04} \\
        \bottomrule
    \end{tabular}
    }
\end{table*}

==> experiments/ablation/table_beta.tex <==
\begin{table*}[h]
  \centering
    \caption{\rub{The accuracy comparison of the fine-tuned models in the colored-MNIST dataset.}}
  \label{exp:tab:ablation:beta:acc}
  \scalebox{1.00}{
  \begin{tabular}{ccccccc}
   \toprule
         &  & \multicolumn{6}{c}{Fine-tuned} \\
         \cmidrule(r){3-7}
         & original & 0.05 & 0.10 & 0.15 & 0.20 & 0.25   \\ %& 0.8  \\
    
    \midrule 
    
    Acc. & 0.8742 & 0.8770 & 0.8536 & 0.8444 & 0.8387 & 0.8353 \\ % &0.0915  \\
    
    \bottomrule
  \end{tabular}
}
\end{table*}

==> experiments/cifar100/gradcam/resnet_correlation_detail.tex <==

\begin{table*}[h]
    \centering
    \caption{Local Spearman rank correlation results on \cfar~dataset2 with ResNet as the model to be explained.}
    \label{tab:exp:cfar:resnet:local:combined}
    \scalebox{0.6}{
    \begin{tabular}{c|cccc|cccc|cccc}
        \toprule
        & \multicolumn{4}{c|}{MoRF vs GT} & \multicolumn{4}{c|}{LeRF vs GT} & \multicolumn{4}{c}{MoRF vs LeRF} \\
        Sparsity & Fidelity & ROAR & R-Fidelity & F-Fidelity & Fidelity & ROAR & R-Fidelity & F-Fidelity & Fidelity & ROAR & R-Fidelity & F-Fidelity \\
        \midrule
        $5\%$ & \ms{0.82}{0.02}  & \ms{1.00}{0.00} & \ms{\textbf{-0.07}}{0.07}& \ms{\textbf{-0.07}}{0.00} & \ms{\textbf{0.89}}{0.08} & \ms{0.88}{0.07} & \ms{-0.54}{0.34} & \ms{-0.20}{0.43} & \ms{0.85}{0.06}  & \ms{0.88}{0.07} & \ms{-0.02}{0.10} & \ms{\textbf{-0.07}}{0.06} \\
        $10\%$ & \ms{0.82}{0.02} & \ms{1.00}{0.00} & \ms{\textbf{-0.03}}{0.00}& \ms{\textbf{-0.03}}{0.00} & \ms{0.93}{0.06} & \ms{0.91}{0.06} & \ms{0.97}{0.03}  & \ms{\textbf{1.00}}{0.00}  & \ms{0.84}{0.07}  & \ms{0.91}{0.06} & \ms{\textbf{-0.03}}{0.00} & \ms{\textbf{-0.03}}{0.00} \\
        $15\%$ & \ms{0.73}{0.10} & \ms{0.97}{0.03} & \ms{\textbf{-0.03}}{0.00}& \ms{\textbf{-0.03}}{0.00} & \ms{0.97}{0.04} & \ms{0.98}{0.02} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{0.74}{0.14}  & \ms{0.97}{0.03} & \ms{\textbf{-0.03}}{0.00} & \ms{\textbf{-0.03}}{0.00} \\
        $20\%$ & \ms{0.72}{0.08} & \ms{0.94}{0.00} & \ms{0.26}{0.00} & \ms{\textbf{-0.07}}{0.00} & \ms{0.98}{0.02} & \ms{0.99}{0.01} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{0.70}{0.10}  & \ms{0.95}{0.02} & \ms{0.26}{0.00}  & \ms{\textbf{-0.07}}{0.07} \\
        $25\%$ & \ms{0.66}{0.09} & \ms{0.93}{0.02} & \ms{0.26}{0.00} & \ms{\textbf{0.25}}{0.00}  & \ms{0.97}{0.03} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{0.66}{0.08}  & \ms{0.93}{0.02} & \ms{0.26}{0.00}  & \ms{\textbf{-0.24}}{0.02} \\
        $30\%$ & \ms{0.65}{0.11} & \ms{0.84}{0.06} & \ms{0.20}{0.06} & \ms{\textbf{-0.61}}{0.00} & \ms{0.98}{0.02} & \ms{0.99}{0.01} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{0.63}{0.12}  & \ms{0.85}{0.06} & \ms{0.20}{0.06}  & \ms{\textbf{-0.61}}{0.02} \\
        $35\%$ & \ms{0.67}{0.08} & \ms{0.88}{0.04} & \ms{0.21}{0.07} & \ms{\textbf{-0.77}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{0.98}{0.02} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{0.67}{0.08}  & \ms{0.90}{0.04} & \ms{0.21}{0.07}  & \ms{\textbf{-0.77}}{0.06} \\
        $40\%$ & \ms{0.62}{0.11} & \ms{0.88}{0.05} & \ms{0.12}{0.09} & \ms{\textbf{-0.86}}{0.00} & \ms{0.98}{0.02} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{0.61}{0.12}  & \ms{0.87}{0.05} & \ms{0.12}{0.09}  & \ms{\textbf{-0.86}}{0.07} \\
        $45\%$ & \ms{0.73}{0.13} & \ms{0.87}{0.05} & \ms{0.09}{0.09} & \ms{\textbf{-0.95}}{0.00} & \ms{0.98}{0.02} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{0.79}{0.11}  & \ms{0.86}{0.05} & \ms{0.09}{0.09}  & \ms{\textbf{-0.95}}{0.02} \\
        $50\%$ & \ms{0.72}{0.12} & \ms{0.95}{0.09} & \ms{-0.06}{0.16}& \ms{\textbf{-0.96}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{0.72}{0.12}  & \ms{0.94}{0.09} & \ms{-0.06}{0.16} & \ms{\textbf{-0.96}}{0.03} \\
        $55\%$ & \ms{0.75}{0.12} & \ms{0.96}{0.02} & \ms{0.12}{0.09} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{0.75}{0.12}  & \ms{0.96}{0.02} & \ms{0.12}{0.09}  & \ms{\textbf{-1.00}}{0.00}\\
        $60\%$ & \ms{0.67}{0.16} & \ms{0.97}{0.03} & \ms{-0.06}{0.18}& \ms{\textbf{-0.97}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{0.67}{0.16}  & \ms{0.97}{0.03} & \ms{-0.06}{0.17} & \ms{\textbf{-0.97}}{0.03}\\
        $65\%$ & \ms{0.64}{0.18} & \ms{0.96}{0.03} & \ms{0.03}{0.24} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{0.64}{0.18}  & \ms{0.96}{0.03} & \ms{0.02}{0.23}  & \ms{\textbf{-1.00}}{0.00}\\
        $70\%$ & \ms{0.80}{0.19} & \ms{0.92}{0.03} & \ms{0.14}{0.07} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{0.80}{0.19}  & \ms{0.92}{0.03} & \ms{0.14}{0.07}  & \ms{\textbf{-1.00}}{0.00}\\
        $75\%$ & \ms{0.71}{0.15} & \ms{0.85}{0.15} & \ms{0.22}{0.21} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{0.71}{0.15}  & \ms{0.84}{0.15} & \ms{0.22}{0.21}  & \ms{\textbf{-1.00}}{0.00}\\
        $80\%$ & \ms{0.56}{0.24} & \ms{0.51}{0.25} & \ms{0.05}{0.28} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{0.56}{0.24}  & \ms{0.51}{0.25} & \ms{0.05}{0.27}  & \ms{\textbf{-1.00}}{0.00}\\
        $85\%$ & \ms{0.32}{0.24} & \ms{-0.01}{0.07}& \ms{0.17}{0.21} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{0.32}{0.24}  & \ms{-0.01}{0.07}& \ms{0.16}{0.21}  & \ms{\textbf{-1.00}}{0.00}\\
        $90\%$ & \ms{-0.38}{0.31}& \ms{-0.24}{0.14}& \ms{-0.20}{0.24}& \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{-0.38}{0.31} & \ms{-0.24}{0.14}& \ms{-0.20}{0.24} & \ms{\textbf{-1.00}}{0.00}\\
        $95\%$ & \ms{-0.46}{0.15} & \ms{0.21}{0.21} & \ms{0.43}{0.27} & \ms{\textbf{-0.93}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{-0.46}{0.15} & \ms{0.21}{0.20} & \ms{0.43}{0.27}  & \ms{\textbf{-0.93}}{0.07}\\
        \midrule
        Avg. Rank & 3.00 & 3.74 & 2.11 & \textbf{1.00} & 2.05 & 1.68 & 1.21 & \textbf{1.11} & 3.00 & 3.74 & 2.16 & \textbf{1.00} \\
        \bottomrule
    \end{tabular}
    }
\end{table*}



% \begin{table*}[h]
%     \centering
%     \caption{``MoRF VS GT'' Local Spearman rank correlation results on \cfar~dataset with ResNet as the model to be explained.}
%     \label{tab:exp:cfar:resnet:local:morf_rank}
%     \scalebox{0.75}{
%     \begin{tabular}{ccccc}
%         \toprule
%         Sparsity & Fidelity & ROAR & R-Fidelity & F-Fidelity \\
%         \midrule
%         $5\%$  & \ms{-0.95}{0.02} & \ms{-0.95}{0.02} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
%         $10\%$ & \ms{-0.82}{0.02} & \ms{-0.49}{0.06} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $15\%$ & \ms{-0.62}{0.03} & \ms{-0.19}{0.08} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $20\%$ & \ms{-0.59}{0.06} & \ms{-0.26}{0.04} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $25\%$ & \ms{-0.39}{0.14} & \ms{-0.45}{0.09} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $30\%$ & \ms{-0.32}{0.08} & \ms{-0.86}{0.07} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $35\%$ & \ms{-0.34}{0.07} & \ms{-0.92}{0.05} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $40\%$ & \ms{-0.07}{0.16} & \ms{-0.94}{0.00} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $45\%$ & \ms{-0.04}{0.12} & \ms{-0.85}{0.05} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $50\%$ & \ms{-0.13}{0.26} & \ms{-0.83}{0.00} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $55\%$ & \ms{-0.08}{0.18} & \ms{-0.68}{0.04} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $60\%$ & \ms{-0.04}{0.35} & \ms{-0.66}{0.00} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $65\%$ & \ms{-0.23}{0.15} & \ms{-0.44}{0.60} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $70\%$ & \ms{-0.53}{0.16} & \ms{-0.39}{0.20} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $75\%$ & \ms{-0.38}{0.10} & \ms{-0.35}{0.13} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $80\%$ & \ms{-0.46}{0.20} & \ms{-0.73}{0.14} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $85\%$ & \ms{0.26}{0.15}  & \ms{-0.67}{0.14} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $90\%$ & \ms{0.11}{0.20}  & \ms{0.04}{0.12}  & \ms{-0.98}{0.03}          & \ms{\textbf{-1.00}}{0.00} \\
%         $95\%$ & \ms{0.66}{0.10}  & \ms{0.37}{0.20}  & \ms{-0.97}{0.05}          & \ms{\textbf{-1.00}}{0.00} \\
%         \midrule
%         Avg. Rank & 6.63 & 6.00 & 1.21 & \textbf{1.00} \\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table*}

% \begin{table*}[h]
%     \centering
%     \caption{``LeRF VS GT'' Local Spearman rank correlation results on \cfar~dataset with ResNet as the model to be explained.}
%     \label{tab:exp:cfar:resnet:local:lerf_rank}
%     \scalebox{0.75}{
%     \begin{tabular}{ccccc}
%         \toprule
%         Sparsity & Fidelity & ROAR & R-Fidelity & F-Fidelity \\
%         \midrule
%         $5\%$  & \ms{0.89}{0.10} & \ms{0.86}{0.11} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $10\%$ & \ms{0.87}{0.11} & \ms{0.88}{0.02} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} \\
%         $15\%$ & \ms{0.87}{0.09} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} \\
%         $20\%$ & \ms{0.99}{0.03} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} \\
%         $25\%$ & \ms{0.99}{0.02} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} \\
%         $30\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} \\
%         $35\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} \\
%         $40\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} \\
%         $45\%$ & \ms{\textbf{1.00}}{0.00} & \ms{0.99}{0.02} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} \\
%         $50\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} \\
%         $55\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} \\
%         $60\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} \\
%         $65\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} \\
%         $70\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} \\
%         $75\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} \\
%         $80\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} \\
%         $85\%$ & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}   & \ms{\textbf{1.00}}{0.00} \\
%         $90\%$ & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}   & \ms{\textbf{1.00}}{0.00} \\
%         $95\%$ & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}   & \ms{\textbf{1.00}}{0.00} \\
%         \midrule
%         Avg. Rank & 2.37 & 1.84 & \textbf{1.00} & \textbf{1.00} \\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table*}



% \begin{table*}[h]
%     \centering
%     \caption{``MoRF VS LeRF'' Local Spearman rank correlation results on \cfar~dataset with ResNet as the model to be explained.}
%     \label{tab:exp:cfar:resnet:local:morf_lerf}
%     \scalebox{0.75}{
%     \begin{tabular}{ccccc}
%         \toprule
%         Sparsity & Fidelity & ROAR & R-Fidelity & F-Fidelity \\
%         \midrule
%         $5\%$  & \ms{-0.84}{0.08} & \ms{-0.76}{0.18} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
%         $10\%$ & \ms{-0.67}{0.12} & \ms{-0.50}{0.06} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $15\%$ & \ms{-0.49}{0.10} & \ms{-0.19}{0.08} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $20\%$ & \ms{-0.58}{0.06} & \ms{-0.26}{0.04} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $25\%$ & \ms{-0.36}{0.18} & \ms{-0.45}{0.09} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $30\%$ & \ms{-0.32}{0.08} & \ms{-0.86}{0.07} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $35\%$ & \ms{-0.34}{0.07} & \ms{-0.92}{0.05} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $40\%$ & \ms{-0.07}{0.16} & \ms{-0.94}{0.00} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $45\%$ & \ms{-0.04}{0.12} & \ms{-0.84}{0.06} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $50\%$ & \ms{-0.13}{0.26} & \ms{-0.83}{0.00} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $55\%$ & \ms{0.08}{0.18}  & \ms{-0.68}{0.04} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $60\%$ & \ms{-0.04}{0.35} & \ms{-0.66}{0.00} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $65\%$ & \ms{-0.23}{0.15} & \ms{-0.44}{0.06} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $70\%$ & \ms{-0.53}{0.16} & \ms{-0.39}{0.02} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $75\%$ & \ms{-0.38}{0.10} & \ms{-0.35}{0.13} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $80\%$ & \ms{-0.46}{0.20} & \ms{-0.73}{0.14} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $85\%$ & \ms{0.26}{0.15}  & \ms{-0.67}{0.14} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00}\\
%         $90\%$ & \ms{0.11}{0.20}  & \ms{0.05}{0.12}  & \ms{-0.98}{0.03}          & \ms{\textbf{-1.00}}{0.00} \\
%         $95\%$ & \ms{0.66}{0.10}  & \ms{0.37}{0.20}  & \ms{-0.97}{0.05}          & \ms{\textbf{-1.00}}{0.00} \\
%         \midrule
%         Avg. Rank & 6.58 & 6.05 & 1.21 & \textbf{1.00} \\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table*}


% \begin{table*}[h]
%     \centering
%         \caption{"MoRF VS GT" Local Spearman rank correlation results on \cfar~dataset with Resnet as the model to be explained. \ds{to be updated}}
%     \label{tab:exp:cfar:resnet:local:morf_rank}
%     \scalebox{0.75}{
%      \begin{tabular}{ccccccccc}
%         \toprule
%         &
%         \multicolumn{2}{c}{Fidelity} &
%         \multicolumn{1}{c}{ROAR} &
%         \multicolumn{2}{c}{R-Fidelity} & 
%         \multicolumn{2}{c}{F-Fidelity} \\
%         \cmidrule(r){2-3} \cmidrule(r){4-4} \cmidrule(r){5-6} \cmidrule(r){7-8} 
%         Sparsity &  origin  & fine-tune  & retrain  & origin  & fine-tune  & origin  & fine-tune \\
%         % Model & Correlation & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
%          \midrule   
%         % & \multicolumn{4}{c}{Local Spearman Correlation $\downarrow$} \\ 
%         % \hline
%         % \multirow{3}{\rotatebox[origin=c]{90}{ViT}}  \ms{\textbf{1.00}}{0.00}
%         $5\%$ &  \ms{-0.95}{0.02} &  \ms{-0.96}{0.02}&  \ms{-0.95}{0.02} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         10\% &  \ms{-0.82}{0.02} &  \ms{-0.78}{0.07} &  \ms{-0.49}{0.06} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         15\% &  \ms{-0.62}{0.03} &  \ms{-0.65}{0.02} &  \ms{-0.19}{0.08} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         20\% &  \ms{-0.59}{0.06} &  \ms{-0.60}{0.06} &  \ms{-0.26}{0.04} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         25\% &  \ms{-0.39}{0.14} &  \ms{-0.68}{0.10} &  \ms{-0.45}{0.09} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
        
%         30\% &  \ms{-0.32}{0.08} &  \ms{-0.49}{0.17} &  \ms{-0.86}{0.07} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         35\% &  \ms{-0.34}{0.07} &  \ms{-0.59}{0.06} &  \ms{-0.92}{0.05} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         40\% &  \ms{-0.07}{0.16} &  \ms{-0.52}{0.13} &  \ms{-0.94}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         45\% &  \ms{-0.04}{0.12} &  \ms{-0.66}{0.17} &  \ms{-0.85}{0.05} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         50\% &  \ms{-0.13}{0.26} &  \ms{-0.84}{0.08} &  \ms{-0.83}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         55\% &  \ms{-0.08}{0.18} &  \ms{-0.79}{0.06} &  \ms{-0.68}{0.04} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
        
%         60\% &  \ms{-0.04}{0.35} &  \ms{-0.72}{0.07} &  \ms{-0.66}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         65\% &  \ms{-0.23}{0.15} &  \ms{-0.90}{0.04} &  \ms{-0.44}{0.60} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         70\% &  \ms{-0.53}{0.16} &  \ms{-0.84}{0.07} &  \ms{-0.39}{0.2} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         75\% &  \ms{-0.38}{0.10} &  \ms{-0.53}{0.10} &  \ms{-0.35}{0.13} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         80\% &  \ms{-0.46}{0.20} &  \ms{-0.87}{0.12} &  \ms{-0.73}{0.14} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         85\% &  \ms{0.26}{0.15} &  \ms{-0.16}{0.14} &  \ms{-0.67}{0.14} &  \ms{\textbf{-1.00}}{0.00} &  \ms{-0.99}{0.02} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
        
%         90\% &  \ms{0.11}{0.20} &  \ms{-0.03}{0.09} &  \ms{0.04}{0.12} &  \ms{-0.98}{0.03} &  \ms{-0.98}{0.06} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         95\% &  \ms{0.66}{0.10} &  \ms{0.24}{0.29}  &  \ms{0.37}{0.20} &  \ms{-0.97}{0.05} &  \ms{-0.93}{0.09} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         \midrule   
%         Avg. Rank & 6.63 & 5.32 & 6.00 & 1.21 & 1.42 & \textbf{1.00} & \textbf{1.00}\\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table*}

% \begin{table*}[h]
%     \centering
%         \caption{"LeRF VS GT" Local Spearman rank correlation results on \cfar~dataset with Resnet as the model to be explained. \ds{to be updated}}
%     \label{tab:exp:cfar:resnet:local:lerf_rank}
%     \scalebox{0.75}{
%      \begin{tabular}{ccccccccc}
%         \toprule
%         &
%         \multicolumn{2}{c}{Fidelity} &
%         \multicolumn{1}{c}{ROAR} &
%         \multicolumn{2}{c}{R-Fidelity} & 
%         \multicolumn{2}{c}{F-Fidelity} \\
%         \cmidrule(r){2-3} \cmidrule(r){4-4} \cmidrule(r){5-6} \cmidrule(r){7-8} 
%         Sparsity &  origin  & fine-tune  & retrain  & origin  & fine-tune  & origin  & fine-tune \\
%         % Model & Correlation & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
%          \midrule   
%         % & \multicolumn{4}{c}{Local Spearman Correlation $\downarrow$} \\ 
%         % \hline
%         % \multirow{3}{\rotatebox[origin=c]{90}{ViT}}  \ms{\textbf{1.00}}{0.00}

%         $5\%$ &  \ms{0.89}{0.10} &  \ms{0.85}{0.11}&  \ms{0.86}{0.11} &  \ms{\textbf{1.00}}{0.00} &  \ms{0.99}{0.02} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         10\% &  \ms{0.87}{0.11} &  \ms{0.95}{0.04} &  \ms{0.88}{0.02} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         15\% &  \ms{0.87}{0.09} &  \ms{0.97}{0.03} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         20\% &  \ms{0.99}{0.03} &  \ms{0.95}{0.02} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         25\% &  \ms{0.99}{0.02} &  \ms{0.99}{0.02} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
        
%         30\% &  \ms{\textbf{1.00}}{0.00} &  \ms{0.99}{0.02} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         35\% &  \ms{\textbf{1.00}}{0.00} &  \ms{0.97}{0.03} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         40\% &  \ms{\textbf{1.00}}{0.00} &  \ms{0.98}{0.03} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         45\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{0.99}{0.02} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         50\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         55\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
        
%         60\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         65\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         70\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         75\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         80\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         85\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
        
%         90\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         95\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         \midrule   
%         Avg. Rank & 2.37 & 3.32 & 1.84 & \textbf{1.00} & 1.16 & \textbf{1.00} & \textbf{1.00}\\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table*}


% \begin{table*}[h]
%     \centering
%         \caption{"MoRF VS LeRF" Local Spearman rank correlation results on \cfar~dataset  with Resnet as the model to be explained.\ds{to be updated}}
%     \label{tab:exp:cfar:resnet:local:morf_lerf}
%     \scalebox{0.75}{
%      \begin{tabular}{ccccccccc}
%         \toprule
%         &
%         \multicolumn{2}{c}{Fidelity} &
%         \multicolumn{1}{c}{ROAR} &
%         \multicolumn{2}{c}{R-Fidelity} & 
%         \multicolumn{2}{c}{F-Fidelity} \\
%         \cmidrule(r){2-3} \cmidrule(r){4-4} \cmidrule(r){5-6} \cmidrule(r){7-8} 
%         Sparsity &  origin  & fine-tune  & retrain  & origin  & fine-tune  & origin  & fine-tune \\
%         % Model & Correlation & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
%          \midrule   
%         % & \multicolumn{4}{c}{Local Spearman Correlation $\downarrow$} \\ 
%         % \hline
%         % \multirow{3}{\rotatebox[origin=c]{90}{ViT}}  \ms{\textbf{1.00}}{0.00}

%         $5\%$ &  \ms{-0.84}{0.08}&  \ms{-0.83}{0.13} &  \ms{-0.76}{0.18} &  \ms{\textbf{-1.00}}{0.00} &  \ms{-0.99}{0.02} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         10\% &  \ms{-0.67}{0.12} &  \ms{-0.71}{0.10} &  \ms{-0.50}{0.06} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         15\% &  \ms{-0.49}{0.10} &  \ms{-0.61}{0.04} &  \ms{-0.19}{0.08} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         20\% &  \ms{-0.58}{0.06} &  \ms{-0.58}{0.08} &  \ms{-0.26}{0.04} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         25\% &  \ms{-0.36}{0.18} &  \ms{-0.65}{0.08} &  \ms{-0.45}{0.09} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
        
%         30\% &  \ms{-0.32}{0.08} &  \ms{-0.46}{0.19} &  \ms{-0.86}{0.07} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         35\% &  \ms{-0.34}{0.07} &  \ms{-0.56}{0.05} &  \ms{-0.92}{0.05} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         40\% &  \ms{-0.07}{0.16} &  \ms{-0.47}{0.11} &  \ms{-0.94}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         45\% &  \ms{-0.04}{0.12} &  \ms{-0.66}{0.17} &  \ms{-0.84}{0.06} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         50\% &  \ms{-0.13}{0.26} &  \ms{-0.84}{0.08} &  \ms{-0.83}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         55\% &  \ms{0.08}{0.18}  &  \ms{-0.79}{0.06} &  \ms{-0.68}{0.04} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
        
%         60\% &  \ms{-0.04}{0.35} &  \ms{-0.72}{0.07} &  \ms{-0.66}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         65\% &  \ms{-0.23}{0.15} &  \ms{-0.90}{0.04} &  \ms{-0.44}{0.06} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         70\% &  \ms{-0.53}{0.16} &  \ms{-0.84}{0.07} &  \ms{-0.39}{0.02} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         75\% &  \ms{-0.38}{0.10} &  \ms{-0.53}{0.10} &  \ms{-0.35}{0.13} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         80\% &  \ms{-0.46}{0.20} &  \ms{-0.87}{0.12} &  \ms{-0.73}{0.14} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         85\% &  \ms{0.26}{0.15}  &  \ms{-0.16}{0.14} &  \ms{-0.67}{0.14} &  \ms{\textbf{-1.00}}{0.00} &  \ms{-0.99}{0.02} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
        
%         90\% &  \ms{0.11}{0.20}  &  \ms{-0.03}{0.09} &  \ms{0.05}{0.12} &  \ms{-0.98}{0.03} &  \ms{-0.98}{0.05} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         95\% &  \ms{0.66}{0.10}  &  \ms{0.24}{0.29}  &  \ms{0.37}{0.20} &  \ms{-0.97}{0.05} &  \ms{-0.93}{0.09} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
        
%         \midrule   
%         Avg. Rank & 6.58 & 5.32 & 6.05 & 1.21 & 1.58 & \textbf{1.00} & \textbf{1.00}\\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table*}



==> experiments/cifar100/gradcam/resnet_fid_images.tex <==
\begin{table*}[h]
    \centering
        \caption{Fidelity results on \cfar~dataset2 with ResNet as the model to be explained.}
    \label{tab:exp:cfar:resnet:fid}
    \scalebox{1.0}{
     \begin{tabular}{ccccc}
        \toprule
        & Fidelity & ROAR & R-Fidelity & F-Fidelity \\
        \midrule
        $Fid^+$
        &
        \begin{minipage}[b]{0.20\columnwidth}
            \centering
            \vspace{2pt}
            \raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/gradcam/resnet/image_ori_resnet-9-explanations_ori_interv0.2_moRF.png}}
        \end{minipage}
        &
        \begin{minipage}[b]{0.20\columnwidth}
            \centering
            \vspace{2pt}
            \raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/gradcam/resnet/image_ori_resnet-9-explanations_roar_interv0.2_moRF.png}}
        \end{minipage}
        &
        \begin{minipage}[b]{0.20\columnwidth}
            \centering
            \vspace{2pt}
            \raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/gradcam/resnet/image_ori_resnet-9-explanations_rfid_interv0.2_moRF.png}}
        \end{minipage}
        &
        \begin{minipage}[b]{0.20\columnwidth}
            \centering
            \vspace{2pt}
            \raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/gradcam/resnet/image_finetune_resnet-9-finetune-explanations_ffid_interv0.2_moRF.png}}
        \end{minipage}
        \\

        $Fid^-$
        &
        \begin{minipage}[b]{0.20\columnwidth}
            \centering
            \vspace{2pt}
            \raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/gradcam/resnet/image_ori_resnet-9-explanations_ori_interv0.2_leRF.png}}
        \end{minipage}
        &
                \begin{minipage}[b]{0.20\columnwidth}
            \centering
            \vspace{2pt}
            \raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/gradcam/resnet/image_ori_resnet-9-explanations_roar_interv0.2_leRF.png}}
        \end{minipage}
        &
        \begin{minipage}[b]{0.20\columnwidth}
            \centering
            \vspace{2pt}
            \raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/gradcam/resnet/image_ori_resnet-9-explanations_rfid_interv0.2_leRF.png}}
        \end{minipage}
        &
        \begin{minipage}[b]{0.20\columnwidth}
            \centering
            \vspace{2pt}
            \raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/gradcam/resnet/image_finetune_resnet-9-finetune-explanations_ffid_interv0.2_leRF.png}}
        \end{minipage}
        \\
        \bottomrule
    \end{tabular}
    }
\end{table*}




% \begin{table*}[h]
%     \centering
%         \caption{Fidelity results on \cfar~dataset with Resnet as the model to be explained. }
%     \label{tab:exp:cfar:resnet:fid}
%     \scalebox{1.0}{
%      \begin{tabular}{ccccc}
%         \toprule
%          & \multicolumn{2}{c}{$Fid^+$} & \multicolumn{2}{c}{$Fid^-$} \\ 
%         \cmidrule(r){2-3} \cmidrule(r){4-5} 
%         Methods &  origin  & retrain/fine-tune  & origin & retrain/fine-tune\\ 
        
%         \midrule 
%         \rotatebox[origin=c]{90}{Fidelity}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/cifar100/resnet/image_ori_resnet-9-explanations_ori_interv0.2_gradcam_moRF.png}}
% 	  \end{minipage}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/cifar100/resnet/image_finetune_resnet-9-finetune-explanations_ori_interv0.2_gradcam_moRF.png}}
% 	  \end{minipage}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/cifar100/resnet/image_ori_resnet-9-explanations_ori_interv0.2_leRF.png}}
% 	  \end{minipage}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/cifar100/resnet/image_finetune_resnet-9-finetune-explanations_ori_interv0.2_leRF.png}}
% 	  \end{minipage}
%         \\

%         \rotatebox[origin=c]{90}{ROAR}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/cifar100/resnet/image_ori_resnet-9-explanations_ori_interv0.2_gradcam_moRF.png}}
% 	  \end{minipage}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/cifar100/resnet/image_ori_resnet-9-explanations_roar_interv0.2_gradcam_moRF.png}}
% 	  \end{minipage}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/cifar100/resnet/image_ori_resnet-9-explanations_ori_interv0.2_leRF.png}}
% 	  \end{minipage}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/cifar100/resnet/image_ori_resnet-9-explanations_roar_interv0.2_leRF.png}}
% 	  \end{minipage}
%         \\

        
%         \rotatebox[origin=c]{90}{R-Fidelity}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/cifar100/resnet/image_ori_resnet-9-explanations_rfid_interv0.2_gradcam_moRF.png}}
% 	  \end{minipage}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/cifar100/resnet/image_finetune_resnet-9-finetune-explanations_rfid_interv0.2_gradcam_moRF.png}}
% 	  \end{minipage}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/cifar100/resnet/image_ori_resnet-9-explanations_rfid_interv0.2_leRF.png}}
% 	  \end{minipage}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/cifar100/resnet/image_finetune_resnet-9-finetune-explanations_rfid_interv0.2_leRF.png}}
% 	  \end{minipage}
%         \\

%         \rotatebox[origin=c]{90}{F-Fidelity}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/cifar100/resnet/image_ori_resnet-9-explanations_ffid_interv0.2_gradcam_moRF.png}}
% 	  \end{minipage}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/cifar100/resnet/image_finetune_resnet-9-finetune-explanations_ffid_interv0.2_gradcam_moRF.png}}
% 	  \end{minipage}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/cifar100/resnet/image_ori_resnet-9-explanations_ffid_interv0.2_leRF.png}}
% 	  \end{minipage}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/cifar100/resnet/image_finetune_resnet-9-finetune-explanations_ffid_interv0.2_leRF.png}}
% 	  \end{minipage}
%         \\

        
%         \bottomrule
        
%     \end{tabular}
%     }
% \end{table*}


% \begin{figure}[h]
%   \centering
%     \subfigure[$\gamma=0.1,\alpha^+ = 0.3$]{\includegraphics[width=0.23\textwidth]{experiments/sparsity/finetune_size0.10_F-Fidelity_alpha0.30_MoRF.png} \hspace{-0.1em}\label{fig:exp:ablation:sparsity10_3}}
%     \subfigure[$\gamma = 0.15,\alpha^+ = 0.3$]{\includegraphics[width=0.23\textwidth]{experiments/sparsity/finetune_size0.15_F-Fidelity_alpha0.30_MoRF.png} \hspace{-0.1em}\label{fig:exp:ablation:sparsity15_3}}
%     \subfigure[$\gamma = 0.2, \alpha^+ = 0.3$]{\includegraphics[width=0.23\textwidth]{experiments/sparsity/finetune_size0.20_F-Fidelity_alpha0.30_MoRF.png} \hspace{-0.1em}\label{fig:exp:ablation:sparsity20_3}} 
%     \subfigure[$\gamma = 0.25, \alpha^+ = 0.3$]{\includegraphics[width=0.23\textwidth]{experiments/sparsity/finetune_size0.25_F-Fidelity_alpha0.30_MoRF.png} \hspace{-0.1em}\label{fig:exp:ablation:sparsity25_3}} \\
    
%     \subfigure[$\gamma=0.1,\alpha^+ = 0.5$]{\includegraphics[width=0.23\textwidth]{experiments/sparsity/finetune_size0.10_F-Fidelity_alpha0.50_MoRF.png} \hspace{-0.1em}\label{fig:exp:ablation:sparsity10_5}}
%     \subfigure[$\gamma = 0.15,\alpha^+ = 0.5$]{\includegraphics[width=0.23\textwidth]{experiments/sparsity/finetune_size0.15_F-Fidelity_alpha0.50_MoRF.png} \hspace{-0.1em}\label{fig:exp:ablation:sparsity15_5}}
%     \subfigure[$\gamma = 0.2, \alpha^+ = 0.5$]{\includegraphics[width=0.23\textwidth]{experiments/sparsity/finetune_size0.20_F-Fidelity_alpha0.50_MoRF.png} \hspace{-0.1em}\label{fig:exp:ablation:sparsity20_5}} 
%     \subfigure[$\gamma = 0.25, \alpha^+ = 0.5$]{\includegraphics[width=0.23\textwidth]{experiments/sparsity/finetune_size0.25_F-Fidelity_alpha0.50_MoRF.png} \hspace{-0.1em}\label{fig:exp:ablation:sparsity25_5}} \\

%     \subfigure[$\gamma=0.1,\alpha^+ = 0.7$]{\includegraphics[width=0.23\textwidth]{experiments/sparsity/finetune_size0.10_F-Fidelity_alpha0.70_MoRF.png} \hspace{-0.1em}\label{fig:exp:ablation:sparsity10_7}  }
%     \subfigure[$\gamma = 0.15,\alpha^+ = 0.7$]{\includegraphics[width=0.23\textwidth]{experiments/sparsity/finetune_size0.15_F-Fidelity_alpha0.70_MoRF.png} \hspace{-0.1em}\label{fig:exp:ablation:sparsity15_7}}
%     \subfigure[$\gamma = 0.2, \alpha^+ = 0.7$]{\includegraphics[width=0.23\textwidth]{experiments/sparsity/finetune_size0.20_F-Fidelity_alpha0.70_MoRF.png} \hspace{-0.1em}\label{fig:exp:ablation:sparsity20_7}} 
%     \subfigure[$\gamma = 0.25, \alpha^+ = 0.7$]{\includegraphics[width=0.23\textwidth]{experiments/sparsity/finetune_size0.25_F-Fidelity_alpha0.70_MoRF.png} \hspace{-0.1em}\label{fig:exp:ablation:sparsity25_7}} \\
    
    
%     \caption{The relationship between ground truth explanation size $\gamma$ and $RFid^+$ in \ffid. We compare different $\alpha^+$ and $\beta$ in the evaluation stage. We observe that the ground truth can be inferred from the $RFid^+$.}
%     \label{fig:exp:cfar:fid}
%         \vspace{-0.3cm}
% \end{figure}

==> experiments/cifar100/resnet_correlation_detail.tex <==

\begin{table*}[h]
    \centering
    \caption{Micro Spearman rank correlation results on \cfar~dataset with ResNet as the model to be explained.}
    \label{tab:exp:cfar:resnet:local:combined}
    \scalebox{0.6}{
    \begin{tabular}{c|cccc|cccc|cccc}
        \toprule
        & \multicolumn{4}{c|}{MoRF vs GT} & \multicolumn{4}{c|}{LeRF vs GT} & \multicolumn{4}{c}{MoRF vs LeRF} \\
        Sparsity & Fidelity & ROAR & R-Fidelity & F-Fidelity & Fidelity & ROAR & R-Fidelity & F-Fidelity & Fidelity & ROAR & R-Fidelity & F-Fidelity \\
        \midrule
        $5\%$  & \ms{-0.95}{0.02} & \ms{-0.95}{0.02} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{0.89}{0.10} & \ms{0.86}{0.11} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.84}{0.08} & \ms{-0.76}{0.18} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $10\%$ & \ms{-0.82}{0.02} & \ms{-0.49}{0.06} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{0.87}{0.11} & \ms{0.88}{0.02} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.67}{0.12} & \ms{-0.50}{0.06} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $15\%$ & \ms{-0.62}{0.03} & \ms{-0.19}{0.08} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{0.87}{0.09} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.49}{0.10} & \ms{-0.19}{0.08} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $20\%$ & \ms{-0.59}{0.06} & \ms{-0.26}{0.04} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{0.99}{0.03} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.58}{0.06} & \ms{-0.26}{0.04} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $25\%$ & \ms{-0.39}{0.14} & \ms{-0.45}{0.09} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{0.99}{0.02} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.36}{0.18} & \ms{-0.45}{0.09} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $30\%$ & \ms{-0.32}{0.08} & \ms{-0.86}{0.07} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.32}{0.08} & \ms{-0.86}{0.07} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $35\%$ & \ms{-0.34}{0.07} & \ms{-0.92}{0.05} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.34}{0.07} & \ms{-0.92}{0.05} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $40\%$ & \ms{-0.07}{0.16} & \ms{-0.94}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.07}{0.16} & \ms{-0.94}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $45\%$ & \ms{-0.04}{0.12} & \ms{-0.85}{0.05} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{0.99}{0.02} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.04}{0.12} & \ms{-0.84}{0.06} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $50\%$ & \ms{-0.13}{0.26} & \ms{-0.83}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.13}{0.26} & \ms{-0.83}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $55\%$ & \ms{-0.08}{0.18} & \ms{-0.68}{0.04} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{0.08}{0.18}  & \ms{-0.68}{0.04} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $60\%$ & \ms{-0.04}{0.35} & \ms{-0.66}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.04}{0.35} & \ms{-0.66}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $65\%$ & \ms{-0.23}{0.15} & \ms{-0.44}{0.06} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.23}{0.15} & \ms{-0.44}{0.06} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $70\%$ & \ms{-0.53}{0.16} & \ms{-0.39}{0.20} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.53}{0.16} & \ms{-0.39}{0.20} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $75\%$ & \ms{-0.38}{0.10} & \ms{-0.35}{0.13} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.38}{0.10} & \ms{-0.35}{0.13} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $80\%$ & \ms{-0.46}{0.20} & \ms{-0.73}{0.14} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.46}{0.20} & \ms{-0.73}{0.14} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $85\%$ & \ms{0.26}{0.15}  & \ms{-0.67}{0.14} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}   & \ms{\textbf{1.00}}{0.00} & \ms{0.26}{0.15}  & \ms{-0.67}{0.14} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00}\\
        $90\%$ & \ms{0.11}{0.20}  & \ms{0.04}{0.12}  & \ms{-0.98}{0.03}         & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}   & \ms{\textbf{1.00}}{0.00} & \ms{0.11}{0.20}  & \ms{0.05}{0.12}  & \ms{-0.98}{0.03}          & \ms{\textbf{-1.00}}{0.00} \\
        $95\%$ & \ms{0.66}{0.10}  & \ms{0.37}{0.20}  & \ms{-0.97}{0.05}         & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}   & \ms{\textbf{1.00}}{0.00} & \ms{0.66}{0.10}  & \ms{0.37}{0.20}  & \ms{-0.97}{0.05}          & \ms{\textbf{-1.00}}{0.00} \\
        \midrule
        Avg. Correlation &  \ms{-0.36}{0.37}  & \ms{-0.54}{0.35}  & \ms{\textbf{-1.00}}{0.01}   & \ms{\textbf{-1.00}}{0.00}  & 0.98 & 0.98 & 1.00 & 1.00 & -0.23 & -0.53 & -1.00 & -1.00  \\
        Avg. Rank & 2.79 & 2.37 & 1.11 & \textbf{1.00} & 1.32 & 1.21 & \textbf{1.00} & \textbf{1.00} & 2.79 & 2.42 & 1.11 & \textbf{1.00} \\
        \bottomrule
    \end{tabular}
    }
\end{table*}



% \begin{table*}[h]
%     \centering
%     \caption{``MoRF VS GT'' Local Spearman rank correlation results on \cfar~dataset with ResNet as the model to be explained.}
%     \label{tab:exp:cfar:resnet:local:morf_rank}
%     \scalebox{0.75}{
%     \begin{tabular}{ccccc}
%         \toprule
%         Sparsity & Fidelity & ROAR & R-Fidelity & F-Fidelity \\
%         \midrule
%         $5\%$  & \ms{-0.95}{0.02} & \ms{-0.95}{0.02} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
%         $10\%$ & \ms{-0.82}{0.02} & \ms{-0.49}{0.06} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $15\%$ & \ms{-0.62}{0.03} & \ms{-0.19}{0.08} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $20\%$ & \ms{-0.59}{0.06} & \ms{-0.26}{0.04} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $25\%$ & \ms{-0.39}{0.14} & \ms{-0.45}{0.09} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $30\%$ & \ms{-0.32}{0.08} & \ms{-0.86}{0.07} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $35\%$ & \ms{-0.34}{0.07} & \ms{-0.92}{0.05} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $40\%$ & \ms{-0.07}{0.16} & \ms{-0.94}{0.00} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $45\%$ & \ms{-0.04}{0.12} & \ms{-0.85}{0.05} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $50\%$ & \ms{-0.13}{0.26} & \ms{-0.83}{0.00} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $55\%$ & \ms{-0.08}{0.18} & \ms{-0.68}{0.04} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $60\%$ & \ms{-0.04}{0.35} & \ms{-0.66}{0.00} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $65\%$ & \ms{-0.23}{0.15} & \ms{-0.44}{0.60} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $70\%$ & \ms{-0.53}{0.16} & \ms{-0.39}{0.20} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $75\%$ & \ms{-0.38}{0.10} & \ms{-0.35}{0.13} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $80\%$ & \ms{-0.46}{0.20} & \ms{-0.73}{0.14} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $85\%$ & \ms{0.26}{0.15}  & \ms{-0.67}{0.14} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $90\%$ & \ms{0.11}{0.20}  & \ms{0.04}{0.12}  & \ms{-0.98}{0.03}          & \ms{\textbf{-1.00}}{0.00} \\
%         $95\%$ & \ms{0.66}{0.10}  & \ms{0.37}{0.20}  & \ms{-0.97}{0.05}          & \ms{\textbf{-1.00}}{0.00} \\
%         \midrule
%         Avg. Rank & 6.63 & 6.00 & 1.21 & \textbf{1.00} \\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table*}

% \begin{table*}[h]
%     \centering
%     \caption{``LeRF VS GT'' Local Spearman rank correlation results on \cfar~dataset with ResNet as the model to be explained.}
%     \label{tab:exp:cfar:resnet:local:lerf_rank}
%     \scalebox{0.75}{
%     \begin{tabular}{ccccc}
%         \toprule
%         Sparsity & Fidelity & ROAR & R-Fidelity & F-Fidelity \\
%         \midrule
%         $5\%$  & \ms{0.89}{0.10} & \ms{0.86}{0.11} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $10\%$ & \ms{0.87}{0.11} & \ms{0.88}{0.02} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} \\
%         $15\%$ & \ms{0.87}{0.09} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} \\
%         $20\%$ & \ms{0.99}{0.03} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} \\
%         $25\%$ & \ms{0.99}{0.02} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} \\
%         $30\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} \\
%         $35\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} \\
%         $40\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} \\
%         $45\%$ & \ms{\textbf{1.00}}{0.00} & \ms{0.99}{0.02} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} \\
%         $50\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} \\
%         $55\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} \\
%         $60\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} \\
%         $65\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} \\
%         $70\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} \\
%         $75\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} \\
%         $80\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} \\
%         $85\%$ & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}   & \ms{\textbf{1.00}}{0.00} \\
%         $90\%$ & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}   & \ms{\textbf{1.00}}{0.00} \\
%         $95\%$ & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}   & \ms{\textbf{1.00}}{0.00} \\
%         \midrule
%         Avg. Rank & 2.37 & 1.84 & \textbf{1.00} & \textbf{1.00} \\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table*}



% \begin{table*}[h]
%     \centering
%     \caption{``MoRF VS LeRF'' Local Spearman rank correlation results on \cfar~dataset with ResNet as the model to be explained.}
%     \label{tab:exp:cfar:resnet:local:morf_lerf}
%     \scalebox{0.75}{
%     \begin{tabular}{ccccc}
%         \toprule
%         Sparsity & Fidelity & ROAR & R-Fidelity & F-Fidelity \\
%         \midrule
%         $5\%$  & \ms{-0.84}{0.08} & \ms{-0.76}{0.18} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
%         $10\%$ & \ms{-0.67}{0.12} & \ms{-0.50}{0.06} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $15\%$ & \ms{-0.49}{0.10} & \ms{-0.19}{0.08} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $20\%$ & \ms{-0.58}{0.06} & \ms{-0.26}{0.04} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $25\%$ & \ms{-0.36}{0.18} & \ms{-0.45}{0.09} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $30\%$ & \ms{-0.32}{0.08} & \ms{-0.86}{0.07} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $35\%$ & \ms{-0.34}{0.07} & \ms{-0.92}{0.05} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $40\%$ & \ms{-0.07}{0.16} & \ms{-0.94}{0.00} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $45\%$ & \ms{-0.04}{0.12} & \ms{-0.84}{0.06} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $50\%$ & \ms{-0.13}{0.26} & \ms{-0.83}{0.00} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $55\%$ & \ms{0.08}{0.18}  & \ms{-0.68}{0.04} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $60\%$ & \ms{-0.04}{0.35} & \ms{-0.66}{0.00} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $65\%$ & \ms{-0.23}{0.15} & \ms{-0.44}{0.06} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $70\%$ & \ms{-0.53}{0.16} & \ms{-0.39}{0.02} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $75\%$ & \ms{-0.38}{0.10} & \ms{-0.35}{0.13} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $80\%$ & \ms{-0.46}{0.20} & \ms{-0.73}{0.14} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $85\%$ & \ms{0.26}{0.15}  & \ms{-0.67}{0.14} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00}\\
%         $90\%$ & \ms{0.11}{0.20}  & \ms{0.05}{0.12}  & \ms{-0.98}{0.03}          & \ms{\textbf{-1.00}}{0.00} \\
%         $95\%$ & \ms{0.66}{0.10}  & \ms{0.37}{0.20}  & \ms{-0.97}{0.05}          & \ms{\textbf{-1.00}}{0.00} \\
%         \midrule
%         Avg. Rank & 6.58 & 6.05 & 1.21 & \textbf{1.00} \\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table*}


% \begin{table*}[h]
%     \centering
%         \caption{"MoRF VS GT" Local Spearman rank correlation results on \cfar~dataset with Resnet as the model to be explained. \ds{to be updated}}
%     \label{tab:exp:cfar:resnet:local:morf_rank}
%     \scalebox{0.75}{
%      \begin{tabular}{ccccccccc}
%         \toprule
%         &
%         \multicolumn{2}{c}{Fidelity} &
%         \multicolumn{1}{c}{ROAR} &
%         \multicolumn{2}{c}{R-Fidelity} & 
%         \multicolumn{2}{c}{F-Fidelity} \\
%         \cmidrule(r){2-3} \cmidrule(r){4-4} \cmidrule(r){5-6} \cmidrule(r){7-8} 
%         Sparsity &  origin  & fine-tune  & retrain  & origin  & fine-tune  & origin  & fine-tune \\
%         % Model & Correlation & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
%          \midrule   
%         % & \multicolumn{4}{c}{Local Spearman Correlation $\downarrow$} \\ 
%         % \hline
%         % \multirow{3}{\rotatebox[origin=c]{90}{ViT}}  \ms{\textbf{1.00}}{0.00}
%         $5\%$ &  \ms{-0.95}{0.02} &  \ms{-0.96}{0.02}&  \ms{-0.95}{0.02} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         10\% &  \ms{-0.82}{0.02} &  \ms{-0.78}{0.07} &  \ms{-0.49}{0.06} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         15\% &  \ms{-0.62}{0.03} &  \ms{-0.65}{0.02} &  \ms{-0.19}{0.08} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         20\% &  \ms{-0.59}{0.06} &  \ms{-0.60}{0.06} &  \ms{-0.26}{0.04} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         25\% &  \ms{-0.39}{0.14} &  \ms{-0.68}{0.10} &  \ms{-0.45}{0.09} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
        
%         30\% &  \ms{-0.32}{0.08} &  \ms{-0.49}{0.17} &  \ms{-0.86}{0.07} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         35\% &  \ms{-0.34}{0.07} &  \ms{-0.59}{0.06} &  \ms{-0.92}{0.05} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         40\% &  \ms{-0.07}{0.16} &  \ms{-0.52}{0.13} &  \ms{-0.94}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         45\% &  \ms{-0.04}{0.12} &  \ms{-0.66}{0.17} &  \ms{-0.85}{0.05} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         50\% &  \ms{-0.13}{0.26} &  \ms{-0.84}{0.08} &  \ms{-0.83}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         55\% &  \ms{-0.08}{0.18} &  \ms{-0.79}{0.06} &  \ms{-0.68}{0.04} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
        
%         60\% &  \ms{-0.04}{0.35} &  \ms{-0.72}{0.07} &  \ms{-0.66}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         65\% &  \ms{-0.23}{0.15} &  \ms{-0.90}{0.04} &  \ms{-0.44}{0.60} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         70\% &  \ms{-0.53}{0.16} &  \ms{-0.84}{0.07} &  \ms{-0.39}{0.2} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         75\% &  \ms{-0.38}{0.10} &  \ms{-0.53}{0.10} &  \ms{-0.35}{0.13} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         80\% &  \ms{-0.46}{0.20} &  \ms{-0.87}{0.12} &  \ms{-0.73}{0.14} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         85\% &  \ms{0.26}{0.15} &  \ms{-0.16}{0.14} &  \ms{-0.67}{0.14} &  \ms{\textbf{-1.00}}{0.00} &  \ms{-0.99}{0.02} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
        
%         90\% &  \ms{0.11}{0.20} &  \ms{-0.03}{0.09} &  \ms{0.04}{0.12} &  \ms{-0.98}{0.03} &  \ms{-0.98}{0.06} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         95\% &  \ms{0.66}{0.10} &  \ms{0.24}{0.29}  &  \ms{0.37}{0.20} &  \ms{-0.97}{0.05} &  \ms{-0.93}{0.09} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         \midrule   
%         Avg. Rank & 6.63 & 5.32 & 6.00 & 1.21 & 1.42 & \textbf{1.00} & \textbf{1.00}\\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table*}

% \begin{table*}[h]
%     \centering
%         \caption{"LeRF VS GT" Local Spearman rank correlation results on \cfar~dataset with Resnet as the model to be explained. \ds{to be updated}}
%     \label{tab:exp:cfar:resnet:local:lerf_rank}
%     \scalebox{0.75}{
%      \begin{tabular}{ccccccccc}
%         \toprule
%         &
%         \multicolumn{2}{c}{Fidelity} &
%         \multicolumn{1}{c}{ROAR} &
%         \multicolumn{2}{c}{R-Fidelity} & 
%         \multicolumn{2}{c}{F-Fidelity} \\
%         \cmidrule(r){2-3} \cmidrule(r){4-4} \cmidrule(r){5-6} \cmidrule(r){7-8} 
%         Sparsity &  origin  & fine-tune  & retrain  & origin  & fine-tune  & origin  & fine-tune \\
%         % Model & Correlation & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
%          \midrule   
%         % & \multicolumn{4}{c}{Local Spearman Correlation $\downarrow$} \\ 
%         % \hline
%         % \multirow{3}{\rotatebox[origin=c]{90}{ViT}}  \ms{\textbf{1.00}}{0.00}

%         $5\%$ &  \ms{0.89}{0.10} &  \ms{0.85}{0.11}&  \ms{0.86}{0.11} &  \ms{\textbf{1.00}}{0.00} &  \ms{0.99}{0.02} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         10\% &  \ms{0.87}{0.11} &  \ms{0.95}{0.04} &  \ms{0.88}{0.02} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         15\% &  \ms{0.87}{0.09} &  \ms{0.97}{0.03} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         20\% &  \ms{0.99}{0.03} &  \ms{0.95}{0.02} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         25\% &  \ms{0.99}{0.02} &  \ms{0.99}{0.02} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
        
%         30\% &  \ms{\textbf{1.00}}{0.00} &  \ms{0.99}{0.02} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         35\% &  \ms{\textbf{1.00}}{0.00} &  \ms{0.97}{0.03} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         40\% &  \ms{\textbf{1.00}}{0.00} &  \ms{0.98}{0.03} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         45\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{0.99}{0.02} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         50\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         55\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
        
%         60\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         65\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         70\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         75\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         80\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         85\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
        
%         90\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         95\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         \midrule   
%         Avg. Rank & 2.37 & 3.32 & 1.84 & \textbf{1.00} & 1.16 & \textbf{1.00} & \textbf{1.00}\\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table*}


% \begin{table*}[h]
%     \centering
%         \caption{"MoRF VS LeRF" Local Spearman rank correlation results on \cfar~dataset  with Resnet as the model to be explained.\ds{to be updated}}
%     \label{tab:exp:cfar:resnet:local:morf_lerf}
%     \scalebox{0.75}{
%      \begin{tabular}{ccccccccc}
%         \toprule
%         &
%         \multicolumn{2}{c}{Fidelity} &
%         \multicolumn{1}{c}{ROAR} &
%         \multicolumn{2}{c}{R-Fidelity} & 
%         \multicolumn{2}{c}{F-Fidelity} \\
%         \cmidrule(r){2-3} \cmidrule(r){4-4} \cmidrule(r){5-6} \cmidrule(r){7-8} 
%         Sparsity &  origin  & fine-tune  & retrain  & origin  & fine-tune  & origin  & fine-tune \\
%         % Model & Correlation & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
%          \midrule   
%         % & \multicolumn{4}{c}{Local Spearman Correlation $\downarrow$} \\ 
%         % \hline
%         % \multirow{3}{\rotatebox[origin=c]{90}{ViT}}  \ms{\textbf{1.00}}{0.00}

%         $5\%$ &  \ms{-0.84}{0.08}&  \ms{-0.83}{0.13} &  \ms{-0.76}{0.18} &  \ms{\textbf{-1.00}}{0.00} &  \ms{-0.99}{0.02} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         10\% &  \ms{-0.67}{0.12} &  \ms{-0.71}{0.10} &  \ms{-0.50}{0.06} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         15\% &  \ms{-0.49}{0.10} &  \ms{-0.61}{0.04} &  \ms{-0.19}{0.08} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         20\% &  \ms{-0.58}{0.06} &  \ms{-0.58}{0.08} &  \ms{-0.26}{0.04} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         25\% &  \ms{-0.36}{0.18} &  \ms{-0.65}{0.08} &  \ms{-0.45}{0.09} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
        
%         30\% &  \ms{-0.32}{0.08} &  \ms{-0.46}{0.19} &  \ms{-0.86}{0.07} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         35\% &  \ms{-0.34}{0.07} &  \ms{-0.56}{0.05} &  \ms{-0.92}{0.05} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         40\% &  \ms{-0.07}{0.16} &  \ms{-0.47}{0.11} &  \ms{-0.94}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         45\% &  \ms{-0.04}{0.12} &  \ms{-0.66}{0.17} &  \ms{-0.84}{0.06} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         50\% &  \ms{-0.13}{0.26} &  \ms{-0.84}{0.08} &  \ms{-0.83}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         55\% &  \ms{0.08}{0.18}  &  \ms{-0.79}{0.06} &  \ms{-0.68}{0.04} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
        
%         60\% &  \ms{-0.04}{0.35} &  \ms{-0.72}{0.07} &  \ms{-0.66}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         65\% &  \ms{-0.23}{0.15} &  \ms{-0.90}{0.04} &  \ms{-0.44}{0.06} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         70\% &  \ms{-0.53}{0.16} &  \ms{-0.84}{0.07} &  \ms{-0.39}{0.02} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         75\% &  \ms{-0.38}{0.10} &  \ms{-0.53}{0.10} &  \ms{-0.35}{0.13} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         80\% &  \ms{-0.46}{0.20} &  \ms{-0.87}{0.12} &  \ms{-0.73}{0.14} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         85\% &  \ms{0.26}{0.15}  &  \ms{-0.16}{0.14} &  \ms{-0.67}{0.14} &  \ms{\textbf{-1.00}}{0.00} &  \ms{-0.99}{0.02} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
        
%         90\% &  \ms{0.11}{0.20}  &  \ms{-0.03}{0.09} &  \ms{0.05}{0.12} &  \ms{-0.98}{0.03} &  \ms{-0.98}{0.05} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         95\% &  \ms{0.66}{0.10}  &  \ms{0.24}{0.29}  &  \ms{0.37}{0.20} &  \ms{-0.97}{0.05} &  \ms{-0.93}{0.09} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
        
%         \midrule   
%         Avg. Rank & 6.58 & 5.32 & 6.05 & 1.21 & 1.58 & \textbf{1.00} & \textbf{1.00}\\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table*}



==> experiments/cifar100/resnet_shapley.tex <==
\begin{table*}[h]
    \centering
        \caption{\rub{Spearman rank correlation and rank results on \cfar~dataset with ResNet explained by SHAP.} }
    \label{tab:exp:cfar:shapley:resnet:correlation}
    \scalebox{0.90}{
     \begin{tabular}{cccccc}
        \toprule
         &
        {Correlation} & 
        Fidelity &
        ROAR &
        R-Fidelity & 
        F-Fidelity \\
         \midrule   
        \multirow{3}{*}{\rotatebox[origin=c]{90}{\shortstack{Macro \\ Corr.}}}
        & MoRF vs GT $\downarrow$   &  \ms{0.99}{0.02}  & \ms{0.93}{0.06}   &\ms{{-1.00}}{0.00} & \ms{{-1.00}}{0.00}   \\
        & LeRF vs GT $\uparrow$     & \ms{{-1.00}}{0.02} & \ms{{-0.34}}{0.15}   &\ms{{-1.00}}{0.00} & \ms{{-1.00}}{0.00} \\
        & MoRF vs LeRF $\downarrow$ & \ms{0.98}{0.00} & \ms{-0.23}{0.19}  &\ms{{1.00}}{0.00} & \ms{{1.00}}{0.00} \\
        \midrule
        \multirow{3}{*}{\rotatebox[origin=c]{90}{\shortstack{Micro \\ Corr.}}}
        & MoRF vs GT  $\downarrow$ &  \ms{0.53}{0.40}  & \ms{0.81}{0.20}  & \ms{{-0.02}}{0.22}   & \ms{{-0.81}}{0.38}   \\
        & LeRF vs GT  $\uparrow$    & \ms{0.99}{0.02}  & \ms{0.99}{0.04}  & \ms{\textbf{1.00}}{0.00}   & \ms{{1.00}}{0.00} \\
        & MoRF vs LeRF $\downarrow$ & \ms{0.53}{0.41}  & \ms{0.81}{0.20}  & \ms{{-0.02}}{0.22}   & \ms{{-0.81}}{0.38} \\
        \midrule
        \multirow{3}{*}{\rotatebox[origin=c]{90}{\shortstack{Micro \\ Rank}}}
        & MoRF vs GT $\downarrow$  & \ms{2.95}{0.23} & \ms{3.95}{0.23} & \ms{1.89}{0.66} & \ms{\textbf{1.21}}{0.42} \\
        & LeRF vs GT  $\downarrow$ & \ms{{2.53}}{1.39} & \ms{1.95}{1.18} & \ms{1.05}{0.23} & \ms{\textbf{1.00}}{0.00} \\
        & MoRF vs LeRF $\downarrow$& \ms{2.89}{0.32} & \ms{3.95}{0.23} & \ms{1.89}{0.56} & \ms{\textbf{1.21}}{0.42}\\
        \bottomrule
    \end{tabular}
    }
\end{table*}

==> experiments/cifar100/vit_correlation_detail.tex <==
\begin{table*}[h]
    \centering
    \caption{Micro Spearman rank correlation results on \cfar~dataset with ViT as the model to be explained.}
    \label{tab:exp:cfar:vit:local:combined}
    \scalebox{0.6}{
    \begin{tabular}{c|cccc|cccc|cccc}
        \toprule
        & \multicolumn{4}{c|}{MoRF vs GT} & \multicolumn{4}{c|}{LeRF vs GT} & \multicolumn{4}{c}{MoRF vs LeRF} \\
        Sparsity & Fidelity & ROAR & R-Fidelity & F-Fidelity & Fidelity & ROAR & R-Fidelity & F-Fidelity & Fidelity & ROAR & R-Fidelity & F-Fidelity \\
        \midrule
        $5\%$  & \ms{\textbf{-1.00}}{0.00} & \ms{-0.98}{0.03} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{0.98}{0.02} & \ms{0.08}{0.15} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.99}{0.00} & \ms{-0.05}{0.21} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $10\%$ & \ms{-0.91}{0.04}          & \ms{-0.85}{0.05} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{0.84}{0.06} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.91}{0.04} & \ms{-0.89}{0.07} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $15\%$ & \ms{-0.85}{0.05}          & \ms{-0.83}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{0.98}{0.03} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.81}{0.09} & \ms{-0.83}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $20\%$ & \ms{-0.73}{0.00}          & \ms{-0.87}{0.06} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{0.98}{0.03} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.79}{0.05} & \ms{-0.87}{0.06} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $25\%$ & \ms{-0.66}{0.00}          & \ms{-0.94}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.66}{0.00} & \ms{-0.94}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $30\%$ & \ms{-0.65}{0.03}          & \ms{-0.92}{0.05} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{0.99}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.66}{0.02} & \ms{-0.91}{0.05} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $35\%$ & \ms{-0.72}{0.08}          & \ms{-0.89}{0.05} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.72}{0.08} & \ms{-0.89}{0.05} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $40\%$ & \ms{-0.79}{0.07}          & \ms{-0.94}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.79}{0.07} & \ms{-0.94}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $45\%$ & \ms{-0.71}{0.08}          & \ms{-0.95}{0.02} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.71}{0.08} & \ms{-0.95}{0.02} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $50\%$ & \ms{-0.63}{0.03}          & \ms{-0.95}{0.02} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.63}{0.03} & \ms{-0.95}{0.02} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $55\%$ & \ms{-0.67}{0.08}          & \ms{-0.97}{0.03} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.69}{0.08} & \ms{-0.97}{0.03} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $60\%$ & \ms{-0.88}{0.07}          & \ms{-0.95}{0.02} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.88}{0.07} & \ms{-0.95}{0.02} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $65\%$ & \ms{-0.96}{0.03}          & \ms{-0.96}{0.02} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.96}{0.03} & \ms{-0.96}{0.02} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $70\%$ & \ms{-0.92}{0.08}          & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.92}{0.08} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $75\%$ & \ms{\textbf{-1.00}}{0.00} & \ms{-0.97}{0.03} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{-0.97}{0.03} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $80\%$ & \ms{-0.97}{0.03}          & \ms{-0.90}{0.06} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.97}{0.03} & \ms{-0.90}{0.06} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $85\%$ & \ms{-0.71}{0.10}          & \ms{-0.85}{0.05} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} & \ms{-0.71}{0.10} & \ms{-0.85}{0.05} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $90\%$ & \ms{0.74}{0.19}           & \ms{-0.71}{0.12} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} & \ms{0.74}{0.19}  & \ms{-0.71}{0.12} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
        $95\%$ & \ms{-0.06}{0.15}          & \ms{-0.87}{0.08} & \ms{-0.97}{0.46}          & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} & \ms{-0.06}{0.15} & \ms{0.87}{0.08}  & \ms{-0.97}{0.05}           & \ms{\textbf{-1.00}}{0.00} \\
        \midrule
        Avg. Correlation & -0.69 & -0.96 & \textbf{-1.00} & \textbf{-1.00} & \textbf{1.00} & 0.94 & \textbf{1.00} & \textbf{1.00}  & -0.69 & -0.77 & \textbf{-1.00} & \textbf{-1.00} \\
        Avg. Rank & 2.58 & 2.16 & 1.05 & \textbf{1.00} & 1.16 & 1.21 & \textbf{1.00} & \textbf{1.00} & 2.63 & 2.21 & 1.05 & \textbf{1.00} \\
        \bottomrule
    \end{tabular}
    }
\end{table*}


% \begin{table*}[h]
%     \centering
%     \caption{``MoRF VS GT'' Local Spearman rank correlation results on \cfar~dataset with ViT as the model to be explained.}
%     \label{tab:exp:cfar:vit:local:morf_rank}
%     \scalebox{0.75}{
%     \begin{tabular}{ccccc}
%         \toprule
%         Sparsity & Fidelity & ROAR & R-Fidelity & F-Fidelity \\
%         \midrule
%         $5\%$  & \ms{\textbf{-1.00}}{0.00} & \ms{-0.98}{0.03} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
%         $10\%$ & \ms{-0.91}{0.04}          & \ms{-0.85}{0.05} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
%         $15\%$ & \ms{-0.85}{0.05}          & \ms{-0.83}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
%         $20\%$ & \ms{-0.73}{0.00}          & \ms{-0.87}{0.06} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
%         $25\%$ & \ms{-0.66}{0.00}          & \ms{-0.94}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
%         $30\%$ & \ms{-0.65}{0.03}          & \ms{-0.92}{0.05} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
%         $35\%$ & \ms{-0.72}{0.08}          & \ms{-0.89}{0.05} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
%         $40\%$ & \ms{-0.79}{0.07}          & \ms{-0.94}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
%         $45\%$ & \ms{-0.71}{0.08}          & \ms{-0.95}{0.02} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
%         $50\%$ & \ms{-0.63}{0.03}          & \ms{-0.95}{0.02} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
%         $55\%$ & \ms{-0.67}{0.08}          & \ms{-0.97}{0.03} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
%         $60\%$ & \ms{-0.88}{0.07}          & \ms{-0.95}{0.02} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
%         $65\%$ & \ms{-0.96}{0.03}          & \ms{-0.96}{0.02} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
%         $70\%$ & \ms{-0.92}{0.08}          & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
%         $75\%$ & \ms{\textbf{-1.00}}{0.00} & \ms{-0.97}{0.03} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
%         $80\%$ & \ms{-0.97}{0.03}          & \ms{-0.90}{0.06} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
%         $85\%$ & \ms{-0.71}{0.10}          & \ms{-0.85}{0.05} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
%         $90\%$ & \ms{0.74}{0.19}           & \ms{-0.71}{0.12} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
%         $95\%$ & \ms{-0.06}{0.15}          & \ms{-0.87}{0.08} & \ms{-0.97}{0.46}          & \ms{\textbf{-1.00}}{0.00} \\
%         \midrule
%         Avg. Rank & 5.47 & 4.95 & 1.11 & \textbf{1.00} \\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table*}

% \begin{table*}[h]
%     \centering
%     \caption{``LeRF VS GT'' Local Spearman rank correlation results on \cfar~dataset with ViT as the model to be explained.}
%     \label{tab:exp:cfar:vit:local:lerf_rank}
%     \scalebox{0.75}{
%     \begin{tabular}{ccccc}
%         \toprule
%         Sparsity & Fidelity & ROAR & R-Fidelity & F-Fidelity \\
%         \midrule
%         $5\%$  & \ms{0.98}{0.02}       & \ms{0.08}{0.15}       & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $10\%$ & \ms{\textbf{1.00}}{0.00} & \ms{0.84}{0.06}       & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $15\%$ & \ms{0.98}{0.03}       & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $20\%$ & \ms{0.98}{0.03}       & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $25\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $30\%$ & \ms{\textbf{1.00}}{0.00} & \ms{0.99}{0.00}       & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $35\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $40\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $45\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $50\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $55\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $60\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $65\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $70\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $75\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $80\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $85\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $90\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $95\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         \midrule
%         Avg. Rank & 1.79 & 1.89 & \textbf{1.00} & \textbf{1.00} \\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table*}

% \begin{table*}[h]
%     \centering
%     \caption{"MoRF VS LeRF" Local Spearman rank correlation results on \cfar~dataset with ViT as the model to be explained.}
%     \label{tab:exp:cfar:vit:local:morf_lerf}
%     \scalebox{0.75}{
%     \begin{tabular}{ccccc}
%         \toprule
%         Sparsity & Fidelity & ROAR & R-Fidelity & F-Fidelity \\
%         \midrule
%         $5\%$  & \ms{-0.99}{0.00} & \ms{-0.05}{0.21} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
%         $10\%$ & \ms{-0.91}{0.04} & \ms{-0.89}{0.07} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $15\%$ & \ms{-0.81}{0.09} & \ms{-0.83}{0.00} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $20\%$ & \ms{-0.79}{0.05} & \ms{-0.87}{0.06} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $25\%$ & \ms{-0.66}{0.00} & \ms{-0.94}{0.00} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $30\%$ & \ms{-0.66}{0.02} & \ms{-0.91}{0.05} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $35\%$ & \ms{-0.72}{0.08} & \ms{-0.89}{0.05} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $40\%$ & \ms{-0.79}{0.07} & \ms{-0.94}{0.00} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $45\%$ & \ms{-0.71}{0.08} & \ms{-0.95}{0.02} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $50\%$ & \ms{-0.63}{0.03} & \ms{-0.95}{0.02} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $55\%$ & \ms{-0.69}{0.08} & \ms{-0.97}{0.03} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $60\%$ & \ms{-0.88}{0.07} & \ms{-0.95}{0.02} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $65\%$ & \ms{-0.96}{0.03} & \ms{-0.96}{0.02} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $70\%$ & \ms{-0.92}{0.08} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $75\%$ & \ms{\textbf{-1.00}}{0.00} & \ms{-0.97}{0.03} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $80\%$ & \ms{-0.97}{0.03} & \ms{-0.90}{0.06} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $85\%$ & \ms{-0.71}{0.10} & \ms{-0.85}{0.05} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $90\%$ & \ms{0.74}{0.19}  & \ms{-0.71}{0.12} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $95\%$ & \ms{-0.06}{0.15} & \ms{0.87}{0.08}  & \ms{-0.97}{0.05}          & \ms{\textbf{-1.00}}{0.00} \\
%         \midrule
%         Avg. Rank & 5.58 & 5.00 & 1.11 & \textbf{1.00} \\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table*}

% \begin{table*}[h]
%     \centering
%         \caption{"MoRF VS GT" Local Spearman rank correlation results on \cfar~dataset with ViT as the model to be explained.}
%     \label{tab:exp:cfar:vit:local:morf_rank}
%     \scalebox{0.75}{
%      \begin{tabular}{ccccccccc}
%         \toprule
%         &
%         \multicolumn{2}{c}{Fidelity} &
%         \multicolumn{1}{c}{ROAR} &
%         \multicolumn{2}{c}{R-Fidelity} & 
%         \multicolumn{2}{c}{F-Fidelity} \\
%         \cmidrule(r){2-3} \cmidrule(r){4-4} \cmidrule(r){5-6} \cmidrule(r){7-8} 
%         Sparsity &  origin  & fine-tune  & retrain  & origin  & fine-tune  & origin  & fine-tune \\
%         % Model & Correlation & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
%          \midrule   
%         % & \multicolumn{4}{c}{Local Spearman Correlation $\downarrow$} \\ 
%         % \hline
%         % \multirow{3}{\rotatebox[origin=c]{90}{ViT}}  \ms{\textbf{1.00}}{0.00}
%         $5\%$ &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00}&   \ms{-0.98}{0.03} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{-0.99}{0.02} &   \ms{\textbf{-1.00}}{0.00}  \\
%         10\% &   \ms{-0.91}{0.04} &   \ms{-0.85}{0.05} &   \ms{-0.85}{0.05} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{-0.69}{0.07} &   \ms{\textbf{-1.00}}{0.00}      \\
%         15\% &   \ms{-0.85}{0.05} &   \ms{-0.83}{0.00} &   \ms{-0.83}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{-0.60}{0.00} &   \ms{\textbf{-1.00}}{0.00}      \\
%         20\% &   \ms{-0.73}{0.00} &   \ms{-0.76}{0.09} &   \ms{-0.87}{0.06} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{-0.79}{0.03} &   \ms{\textbf{-1.00}}{0.00}     \\
%         25\% &   \ms{-0.66}{0.00} &   \ms{-0.89}{0.05} &   \ms{-0.94}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{-0.95}{0.07} &   \ms{\textbf{-1.00}}{0.00}     \\
        
%         30\% &   \ms{-0.65}{0.03} &   \ms{-0.89}{0.05} &   \ms{-0.92}{0.05} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00}     \\
%         35\% &   \ms{-0.72}{0.08} &   \ms{-0.73}{0.08} &   \ms{-0.89}{0.05} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00}     \\
%         40\% &   \ms{-0.79}{0.07} &   \ms{-0.78}{0.09} &   \ms{-0.94}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00}  \\
%         45\% &   \ms{-0.71}{0.08} &   \ms{-0.63}{0.03} &   \ms{-0.95}{0.02} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00}     \\
%         50\% &   \ms{-0.63}{0.03} &   \ms{-0.80}{0.03} &   \ms{-0.95}{0.02} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00}     \\
%         55\% &   \ms{-0.67}{0.08} &   \ms{-0.64}{0.02} &   \ms{-0.97}{0.03} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00}     \\
        
%         60\% &   \ms{-0.88}{0.07} &   \ms{-0.68}{0.08} &   \ms{-0.95}{0.02} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00}     \\
%         65\% &   \ms{-0.96}{0.03} &   \ms{-0.74}{0.08} &   \ms{-0.96}{0.02} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00}     \\
%         70\% &   \ms{-0.92}{0.08} &   \ms{-0.64}{0.10} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00}     \\
%         75\% &   \ms{\textbf{-1.00}}{0.00} &   \ms{-0.83}{0.00} &   \ms{-0.97}{0.03} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00}     \\
%         80\% &   \ms{-0.97}{0.03} &   \ms{-0.80}{0.04} &   \ms{-0.90}{0.06} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00}     \\
%         85\% &   \ms{-0.71}{0.10} &   \ms{-0.49}{0.15} &   \ms{-0.85}{0.05} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00}     \\
        
%         90\% &   \ms{0.74}{0.19} &   \ms{0.46}{0.27}   &   \ms{-0.71}{0.12} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00}     \\
%         95\% &   \ms{-0.06}{0.15} &   \ms{0.20}{0.21}  &   \ms{-0.87}{0.08} &   \ms{-0.97}{0.46} &   \ms{-0.99}{0.02} &   \ms{-0.93}{0.08} &   \ms{\textbf{-1.00}}{0.00}     \\
%         \midrule   
%         Avg. Rank & 5.47 & 6.16 & 4.95 & 1.11 & 1.05 & 2.42 & \textbf{1.00} \\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table*}

% \begin{table*}[h]
%     \centering
%         \caption{"LeRF VS GT" Local Spearman rank correlation results on \cfar~dataset with ViT as the model to be explained.}
%     \label{tab:exp:cfar:vit:local:lerf_rank}
%     \scalebox{0.75}{
%      \begin{tabular}{ccccccccc}
%         \toprule
%         &
%         \multicolumn{2}{c}{Fidelity} &
%         \multicolumn{1}{c}{ROAR} &
%         \multicolumn{2}{c}{R-Fidelity} & 
%         \multicolumn{2}{c}{F-Fidelity} \\
%         \cmidrule(r){2-3} \cmidrule(r){4-4} \cmidrule(r){5-6} \cmidrule(r){7-8} 
%         Sparsity &  origin  & fine-tune  & retrain  & origin  & fine-tune  & origin  & fine-tune \\
%         % Model & Correlation & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
%          \midrule   
%         % & \multicolumn{4}{c}{Local Spearman Correlation $\downarrow$} \\ 
%         % \hline
%         % \multirow{3}{\rotatebox[origin=c]{90}{ViT}}  \ms{\textbf{1.00}}{0.00}
%         $5\%$ &   \ms{0.98}{0.02} &   \ms{0.54}{0.18}&   \ms{0.08}{0.15} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00}  \\
%         10\% &   \ms{\textbf{1.00}}{0.00} &   \ms{0.78}{0.10} &   \ms{0.84}{0.06} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00}      \\
%         15\% &   \ms{0.98}{0.03} &   \ms{0.95}{0.06} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00}      \\
%         20\% &   \ms{0.98}{0.03} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00}     \\
%         25\% &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00}     \\
        
%         30\% &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{0.99}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00}     \\
%         35\% &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00}     \\
%         40\% &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00}  \\
%         45\% &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00}     \\
%         50\% &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00}     \\
%         55\% &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00}     \\
        
%         60\% &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00}     \\
%         65\% &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00}     \\
%         70\% &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00}     \\
%         75\% &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00}     \\
%         80\% &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00}     \\
%         85\% &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00}     \\
        
%         90\% &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00}     \\
%         95\% &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00} &   \ms{\textbf{1.00}}{0.00}     \\
%         \midrule   
%         Avg. Rank & 1.79 & 1.89 & 1.89 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00}\\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table*}


% \begin{table*}[h]
%     \centering
%         \caption{"MoRF VS LeRF" Local Spearman rank correlation results on \cfar~dataset with ViT as the model to be explained.}
%     \label{tab:exp:cfar:vit:local:morf_lerf}
%     \scalebox{0.75}{
%      \begin{tabular}{ccccccccc}
%         \toprule
%         &
%         \multicolumn{2}{c}{Fidelity} &
%         \multicolumn{1}{c}{ROAR} &
%         \multicolumn{2}{c}{R-Fidelity} & 
%         \multicolumn{2}{c}{F-Fidelity} \\
%         \cmidrule(r){2-3} \cmidrule(r){4-4} \cmidrule(r){5-6} \cmidrule(r){7-8} 
%         Sparsity &  origin  & fine-tune  & retrain  & origin  & fine-tune  & origin  & fine-tune \\
%         % Model & Correlation & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
%          \midrule   
%         % & \multicolumn{4}{c}{Local Spearman Correlation $\downarrow$} \\ 
%         % \hline
%         % \multirow{3}{\rotatebox[origin=c]{90}{ViT}}  \ms{\textbf{1.00}}{0.00}
%         $5\%$ &   \ms{-0.99}{0.00} &   \ms{-0.54}{0.18}&   \ms{-0.05}{0.21} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{-0.99}{0.02} &   \ms{\textbf{-1.00}}{0.00}  \\
%         10\% &   \ms{-0.91}{0.04} &   \ms{-0.69}{0.25} &   \ms{-0.89}{0.07} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{-0.69}{0.07} &   \ms{\textbf{-1.00}}{0.00}      \\
%         15\% &   \ms{-0.81}{0.09} &   \ms{-0.77}{0.08} &   \ms{-0.83}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{-0.60}{0.00} &   \ms{\textbf{-1.00}}{0.00}      \\
%         20\% &   \ms{-0.79}{0.05} &   \ms{-0.76}{0.08} &   \ms{-0.87}{0.06} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{-0.80}{0.03} &   \ms{\textbf{-1.00}}{0.00}     \\
%         25\% &   \ms{-0.66}{0.00} &   \ms{-0.89}{0.05} &   \ms{-0.94}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{-0.95}{0.07} &   \ms{\textbf{-1.00}}{0.00}     \\
        
%         30\% &   \ms{-0.66}{0.02} &   \ms{-0.89}{0.05} &   \ms{-0.91}{0.05} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00}     \\
%         35\% &   \ms{-0.72}{0.08} &   \ms{-0.73}{0.08} &   \ms{-0.89}{0.05} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00}     \\
%         40\% &   \ms{-0.79}{0.07} &   \ms{-0.78}{0.09} &   \ms{-0.94}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00}  \\
%         45\% &   \ms{-0.71}{0.08} &   \ms{-0.63}{0.03} &   \ms{-0.95}{0.02} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00}     \\
%         50\% &   \ms{-0.63}{0.03} &   \ms{-0.80}{0.03} &   \ms{-0.95}{0.02} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00}     \\
%         55\% &   \ms{-0.69}{0.08} &   \ms{-0.64}{0.02} &   \ms{-0.97}{0.03} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00}     \\
        
%         60\% &   \ms{-0.88}{0.07} &   \ms{-0.68}{0.08} &   \ms{-0.95}{0.02} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00}     \\
%         65\% &   \ms{-0.96}{0.03} &   \ms{-0.74}{0.08} &   \ms{-0.96}{0.02} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00}     \\
%         70\% &   \ms{-0.92}{0.08} &   \ms{-0.64}{0.10} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00}     \\
%         75\% &   \ms{\textbf{-1.00}}{0.00} &   \ms{-0.83}{0.00} &   \ms{-0.97}{0.03} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00}     \\
%         80\% &   \ms{-0.97}{0.03} &   \ms{-0.80}{0.4}  &   \ms{-0.90}{0.06} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00}     \\
%         85\% &   \ms{-0.71}{0.10} &   \ms{-0.49}{0.15} &   \ms{-0.85}{0.05} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00}     \\
        
%         90\% &   \ms{0.74}{0.19} &   \ms{0.46}{0.27}   &   \ms{-0.71}{0.12} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00} &   \ms{\textbf{-1.00}}{0.00}     \\
%         95\% &   \ms{-0.06}{0.15} &   \ms{0.20}{0.21}  &   \ms{0.87}{0.08} &   \ms{-0.97}{0.05} &   \ms{-0.99}{0.02} &   \ms{-0.93}{0.08} &   \ms{\textbf{-1.00}}{0.00}     \\
%         \midrule   
%         Avg. Rank & 5.58 & 6.53 & 5.00 & 1.11 & 1.05 & 2.26 & \textbf{1.00} \\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table*}



==> experiments/his/boolq-bert-ori.tex <==
\begin{table*}[h]
    \centering
        \caption{Rank Spearman correlation results on \sst~dataset with Bert as the model to be explained. The x-axis of the local correlation is the explanation size with hyperparameter top $k$. The global correlation means the rank Spearman correlation of average fidelity. The best performance is marked as bold. For R-Fidelity and F-Fidelity, $\alpha_1=\alpha_2=0.5$. In F-Fidelity, $\beta=0.1$. }
    \label{tab:exp:sst:bert}
    \scalebox{0.75}{
     \begin{tabular}{cccccccccc}
        \toprule
        \multirow{2}{*}{Model} &
        \multirow{2}{*}{Correlation} &
        \multicolumn{2}{c}{Fidelity} &
        \multicolumn{2}{c}{FIM} & 
        \multicolumn{2}{c}{R-Fidelity} & 
        \multicolumn{2}{c}{F-Fidelity} \\
        \cmidrule(r){3-4} \cmidrule(r){5-6} \cmidrule(r){7-8} \cmidrule(r){9-10}
        & &  w/o  & w/  & w/o  & w/  & w/o  & w/  & w/o  & w/ \\
        % Model & Correlation & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
         \midrule   
        % & \multicolumn{4}{c}{Local Spearman Correlation $\downarrow$} \\ 
        % \hline
        \multirow{3}{*}{\rotatebox[origin=c]{90}{Bert}}
        % \multirow{3}{\rotatebox[origin=c]{90}{Res.}} 
        & MoRF VS GT $\uparrow$ &  \ms{1.00}{0.00} &  \ms{1.00}{0.00} & & & \ms{1.00}{0.00} & \ms{1.00}{0.00} & \ms{1.00}{0.00} & \ms{1.00}{0.00} \\
        & LeRF VS GT $\downarrow$ & \ms{-0.95}{0.02} & \ms{-1.00}{0.00}  & & & \ms{-1.00}{0.00} & \ms{-1.00}{0.00} & \ms{1.00}{0.00} & \ms{1.00}{0.00} \\
        & MoRF VS LeRF $\downarrow$ &  \ms{-0.95}{0.02} &  \ms{-1.00}{0.00} & & & \ms{-1.00}{0.00} & \ms{-1.00}{0.00} & \ms{1.00}{0.00} & \ms{1.00}{0.00}\\
        \hline
        \multirow{3}{*}{\rotatebox[origin=c]{90}{GPT2}}
        % \multirow{3}{\rotatebox[origin=c]{90}{ViT}} 
        & MoRF VS GT $\uparrow$ &  \ms{0.94}{0.06}  &  \ms{0.97}{0.03}  & & & \ms{0.91}{0.09}  & \ms{0.97}{0.03} & \ms{0.89}{0.14} & \ms{0.98}{0.03} \\
        & LeRF VS GT $\downarrow$ &  \ms{-0.97}{0.03} &  \ms{-1.00}{0.00} & & & \ms{-0.92}{0.08} & \ms{-0.99}{0.02} & \ms{-0.95}{0.07} & \ms{-0.98}{0.05} \\
        & MoRF VS LeRF $\downarrow$&  \ms{-0.92}{0.08}   & \ms{-0.97}{0.03} & & & \ms{-0.89}{0.07} & \ms{-0.98}{0.03} & \ms{-0.90}{0.15} & \ms{-0.95}{0.04}\\
        
        % % \makecell*[c]{Global \\ Correlation $\downarrow$ } & \\
        % w/o fine-tune & $0.33\pm0.08$ & $0.94\pm0.06$ & $-0.33\pm0.06$ & $-\textbf{0.87}\pm0.06$ \\
        % w/ fine-tune & $-\textbf{1.00}\pm0.00$ & $-{0.68}\pm0.08$ & $-\textbf{1.00}\pm0.00$ & $-\textbf{1.00}\pm0.00$ \\

        
        % w/o fine-tune & $-0.82\pm0.02$ & $0.89\pm0.07$ & $-\textbf{1.00}\pm0.00$ & $-\textbf{1.00}\pm0.00$ \\
        % w/ fine-tune  & $-0.47\pm0.04$ & $0.83\pm0.00$ & $-\textbf{1.00}\pm0.00$ & $-\textbf{1.00}\pm0.00$ \\
        \bottomrule

        
    \end{tabular}
}    
\end{table*}


==> experiments/his/food101-resnet-finetune-fid.tex <==

% \begin{table*}[h]
%     \centering
%         \caption{Fidelity results on \food~dataset with finetuned Resnet-18 as the model to be explained. The x-axis of the local correlation is the explanation size with hyperparameter top $k$. The global correlation means the rank Spearman correlation of average fidelity. The best performance is marked as bold. For R-Fidelity and F-Fidelity, $\alpha_1=\alpha_2=0.5$. In F-Fidelity, $\beta=0.1$. }
%     \label{tab:exp:food:resnet-finetune:fid}
%     \scalebox{1.0}{
%      \begin{tabular}{ccccc}
%         \hline
%         Results  & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
%         \hline   
%         \makecell*[c]{$Fid^+$}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_finetune_model_ori_interv0.2_gradcam_moRF.png}}
% 	  \end{minipage}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_finetune_model_ori_interv0.2_gradcam_moRF.png}}
% 	  \end{minipage}
        
%         & 
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_finetune_model_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_moRF.png}}
% 	  \end{minipage}

%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_finetune_model_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_moRF.png}}
% 	  \end{minipage}        \\

%         \makecell*[c]{$Fid^-$ }
%          &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_finetune_model_ori_interv0.2_gradcam_leRF.png}}
% 	  \end{minipage}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_finetune_model_ori_interv0.2_gradcam_leRF.png}}
% 	  \end{minipage}
        
%         & 
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_finetune_model_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_leRF.png}}
% 	  \end{minipage}

%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_finetune_model_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_leRF.png}}
% 	  \end{minipage}        \\
            
%          \hline
        
%     \end{tabular}
%     }
% \end{table*}

\begin{table*}[h]
    \centering
        \caption{Fidelity results on \food~dataset with finetuned Resnet-18 as the model to be explained. The x-axis of the local correlation is the explanation size with hyperparameter top $k$. The global correlation means the rank Spearman correlation of average fidelity. The best performance is marked as bold. For R-Fidelity and F-Fidelity, $\alpha_1=\alpha_2=0.5$. In F-Fidelity, $\beta=0.1$.}
        % The global correlation means the rank Spearman correlation of average fidelity. The best performance is marked as bold. 
    \label{tab:exp:food:resnet-finetune:fid}
    \scalebox{1.0}{
     \begin{tabular}{ccccc}
        \hline
        Method  & {$Fid^+$}  & {$Fid^-$ } & \makecell*[c]{Local Spearman \\ Correlation }  \\ %R-Fidelity  &  {F-Fidelity} \\
        \hline   
        % \makecell*[c]{$Fid^+$}
        Fidelity &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_finetune_model_ori_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_finetune_model_ori_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        
        & 
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_finetune_model_ori_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage} \\

        % \makecell*[c]{$Fid^-$ }
         ROAD &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_finetune_model_road_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_finetune_model_road_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        & 
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_finetune_model_road_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage} \\

        
         R-Fidelity &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_finetune_model_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_finetune_model_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        & 
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_finetune_model_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage} \\

         F-Fidelity &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_finetune_model_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_finetune_model_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        & 
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_finetune_model_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage} \\
            
         \hline
        
    \end{tabular}
    }
\end{table*}



==> experiments/his/food101-resnet-finetune.tex <==
\begin{table*}[h]
    \centering
        \caption{Rank Spearman correlation results on \food~dataset with finetuned Resnet-18 as the model to be explained. The x-axis of the local correlation is the explanation size with hyperparameter top $k$. The global correlation means the rank Spearman correlation of average fidelity. The best performance is marked as bold. For R-Fidelity and F-Fidelity, $\alpha_1=\alpha_2=0.5$. In F-Fidelity, $\beta=0.1$.}
    \label{tab:exp:food:resnet-finetune}
    \scalebox{1.0}{
     \begin{tabular}{ccccc}
        \hline
        Results  & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
        \hline   
        \makecell*[c]{Local \\ Correlation $\downarrow$ }
        &
        \begin{minipage}[b]{0.18\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_finetune_model_ori_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.18\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_finetune_model_ori_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage}
        
        & 
        \begin{minipage}[b]{0.18\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_finetune_model_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage}

        &
        \begin{minipage}[b]{0.18\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_finetune_model_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage}        \\

        \makecell*[c]{Global \\ Correlation $\downarrow$ }
         & ${0.61}\pm0.02$ & Placeholder & ${0.28}\pm0.05$ & $\textbf{-0.26}\pm0.00$ \\
        \hline

        
    \end{tabular}
    }
\end{table*}

==> experiments/his/food101-resnet-ori-fid.tex <==

% \begin{table*}[h]
%     \centering
%         \caption{Fidelity results on \food~dataset with Resnet-18 as the model to be explained. The x-axis of the local correlation is the explanation size with hyperparameter top $k$. The global correlation means the rank Spearman correlation of average fidelity. The best performance is marked as bold. For R-Fidelity and F-Fidelity, $\alpha_1=\alpha_2=0.5$. In F-Fidelity, $\beta=0.1$. }
%     \label{tab:exp:food:resnet:fid}
%     \scalebox{1.0}{
%      \begin{tabular}{ccccc}
%         \hline
%         Results  & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
%         \hline   
%         \makecell*[c]{$Fid^+$}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_model_ori_interv0.2_gradcam_moRF.png}}
% 	  \end{minipage}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_model_ori_interv0.2_gradcam_moRF.png}}
% 	  \end{minipage}
        
%         & 
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_model_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_moRF.png}}
% 	  \end{minipage}

%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_model_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_moRF.png}}
% 	  \end{minipage}        \\

%         \makecell*[c]{$Fid^-$ }
%          &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_model_ori_interv0.2_gradcam_leRF.png}}
% 	  \end{minipage}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_model_ori_interv0.2_gradcam_leRF.png}}
% 	  \end{minipage}
        
%         & 
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_model_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_leRF.png}}
% 	  \end{minipage}

%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_model_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_leRF.png}}
% 	  \end{minipage}        \\
            
%          \hline
        
%     \end{tabular}
%     }
% \end{table*}


\begin{table*}[h]
    \centering
        \caption{Fidelity results on \food~dataset with Resnet-18 as the model to be explained. The x-axis of the local correlation is the explanation size with hyperparameter top $k$. The global correlation means the rank Spearman correlation of average fidelity. The best performance is marked as bold. For R-Fidelity and F-Fidelity, $\alpha_1=\alpha_2=0.5$. In F-Fidelity, $\beta=0.1$.}
        % The global correlation means the rank Spearman correlation of average fidelity. The best performance is marked as bold. 
    \label{tab:exp:food:resnet:fid}
    \scalebox{1.0}{
     \begin{tabular}{ccccc}
        \hline
        Method  & {$Fid^+$}  & {$Fid^-$ } & \makecell*[c]{Local Spearman \\ Correlation }  \\ %R-Fidelity  &  {F-Fidelity} \\
        \hline   
        % \makecell*[c]{$Fid^+$}
        Fidelity &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_model_ori_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_model_ori_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        
        & 
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_model_ori_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage} \\

        % \makecell*[c]{$Fid^-$ }
         ROAD &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_model_road_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_model_road_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        & 
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_model_road_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage} \\

        
         R-Fidelity &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_model_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_model_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        & 
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_model_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage} \\

         F-Fidelity &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_model_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_model_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        & 
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_model_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage} \\
            
         \hline
        
    \end{tabular}
    }
\end{table*}




==> experiments/his/food101-resnet-ori.tex <==
% \begin{table*}[h]
%     \centering
%     \caption{Rank Spearman correlation results on \food ~dataset with Resnet-18 as the model to be explained. The x-axis of the local correlation is the explanation size with hyperparameter top $k$. The global correlation means the rank Spearman correlation of average fidelity. The best performance is marked as bold. For R-Fidelity and F-Fidelity, $\alpha_1=\alpha_2=0.5$. In F-Fidelity, $\beta=0.1$. }
%     \label{tab:exp:food:resnet}
%     \scalebox{1.0}{
%     \begin{tabular}{ccccc}
%         \hline
%         Results  & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
%         \hline   
%         \makecell*[c]{Local \\ Correlation $\downarrow$ }
%         &
%         \begin{minipage}[b]{0.18\columnwidth}
%             \centering
%             \includegraphics[width=\linewidth]{experiments/food101/image_ori_model_ori_interv0.2_gradcam_SpearmanCoeff.png}
%         \end{minipage}
%         &
%         \begin{minipage}[b]{0.18\columnwidth}
%             \centering
%             \includegraphics[width=\linewidth]{experiments/food101/image_ori_model_ori_interv0.2_gradcam_SpearmanCoeff.png}
%         \end{minipage}
%         & 
%         \begin{minipage}[b]{0.18\columnwidth}
%             \centering
%             \includegraphics[width=\linewidth]{experiments/food101/image_ori_model_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_SpearmanCoeff.png}
%         \end{minipage}
%         &
%         \begin{minipage}[b]{0.18\columnwidth}
%             \centering
%             \includegraphics[width=\linewidth]{experiments/food101/image_ori_model_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_SpearmanCoeff.png}
%         \end{minipage} \\
%         \makecell*[c]{Global \\ Correlation $\downarrow$ }
%         & $0.90\pm0.06$ & Placeholder & $0.65\pm0.00$ & $\textbf{0.26}\pm0.00$ \\
%         \hline
%     \end{tabular}
%     }
% \end{table*}
% \begin{table*}[h]
%     \centering
%     \caption{Rank Spearman correlation results on \food ~dataset with Resnet-18 as the model to be explained. The x-axis of the local correlation is the explanation size with hyperparameter top $k$. The global correlation means the rank Spearman correlation of average fidelity. The best performance is marked as bold. For R-Fidelity and F-Fidelity, $\alpha_1=\alpha_2=0.5$. In F-Fidelity, $\beta=0.1$. }
%     \label{tab:exp:food:resnet}
%     \scalebox{1.0}{
%      \begin{tabular}{ccccc}
%         \hline
%         Results  & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
%         \hline   
%         \makecell*[c]{Local \\ Correlation $\downarrow$ }
%         &
%         \begin{minipage}[b]{0.18\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_model_ori_interv0.2_gradcam_SpearmanCoeff.png}}
% 	  \end{minipage}
%         &
%         \begin{minipage}[b]{0.18\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_model_ori_interv0.2_gradcam_SpearmanCoeff.png}}
% 	  \end{minipage}
        
%         & 
%         \begin{minipage}[b]{0.18\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_model_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_SpearmanCoeff.png}}
% 	  \end{minipage}

%         &
%         \begin{minipage}[b]{0.18\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_model_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_SpearmanCoeff.png}}
% 	  \end{minipage}        \\

%         \makecell*[c]{Global \\ Correlation $\downarrow$ }
%          & $0.90\pm0.06$ & Placeholder & $0.65\pm0.00$ & $\textbf{0.26}\pm0.00$ \\
%         \hline

        
%     \end{tabular}
%     }
% \end{table*}

\begin{table*}[h]
    \centering
        \caption{Global Spearman rank correlation results on \food~dataset which compares the average fidelity of different explanation size between $5\%$ to $95\%$. The best performance is marked as bold. For R-Fidelity and F-Fidelity, $\alpha_1=\alpha_2=0.5$. In F-Fidelity, $\beta=0.1$. }
    \label{tab:exp:food:resnet}
    \scalebox{0.75}{
     \begin{tabular}{cccccccccc}
        \toprule
        \multirow{2}{*}{Model} &
        \multirow{2}{*}{Correlation} &
        \multicolumn{2}{c}{Fidelity} &
        \multicolumn{2}{c}{ROAD} & 
        \multicolumn{2}{c}{R-Fidelity} & 
        \multicolumn{2}{c}{F-Fidelity} \\
        \cmidrule(r){3-4} \cmidrule(r){5-6} \cmidrule(r){7-8} \cmidrule(r){9-10}
        & &  w/o  & w/  & w/o  & w/  & w/o  & w/  & w/o  & w/ \\
        % Model & Correlation & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
         \midrule   
        % & \multicolumn{4}{c}{Local Spearman Correlation $\downarrow$} \\ 
        % \hline
        \multirow{3}{*}{\rotatebox[origin=c]{90}{Res.}}
        % \multirow{3}{\rotatebox[origin=c]{90}{Res.}} 
        & MoRF VS GT $\uparrow$ &  \ms{-0.90}{0.06}  &  \ms{-0.61}{0.02}  &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00} &  \ms{-0.65}{0.02} &  \ms{-0.28}{0.05}  &  \ms{-0.26}{0.00}    &  \ms{0.25}{0.00}\\
        & LeRF VS GT $\downarrow$ & \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{-0.92}{0.05} &  \ms{0.62}{0.02} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} \\
        & MoRF VS LeRF $\downarrow$ &  \ms{0.90}{0.06} &  \ms{0.61}{0.02} &  \ms{\textbf{-0.92}}{0.05} &  \ms{0.62}{0.02} &  \ms{0.65}{0.02} &  \ms{0.28}{0.05}  &  \ms{0.26}{0.00}   &  \ms{\textbf{-0.26}}{0.00}\\
        \hline
        \multirow{3}{*}{\rotatebox[origin=c]{90}{ViT}}
        % \multirow{3}{\rotatebox[origin=c]{90}{ViT}} 
        & MoRF VS GT $\uparrow$ &  \ms{0.94}{0.00}  &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00} \\
        & LeRF VS GT $\downarrow$ &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{0.83}{0.00}  &  \ms{0.83}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
        & MoRF VS LeRF $\downarrow$ & \ms{-0.94}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{0.83}{0.00}  &  \ms{0.83}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
        
        % % \makecell*[c]{Global \\ Correlation $\downarrow$ } & \\
        % w/o fine-tune & $0.33\pm0.08$ & $0.94\pm0.06$ & $-0.33\pm0.06$ & $-\textbf{0.87}\pm0.06$ \\
        % w/ fine-tune & $-\textbf{1.00}\pm0.00$ & $-{0.68}\pm0.08$ & $-\textbf{1.00}\pm0.00$ & $-\textbf{1.00}\pm0.00$ \\

        
        % w/o fine-tune & $-0.82\pm0.02$ & $0.89\pm0.07$ & $-\textbf{1.00}\pm0.00$ & $-\textbf{1.00}\pm0.00$ \\
        % w/ fine-tune  & $-0.47\pm0.04$ & $0.83\pm0.00$ & $-\textbf{1.00}\pm0.00$ & $-\textbf{1.00}\pm0.00$ \\
        \bottomrule

        
    \end{tabular}
    }
\end{table*}


==> experiments/his/food101-vit-finetune-fid.tex <==

% \begin{table*}[h]
%     \centering
%         \caption{Fidelity results on \tinyimagenet~dataset with finetuned ViT as the model to be explained. The x-axis of the local correlation is the explanation size with hyperparameter top $k$. The global correlation means the rank Spearman correlation of average fidelity. The best performance is marked as bold. For R-Fidelity and F-Fidelity, $\alpha_1=\alpha_2=0.5$. In F-Fidelity, $\beta=0.1$. }
%     \label{tab:exp:food:vit-finetune:fid}
%     \scalebox{1.0}{
%      \begin{tabular}{ccccc}
%         \hline
%         Results  & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
%         \hline   
%         \makecell*[c]{$Fid^+$}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_finetune_vitmodel_ori_interv0.2_gradcam_moRF.png}}
% 	  \end{minipage}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_finetune_vitmodel_ori_interv0.2_gradcam_moRF.png}}
% 	  \end{minipage}
        
%         & 
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_finetune_vitmodel_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_moRF.png}}
% 	  \end{minipage}

%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_finetune_vitmodel_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_moRF.png}}
% 	  \end{minipage}        \\

%         \makecell*[c]{$Fid^-$ }
%          &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_finetune_vitmodel_ori_interv0.2_gradcam_leRF.png}}
% 	  \end{minipage}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_finetune_vitmodel_ori_interv0.2_gradcam_leRF.png}}
% 	  \end{minipage}
        
%         & 
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_finetune_vitmodel_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_leRF.png}}
% 	  \end{minipage}

%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_finetune_vitmodel_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_leRF.png}}
% 	  \end{minipage}        \\
            
%          \hline
        
%     \end{tabular}
%     }
% \end{table*}

\begin{table*}[h]
    \centering
        \caption{Fidelity results on \food~dataset with finetuned ViT as the model to be explained. The x-axis of the local correlation is the explanation size with hyperparameter top $k$. The global correlation means the rank Spearman correlation of average fidelity. The best performance is marked as bold. For R-Fidelity and F-Fidelity, $\alpha_1=\alpha_2=0.5$. In F-Fidelity, $\beta=0.1$.}
        % The global correlation means the rank Spearman correlation of average fidelity. The best performance is marked as bold. 
    \label{tab:exp:food:vit-finetune:fid}
    \scalebox{1.0}{
     \begin{tabular}{ccccc}
        \hline
        Method  & {$Fid^+$}  & {$Fid^-$ } & \makecell*[c]{Local Spearman \\ Correlation }  \\ %R-Fidelity  &  {F-Fidelity} \\
        \hline   
        % \makecell*[c]{$Fid^+$}
        Fidelity &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_finetune_vitmodel_ori_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_finetune_vitmodel_ori_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        
        & 
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_finetune_vitmodel_ori_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage} \\

        % \makecell*[c]{$Fid^-$ }
         ROAD &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_finetune_vitmodel_road_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_finetune_vitmodel_road_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        & 
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_finetune_vitmodel_road_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage} \\

        
         R-Fidelity &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_finetune_vitmodel_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_finetune_vitmodel_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        & 
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_finetune_vitmodel_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage} \\

         F-Fidelity &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_finetune_vitmodel_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_finetune_vitmodel_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        & 
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_finetune_vitmodel_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage} \\
            
         \hline
        
    \end{tabular}
    }
\end{table*}


==> experiments/his/food101-vit-finetune.tex <==
\begin{table*}[h]
    \centering
        \caption{Rank Spearman correlation results on \food~dataset with finetuned ViT as the model to be explained. The x-axis of the local correlation is the explanation size with hyperparameter top $k$. The global correlation means the rank Spearman correlation of average fidelity. The best performance is marked as bold. For R-Fidelity and F-Fidelity, $\alpha_1=\alpha_2=0.5$. In F-Fidelity, $\beta=0.1$. }
    \label{tab:exp:food:vit-finetune}
    \scalebox{1.0}{
     \begin{tabular}{ccccc}
        \hline
        Results  & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
        \hline   
        \makecell*[c]{Local \\ Correlation $\downarrow$ }
        &
        \begin{minipage}[b]{0.18\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_finetune_vitmodel_ori_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.18\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_finetune_vitmodel_ori_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage}
        
        & 
        \begin{minipage}[b]{0.18\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_finetune_vitmodel_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage}

        &
        \begin{minipage}[b]{0.18\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_finetune_vitmodel_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage}        \\

        \makecell*[c]{Global \\ Correlation $\downarrow$ }
         & $\textbf{-1.00}\pm0.02$ & PlaceHolder & $\textbf{-1.00}\pm0.00$ & $\textbf{-1.00}\pm0.00$ \\
        \hline

        
    \end{tabular}
    }
\end{table*}

==> experiments/his/food101-vit-ori-fid.tex <==

% \begin{table*}[h]
%     \centering
%         \caption{Fidelity results on \food~dataset with ViT as the model to be explained. The x-axis of the local correlation is the explanation size with hyperparameter top $k$. The global correlation means the rank Spearman correlation of average fidelity. The best performance is marked as bold. For R-Fidelity and F-Fidelity, $\alpha_1=\alpha_2=0.5$. In F-Fidelity, $\beta=0.1$. }
%     \label{tab:exp:food:vit:fid}
%     \scalebox{1.0}{
%      \begin{tabular}{ccccc}
%         \hline
%         Results  & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
%         \hline   
%         \makecell*[c]{$Fid^+$}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_vitmodel_ori_interv0.2_gradcam_moRF.png}}
% 	  \end{minipage}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_vitmodel_ori_interv0.2_gradcam_moRF.png}}
% 	  \end{minipage}
        
%         & 
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_vitmodel_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_moRF.png}}
% 	  \end{minipage}

%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_vitmodel_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_moRF.png}}
% 	  \end{minipage}        \\

%         \makecell*[c]{$Fid^-$ }
%          &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_vitmodel_ori_interv0.2_gradcam_leRF.png}}
% 	  \end{minipage}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_vitmodel_ori_interv0.2_gradcam_leRF.png}}
% 	  \end{minipage}
        
%         & 
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_vitmodel_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_leRF.png}}
% 	  \end{minipage}

%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_vitmodel_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_leRF.png}}
% 	  \end{minipage}        \\
            
%          \hline
        
%     \end{tabular}
%     }
% \end{table*}


\begin{table*}[h]
    \centering
        \caption{Fidelity results on \food~dataset with ViT as the model to be explained. The x-axis of the local correlation is the explanation size with hyperparameter top $k$. The global correlation means the rank Spearman correlation of average fidelity. The best performance is marked as bold. For R-Fidelity and F-Fidelity, $\alpha_1=\alpha_2=0.5$. In F-Fidelity, $\beta=0.1$.}
        % The global correlation means the rank Spearman correlation of average fidelity. The best performance is marked as bold. 
    \label{tab:exp:food:vit:fid}
    \scalebox{1.0}{
     \begin{tabular}{ccccc}
        \hline
        Method  & {$Fid^+$}  & {$Fid^-$ } & \makecell*[c]{Local Spearman \\ Correlation }  \\ %R-Fidelity  &  {F-Fidelity} \\
        \hline   
        % \makecell*[c]{$Fid^+$}
        Fidelity &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_vitmodel_ori_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_vitmodel_ori_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        
        & 
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_vitmodel_ori_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage} \\

        % \makecell*[c]{$Fid^-$ }
         ROAD &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_vitmodel_road_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_vitmodel_road_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        & 
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_vitmodel_road_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage} \\

        
         R-Fidelity &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_vitmodel_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_vitmodel_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        & 
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_vitmodel_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage} \\

         F-Fidelity &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_vitmodel_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_vitmodel_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        & 
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_vitmodel_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage} \\
            
         \hline
        
    \end{tabular}
    }
\end{table*}




==> experiments/his/food101-vit-ori.tex <==
\begin{table*}[h]
    \centering
        \caption{Rank Spearman correlation results on \food~dataset with ViT as the model to be explained. The x-axis of the local correlation is the explanation size with hyperparameter top $k$. The global correlation means the rank Spearman correlation of average fidelity. The best performance is marked as bold. For R-Fidelity and F-Fidelity, $\alpha_1=\alpha_2=0.5$. In F-Fidelity, $\beta=0.1$. }
    \label{tab:exp:food:vit}
    \scalebox{1.0}{
     \begin{tabular}{ccccc}
        \hline
        Results  & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
        \hline   
        \makecell*[c]{Local \\ Correlation $\downarrow$ }
        &
        \begin{minipage}[b]{0.18\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_vitmodel_ori_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.18\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_vitmodel_ori_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage}
        
        & 
        \begin{minipage}[b]{0.18\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_vitmodel_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage}

        &
        \begin{minipage}[b]{0.18\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_vitmodel_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage}        \\

        \makecell*[c]{Global \\ Correlation $\downarrow$ }
         & $-0.94\pm0.00$ & PlaceHolder & $\textbf{-1.00}\pm0.00$ & $\textbf{-1.00}\pm0.00$ \\
        \hline

        
    \end{tabular}
    }
\end{table*}

==> experiments/his/sst2-bert-finetune-fid.tex <==
\begin{table*}[h]
    \centering
        \caption{Fidelity results on \sst~dataset with finetuned Bert as the model to be explained. The x-axis of the local correlation is the explanation size with hyperparameter top $k$. The global correlation means the rank Spearman correlation of average fidelity. The best performance is marked as bold. For R-Fidelity and F-Fidelity, $\alpha_1=\alpha_2=0.5$. In F-Fidelity, $\beta=0.1$. }
    \label{tab:exp:sst:bert-finetune:fid}
    \scalebox{1.0}{
     \begin{tabular}{cccc}

        \hline
        Method  & {$Fid^+$}  & {$Fid^-$ } & \makecell*[c]{Local Spearman \\ Correlation }  \\ %R-Fidelity  &  {F-Fidelity} \\
        \hline   
        % \makecell*[c]{$Fid^+$}
        Fidelity &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_finetune_bert_ori_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_finetune_bert_ori_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        
        & 
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_finetune_bert_ori_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage} \\
        
         R-Fidelity &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_finetune_bert_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_finetune_bert_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        & 
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_finetune_bert_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage} \\

         F-Fidelity &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_finetune_bert_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_finetune_bert_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        & 
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_finetune_bert_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage} \\
            
         \hline
        
        
    \end{tabular}
    }
\end{table*}

==> experiments/his/sst2-bert-finetune.tex <==
\begin{table*}[h]
    \centering
        \caption{Rank Spearman correlation results on \sst~dataset with finetuned Bert as the model to be explained. The x-axis of the local correlation is the explanation size with hyperparameter top $k$. The global correlation means the rank Spearman correlation of average fidelity. The best performance is marked as bold. For R-Fidelity and F-Fidelity, $\alpha_1=\alpha_2=0.5$. In F-Fidelity, $\beta=0.1$. }
    \label{tab:exp:sst:bert-finetune}
    \scalebox{1.0}{
     \begin{tabular}{cccc}
        \hline
        Results  & Fidelity  & R-Fidelity  &  {F-Fidelity} \\
        \hline   
        \makecell*[c]{Local \\ Correlation $\downarrow$ }
        &
        \begin{minipage}[b]{0.18\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_finetune_bert_ori_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage}
  %       &
  %       \begin{minipage}[b]{0.18\columnwidth}
		% \centering
  %               \vspace{2pt}
		% \raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_vitmodel_ori_interv0.2_gradcam_SpearmanCoeff.png}}
	 %  \end{minipage}
        
        & 
        \begin{minipage}[b]{0.18\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_finetune_bert_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage}

        &
        \begin{minipage}[b]{0.18\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_finetune_bert_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage}        \\

        \makecell*[c]{Global \\ Correlation $\downarrow$ }
         & $\textbf{-1.00}\pm0.00$ & $\textbf{-1.00}\pm0.00$ & $\textbf{-1.00}\pm0.00$ \\
        \hline

        
    \end{tabular}
    }
\end{table*}

==> experiments/his/sst2-bert-ori-fid.tex <==
% \begin{table*}[h]
%     \centering
%         \caption{Fidelity results on \sst~dataset with Bert as the model to be explained. The x-axis of the local correlation is the explanation size with hyperparameter top $k$. The global correlation means the rank Spearman correlation of average fidelity. The best performance is marked as bold. For R-Fidelity and F-Fidelity, $\alpha_1=\alpha_2=0.5$. In F-Fidelity, $\beta=0.1$. }
%     \label{tab:exp:sst:bert:fid}
%     \scalebox{1.0}{
%      \begin{tabular}{cccc}
%         \hline
%         Results  & Fidelity  & R-Fidelity  &  {F-Fidelity} \\
%         \hline   
%         \makecell*[c]{$Fid^+$}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_ori_bert_ori_interv0.2_gradcam_moRF.png}}
% 	  \end{minipage}
%         & 
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_ori_bert_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_moRF.png}}
% 	  \end{minipage}

%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_ori_bert_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_moRF.png}}
% 	  \end{minipage}        \\

%         \makecell*[c]{$Fid^-$ }
%          &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_ori_bert_ori_interv0.2_gradcam_leRF.png}}
% 	  \end{minipage}
        
        
%         & 
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_ori_bert_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_leRF.png}}
% 	  \end{minipage}

%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_ori_bert_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_leRF.png}}
% 	  \end{minipage}        \\
            
%          \hline
        
%     \end{tabular}
%     }
% \end{table*}

\begin{table*}[h]
    \centering
        \caption{Fidelity results on \sst~dataset with Bert as the model to be explained. The x-axis of the local correlation is the explanation size with hyperparameter top $k$. The global correlation means the rank Spearman correlation of average fidelity. The best performance is marked as bold. For R-Fidelity and F-Fidelity, $\alpha_1=\alpha_2=0.5$. In F-Fidelity, $\beta=0.1$. }
    % The global correlation means the rank Spearman correlation of average fidelity. The best performance is marked as bold. 
    \label{tab:exp:sst:bert:fid}
    \scalebox{1.0}{
     \begin{tabular}{ccccc}
        \hline
        Method  & {$Fid^+$}  & {$Fid^-$ } & \makecell*[c]{Local Spearman \\ Correlation }  \\ %R-Fidelity  &  {F-Fidelity} \\
        \hline   
        % \makecell*[c]{$Fid^+$}
        Fidelity &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_ori_bert_ori_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_ori_bert_ori_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        
        & 
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_ori_bert_ori_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage} \\

        % \makecell*[c]{$Fid^-$ }

         R-Fidelity &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_ori_bert_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_ori_bert_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        & 
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_ori_bert_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage} \\

         F-Fidelity &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_ori_bert_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_ori_bert_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        & 
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_ori_bert_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage} \\
            
         \hline
        
    \end{tabular}
    }
\end{table*}


==> experiments/his/sst2-bert-ori.tex <==
% \begin{table*}[h]
%     \centering
%         \caption{Rank Spearman correlation results on \sst~dataset with Bert as the model to be explained. The x-axis of the local correlation is the explanation size with hyperparameter top $k$. The global correlation means the rank Spearman correlation of average fidelity. The best performance is marked as bold. For R-Fidelity and F-Fidelity, $\alpha_1=\alpha_2=0.5$. In F-Fidelity, $\beta=0.1$. }
%     \label{tab:exp:sst:bert}
%     \scalebox{1.0}{
%      \begin{tabular}{cccc}
%         \hline
%         Results  & Fidelity  & R-Fidelity  &  {F-Fidelity} \\
%         \hline   
%         \makecell*[c]{Local \\ Correlation $\downarrow$ }
%         &
%         \begin{minipage}[b]{0.18\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_ori_bert_ori_interv0.2_gradcam_SpearmanCoeff.png}}
% 	  \end{minipage}
%   %       &
%   %       \begin{minipage}[b]{0.18\columnwidth}
% 		% \centering
%   %               \vspace{2pt}
% 		% \raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_vitmodel_ori_interv0.2_gradcam_SpearmanCoeff.png}}
% 	 %  \end{minipage}
        
%         & 
%         \begin{minipage}[b]{0.18\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_ori_bert_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_SpearmanCoeff.png}}
% 	  \end{minipage}

%         &
%         \begin{minipage}[b]{0.18\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_ori_bert_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_SpearmanCoeff.png}}
% 	  \end{minipage}        \\

%         \makecell*[c]{Global \\ Correlation $\downarrow$ }
%          & $\textbf{-1.00}\pm0.00$ & $\textbf{-1.00}\pm0.00$ & $\textbf{-1.00}\pm0.00$ \\
%         \hline

        
%     \end{tabular}
%     }
% \end{table*}

% \begin{table*}[h]
%     \centering
%         \caption{Rank Spearman correlation results on \sst~dataset with Bert as the model to be explained. The x-axis of the local correlation is the explanation size with hyperparameter top $k$. The global correlation means the rank Spearman correlation of average fidelity. The best performance is marked as bold. For R-Fidelity and F-Fidelity, $\alpha_1=\alpha_2=0.5$. In F-Fidelity, $\beta=0.1$. }
%     \label{tab:exp:sst:bert}
%     \scalebox{1.0}{
%      \begin{tabular}{cccc}
%         \hline
%           & Fidelity  & R-Fidelity  &  {F-Fidelity} \\
%         \hline   
%         \makecell*[c]{Local \quad \\Spearman \quad \\ Correlation $\downarrow$ }
%         &
%         \begin{minipage}[b]{0.185\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/merge/image_finetune_bert_ori_interv0.2_gradcam_SpearmanCoeff.png}}
% 	  \end{minipage}
%   %       &
%   %       \begin{minipage}[b]{0.18\columnwidth}
% 		% \centering
%   %               \vspace{2pt}
% 		% \raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_vitmodel_ori_interv0.2_gradcam_SpearmanCoeff.png}}
% 	 %  \end{minipage}
        
%         & 
%         \begin{minipage}[b]{0.185\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/merge/image_finetune_bert_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_SpearmanCoeff.png}}
% 	  \end{minipage}

%         &
%         \begin{minipage}[b]{0.185\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/merge/image_finetune_bert_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_SpearmanCoeff.png}}
% 	  \end{minipage}        \\
%    \\
%    \hline
%     \multicolumn{4}{c}{Global Spearman Correlation $\downarrow$} \\ 
%    \hline

%         % \makecell*[c]{Global \\ Correlation $\downarrow$ }
%          w/o fine-tune &   $\textbf{-1.00}\pm0.00$ & $\textbf{-1.00}\pm0.00$ & $\textbf{-1.00}\pm0.00$ \\
%          w/ fine-tune &  $\textbf{-1.00}\pm0.00$ & $\textbf{-1.00}\pm0.00$ & $\textbf{-1.00}\pm0.00$ \\
%         \hline

        
%     \end{tabular}
%     }
% \end{table*}

\begin{table*}[h]
    \centering
        \caption{Rank Spearman correlation results on \sst~dataset with Bert as the model to be explained. The x-axis of the local correlation is the explanation size with hyperparameter top $k$. The global correlation means the rank Spearman correlation of average fidelity. The best performance is marked as bold. For R-Fidelity and F-Fidelity, $\alpha_1=\alpha_2=0.5$. In F-Fidelity, $\beta=0.1$. }
    \label{tab:exp:sst:bert}
    \scalebox{0.75}{
     \begin{tabular}{cccccccccc}
        \toprule
        \multirow{2}{*}{Model} &
        \multirow{2}{*}{Correlation} &
        \multicolumn{2}{c}{Fidelity} &
        \multicolumn{2}{c}{FIM} & 
        \multicolumn{2}{c}{R-Fidelity} & 
        \multicolumn{2}{c}{F-Fidelity} \\
        \cmidrule(r){3-4} \cmidrule(r){5-6} \cmidrule(r){7-8} \cmidrule(r){9-10}
        & &  w/o  & w/  & w/o  & w/  & w/o  & w/  & w/o  & w/ \\
        % Model & Correlation & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
         \midrule   
        % & \multicolumn{4}{c}{Local Spearman Correlation $\downarrow$} \\ 
        % \hline
        \multirow{3}{*}{\rotatebox[origin=c]{90}{Bert}}
        % \multirow{3}{\rotatebox[origin=c]{90}{Res.}} 
        & MoRF VS GT $\uparrow$ &  \ms{1.00}{0.00} &  \ms{1.00}{0.00} & & & \ms{1.00}{0.00} & \ms{1.00}{0.00} & \ms{1.00}{0.00} & \ms{1.00}{0.00} \\
        & LeRF VS GT $\downarrow$ & \ms{-1.00}{0.00} & \ms{-1.00}{0.00}  & & & \ms{-1.00}{0.00} & \ms{-1.00}{0.00} & \ms{1.00}{0.00} & \ms{1.00}{0.00} \\
        & MoRF VS LeRF $\downarrow$ &  \ms{-1.00}{0.00} &  \ms{-1.00}{0.00} & & & \ms{-1.00}{0.00} & \ms{-1.00}{0.00} & \ms{1.00}{0.00} & \ms{1.00}{0.00}\\
        \hline
        \multirow{3}{*}{\rotatebox[origin=c]{90}{GPT2}}
        % \multirow{3}{\rotatebox[origin=c]{90}{ViT}} 
        & MoRF VS GT $\uparrow$ &  \ms{0.94}{0.06}  &  \ms{0.97}{0.03}  & & & \ms{0.91}{0.09}  & \ms{0.97}{0.03} & \ms{0.89}{0.14} & \ms{0.98}{0.03} \\
        & LeRF VS GT $\downarrow$ &  \ms{-0.97}{0.03} &  \ms{-1.00}{0.00} & & & \ms{-0.92}{0.08} & \ms{-0.99}{0.02} & \ms{-0.95}{0.07} & \ms{-0.98}{0.05} \\
        & MoRF VS LeRF $\downarrow$&  \ms{-0.92}{0.08}   & \ms{-0.97}{0.03} & & & \ms{-0.89}{0.07} & \ms{-0.98}{0.03} & \ms{-0.90}{0.15} & \ms{-0.95}{0.04}\\
        
        % % \makecell*[c]{Global \\ Correlation $\downarrow$ } & \\
        % w/o fine-tune & $0.33\pm0.08$ & $0.94\pm0.06$ & $-0.33\pm0.06$ & $-\textbf{0.87}\pm0.06$ \\
        % w/ fine-tune & $-\textbf{1.00}\pm0.00$ & $-{0.68}\pm0.08$ & $-\textbf{1.00}\pm0.00$ & $-\textbf{1.00}\pm0.00$ \\

        
        % w/o fine-tune & $-0.82\pm0.02$ & $0.89\pm0.07$ & $-\textbf{1.00}\pm0.00$ & $-\textbf{1.00}\pm0.00$ \\
        % w/ fine-tune  & $-0.47\pm0.04$ & $0.83\pm0.00$ & $-\textbf{1.00}\pm0.00$ & $-\textbf{1.00}\pm0.00$ \\
        \bottomrule

        
    \end{tabular}
}    
\end{table*}


==> experiments/his/sst2-gpt2-finetune-fid.tex <==
\begin{table*}[h]
    \centering
        \caption{Fidelity results on \sst~dataset with finetuned GPT2 as the model to be explained. The x-axis of the local correlation is the explanation size with hyperparameter top $k$. The global correlation means the rank Spearman correlation of average fidelity. The best performance is marked as bold. For R-Fidelity and F-Fidelity, $\alpha_1=\alpha_2=0.5$. In F-Fidelity, $\beta=0.1$. }
    \label{tab:exp:sst:gpt2-finetune:fid}
    \scalebox{1.0}{
     \begin{tabular}{cccc}
        \hline
        Method  & {$Fid^+$}  & {$Fid^-$ } & \makecell*[c]{Local Spearman \\ Correlation }  \\ %R-Fidelity  &  {F-Fidelity} \\
        \hline   
        % \makecell*[c]{$Fid^+$}
        Fidelity &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_finetune_gpt2_ori_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_finetune_gpt2_ori_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        
        & 
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_finetune_gpt2_ori_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage} \\

        % \makecell*[c]{$Fid^-$ }

         R-Fidelity &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_finetune_gpt2_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_finetune_gpt2_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        & 
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_finetune_gpt2_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage} \\

         F-Fidelity &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_finetune_gpt2_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_finetune_gpt2_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        & 
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_finetune_gpt2_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage} \\
            
         \hline
        
    \end{tabular}
    }
\end{table*}

==> experiments/his/sst2-gpt2-finetune.tex <==
\begin{table*}[h]
    \centering
        \caption{Rank Spearman correlation results on \sst~dataset with finetuned GPT2 as the model to be explained. The x-axis of the local correlation is the explanation size with hyperparameter top $k$. The global correlation means the rank Spearman correlation of average fidelity. The best performance is marked as bold. For R-Fidelity and F-Fidelity, $\alpha_1=\alpha_2=0.5$. In F-Fidelity, $\beta=0.1$. }
    \label{tab:exp:sst:gpt2-finetune}
    \scalebox{1.0}{
     \begin{tabular}{cccc}
        \hline
        Results  & Fidelity  & R-Fidelity  &  {F-Fidelity} \\
        \hline   
        \makecell*[c]{Local \\ Correlation $\downarrow$ }
        &
        \begin{minipage}[b]{0.18\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_finetune_gpt2_ori_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage}
  %       &
  %       \begin{minipage}[b]{0.18\columnwidth}
		% \centering
  %               \vspace{2pt}
		% \raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_vitmodel_ori_interv0.2_gradcam_SpearmanCoeff.png}}
	 %  \end{minipage}
        
        & 
        \begin{minipage}[b]{0.18\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_finetune_gpt2_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage}

        &
        \begin{minipage}[b]{0.18\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_finetune_gpt2_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage}        \\

        \makecell*[c]{Global \\ Correlation $\downarrow$ }
         & $-0.21\pm0.22$ & ${-0.27}\pm0.14$ & $\textbf{-0.76}\pm0.08$ \\
        \hline

        
    \end{tabular}
    }
\end{table*}

==> experiments/his/sst2-gpt2-ori-fid.tex <==
\begin{table*}[h]
    \centering
        \caption{Fidelity results on \sst~dataset with GPT2 as the model to be explained. The x-axis of the local correlation is the explanation size with hyperparameter top $k$. The global correlation means the rank Spearman correlation of average fidelity. The best performance is marked as bold. For R-Fidelity and F-Fidelity, $\alpha_1=\alpha_2=0.5$. In F-Fidelity, $\beta=0.1$. }
    \label{tab:exp:sst:gpt2:fid}
    \scalebox{1.0}{
     \begin{tabular}{cccc}
        \hline
        Method  & {$Fid^+$}  & {$Fid^-$ } & \makecell*[c]{Local Spearman \\ Correlation }  \\ %R-Fidelity  &  {F-Fidelity} \\
        \hline   
        % \makecell*[c]{$Fid^+$}
        Fidelity &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_ori_gpt2_ori_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_ori_gpt2_ori_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        
        & 
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_ori_gpt2_ori_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage} \\

        % \makecell*[c]{$Fid^-$ }

         R-Fidelity &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_ori_gpt2_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_ori_gpt2_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        & 
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_ori_gpt2_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage} \\

         F-Fidelity &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_ori_gpt2_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_ori_gpt2_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        & 
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_ori_gpt2_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage} \\
            
         \hline
        
    \end{tabular}
    }
\end{table*}

==> experiments/his/sst2-gpt2-ori.tex <==
\begin{table*}[h]
    \centering
        \caption{Rank Spearman correlation results on \sst~dataset with GPT2 as the model to be explained. The x-axis of the local correlation is the explanation size with hyperparameter top $k$. The global correlation means the rank Spearman correlation of average fidelity. The best performance is marked as bold. For R-Fidelity and F-Fidelity, $\alpha_1=\alpha_2=0.5$. In F-Fidelity, $\beta=0.1$. }
    \label{tab:exp:sst:gpt2}
    \scalebox{1.0}{
     \begin{tabular}{cccc}
        \hline
        Results  & Fidelity  & R-Fidelity  &  {F-Fidelity} \\
        \hline   
        \makecell*[c]{Local \\ Correlation $\downarrow$ }
        &
        \begin{minipage}[b]{0.18\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_ori_gpt2_ori_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage}
  %       &
  %       \begin{minipage}[b]{0.18\columnwidth}
		% \centering
  %               \vspace{2pt}
		% \raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/food101/image_ori_vitmodel_ori_interv0.2_gradcam_SpearmanCoeff.png}}
	 %  \end{minipage}
        
        & 
        \begin{minipage}[b]{0.18\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_ori_gpt2_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage}

        &
        \begin{minipage}[b]{0.18\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/SST2/image_ori_gpt2_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage}        \\

        \makecell*[c]{Global \\ Correlation $\downarrow$ }
         & $-0.93\pm0.02$ & $\textbf{-0.95}\pm0.04$ & ${-0.93}\pm0.02$ \\
        \hline

        
    \end{tabular}
    }
\end{table*}

==> experiments/his/tinyimagenet-resnet-finetune-fid.tex <==

% \begin{table*}[h]
%     \centering
%         \caption{Fidelity results on \tinyimagenet~dataset with finetuned Resnet-18 as the model to be explained. The x-axis of the local correlation is the explanation size with hyperparameter top $k$. The global correlation means the rank Spearman correlation of average fidelity. The best performance is marked as bold. For R-Fidelity and F-Fidelity, $\alpha_1=\alpha_2=0.5$. In F-Fidelity, $\beta=0.1$. }
%     \label{tab:exp:tinyimagenet:resnet-finetune:fid}
%     \scalebox{1.0}{
%      \begin{tabular}{ccccc}
%         \hline
%         Results  & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
%         \hline   
%         \makecell*[c]{$Fid^+$}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_finetune_model_ori_interv0.2_gradcam_moRF.png}}
% 	  \end{minipage}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_finetune_model_road_interv0.2_gradcam_moRF.png}}
% 	  \end{minipage}
        
%         & 
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_finetune_model_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_moRF.png}}
% 	  \end{minipage}

%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_finetune_model_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_moRF.png}}
% 	  \end{minipage}        \\

%         \makecell*[c]{$Fid^-$ }
%          &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_finetune_model_ori_interv0.2_gradcam_leRF.png}}
% 	  \end{minipage}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_finetune_model_road_interv0.2_gradcam_leRF.png}}
% 	  \end{minipage}
        
%         & 
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_finetune_model_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_leRF.png}}
% 	  \end{minipage}

%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_finetune_model_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_leRF.png}}
% 	  \end{minipage}        \\
            
%          \hline
        
%     \end{tabular}
%     }
% \end{table*}


\begin{table*}[h]
    \centering
        \caption{Fidelity results on \tinyimagenet~dataset with fine-tuned Resnet-18 as the model to be explained. The x-axis of the local correlation is the explanation size with hyperparameter top $k$. For R-Fidelity and F-Fidelity, $\alpha_1=\alpha_2=0.5$. In F-Fidelity, $\beta=0.1$. }
        % The global correlation means the rank Spearman correlation of average fidelity. The best performance is marked as bold. 
    \label{tab:exp:tinyimagenet:resnet-finetune:fid}
    \scalebox{1.0}{
     \begin{tabular}{ccccc}
        \hline
        Method  & {$Fid^+$}  & {$Fid^-$ } & \makecell*[c]{Local Spearman \\ Correlation }  \\ %R-Fidelity  &  {F-Fidelity} \\
        \hline   
        % \makecell*[c]{$Fid^+$}
        Fidelity &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_finetune_model_ori_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_finetune_model_ori_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        
        & 
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_finetune_model_ori_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage} \\

        % \makecell*[c]{$Fid^-$ }
         ROAD &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_finetune_model_road_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_finetune_model_road_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        & 
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_finetune_model_road_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage} \\

        
         R-Fidelity &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_finetune_model_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_finetune_model_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        & 
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_finetune_model_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage} \\

         F-Fidelity &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_finetune_model_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_finetune_model_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        & 
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_finetune_model_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage} \\
            
         \hline
        
    \end{tabular}
    }
\end{table*}


==> experiments/his/tinyimagenet-resnet-finetune.tex <==

\begin{table*}[h]
    \centering
        \caption{Rank Spearman correlation results on \tinyimagenet~dataset with finetuned Resnet-18 as the model to be explained. The x-axis of the local correlation is the explanation size with hyperparameter top $k$. The global correlation means the rank Spearman correlation of average fidelity. The best performance is marked as bold. For R-Fidelity and F-Fidelity, $\alpha_1=\alpha_2=0.5$. In F-Fidelity, $\beta=0.1$.}
    \label{tab:exp:tinyimagenet:resnet-finetune}
    \scalebox{1.0}{
     \begin{tabular}{ccccc}
        \hline
        Results  & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
        \hline   
        \makecell*[c]{Local \\ Correlation $\downarrow$ }
        &
        \begin{minipage}[b]{0.18\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_finetune_model_ori_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.18\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_finetune_model_road_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage}
        
        & 
        \begin{minipage}[b]{0.18\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_finetune_model_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage}

        &
        \begin{minipage}[b]{0.18\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_finetune_model_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage}        \\

        \makecell*[c]{Global \\ Correlation $\downarrow$ }
         & $-\textbf{1.00}\pm0.00$ & $-{0.68}\pm0.08$ & $-\textbf{1.00}\pm0.00$ & $-\textbf{1.00}\pm0.00$ \\
        \hline

        
    \end{tabular}
    }
\end{table*}

==> experiments/his/tinyimagenet-resnet-ori-fid.tex <==

\begin{table*}[h]
    \centering
        \caption{Fidelity results on \tinyimagenet~dataset with Resnet-18 as the model to be explained. The x-axis of the local correlation is the explanation size with hyperparameter top $k$. For R-Fidelity and F-Fidelity, $\alpha_1=\alpha_2=0.5$. In F-Fidelity, $\beta=0.1$. }
        % The global correlation means the rank Spearman correlation of average fidelity. The best performance is marked as bold. 
    \label{tab:exp:tinyimagenet:resnet:fid}
    \scalebox{1.0}{
     \begin{tabular}{ccccc}
        \hline
        Method  & {$Fid^+$}  & {$Fid^-$ } & \makecell*[c]{Local Spearman \\ Correlation }  \\ %R-Fidelity  &  {F-Fidelity} \\
        \hline   
        % \makecell*[c]{$Fid^+$}
        Fidelity &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_ori_model_ori_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_ori_model_ori_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        
        & 
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_ori_model_ori_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage} \\

        % \makecell*[c]{$Fid^-$ }
         ROAD &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_ori_model_road_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_ori_model_road_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        & 
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_ori_model_road_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage} \\

        
         R-Fidelity &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_ori_model_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_ori_model_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        & 
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_ori_model_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage} \\

         F-Fidelity &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_ori_model_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_ori_model_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        & 
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_ori_model_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage} \\
            
         \hline
        
    \end{tabular}
    }
\end{table*}

==> experiments/his/tinyimagenet-resnet-ori.tex <==
% \begin{table*}[h]
%     \centering
%         \caption{Rank Spearman correlation results on \tinyimagenet~dataset with Resnet-18 as the model to be explained. The x-axis of the local correlation is the explanation size with hyperparameter top $k$. The global correlation means the rank Spearman correlation of average fidelity. The best performance is marked as bold. For R-Fidelity and F-Fidelity, $\alpha_1=\alpha_2=0.5$. In F-Fidelity, $\beta=0.1$. }
%     \label{tab:exp:tinyimagenet:resnet}
%     \scalebox{1.0}{
%      \begin{tabular}{ccccc}
%         \hline
%         Results  & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
%         \hline   
%         \makecell*[c]{Local \\ Correlation $\downarrow$ }
%         &
%         \begin{minipage}[b]{0.18\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_ori_model_ori_interv0.2_gradcam_SpearmanCoeff.png}}
% 	  \end{minipage}
%         &
%         \begin{minipage}[b]{0.18\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_ori_model_road_interv0.2_gradcam_SpearmanCoeff.png}}
% 	  \end{minipage}
        
%         & 
%         \begin{minipage}[b]{0.18\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_ori_model_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_SpearmanCoeff.png}}
% 	  \end{minipage}

%         &
%         \begin{minipage}[b]{0.18\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_ori_model_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_SpearmanCoeff.png}}
% 	  \end{minipage}        \\

%         \makecell*[c]{Global \\ Correlation $\downarrow$ }
%          & $0.33\pm0.08$ & $0.94\pm0.06$ & $-0.33\pm0.06$ & $-\textbf{0.87}\pm0.06$ \\
%         \hline

        
%     \end{tabular}
%     }
% \end{table*}

% \begin{table*}[h]
%     \centering
%         \caption{Rank Spearman correlation results on \tinyimagenet~dataset with Resnet-18 as the model to be explained. The x-axis of the local correlation is the explanation size with hyperparameter top $k$. The global correlation means the rank Spearman correlation of average fidelity. The best performance is marked as bold. For R-Fidelity and F-Fidelity, $\alpha_1=\alpha_2=0.5$. In F-Fidelity, $\beta=0.1$. }
%     \label{tab:exp:tinyimagenet:resnet}
%     \scalebox{1.0}{
%      \begin{tabular}{ccccc}
%         \hline
%           & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
%         \hline   
%         % & \multicolumn{4}{c}{Local Spearman Correlation $\downarrow$} \\ 
%         \makecell*[c]{Local \quad \\Spearman \quad \\ Correlation $\downarrow$ }
%         &
%         \begin{minipage}[b]{0.18\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/merge/image_finetune_model_ori_interv0.2_gradcam_SpearmanCoeff.png}}
% 	  \end{minipage}
%         &
%         \begin{minipage}[b]{0.18\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/merge/image_finetune_model_road_interv0.2_gradcam_SpearmanCoeff.png}}
% 	  \end{minipage}
        
%         & 
%         \begin{minipage}[b]{0.18\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/merge/image_finetune_model_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_SpearmanCoeff.png}}
% 	  \end{minipage}

%         &
%         \begin{minipage}[b]{0.18\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/merge/image_finetune_model_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_SpearmanCoeff.png}}
% 	  \end{minipage}        \\
%         \\
%         \hline
%         \multicolumn{5}{c}{Global Spearman Correlation $\downarrow$} \\ 
%         \hline
%         % \makecell*[c]{Global \\ Correlation $\downarrow$ } & \\
%         w/o fine-tune & $0.33\pm0.08$ & $0.94\pm0.06$ & $-0.33\pm0.06$ & $-\textbf{0.87}\pm0.06$ \\
%         w/ fine-tune & $-\textbf{1.00}\pm0.00$ & $-{0.68}\pm0.08$ & $-\textbf{1.00}\pm0.00$ & $-\textbf{1.00}\pm0.00$ \\
%         \hline

        
%     \end{tabular}
%     }
% \end{table*}


\begin{table*}[h]
    \centering
        \caption{Global Spearman rank correlation results on \tinyimagenet~dataset which compares the average fidelity of different explanation size between $5\%$ to $95\%$. The best performance is marked as bold. For R-Fidelity and F-Fidelity, $\alpha_1=\alpha_2=0.5$. In F-Fidelity, $\beta=0.1$. }
    \label{tab:exp:tinyimagenet:resnet}
    \scalebox{0.75}{
     \begin{tabular}{cccccccccc}
        \toprule
        \multirow{2}{*}{Model} &
        \multirow{2}{*}{Correlation} &
        \multicolumn{2}{c}{Fidelity} &
        \multicolumn{2}{c}{ROAD} & 
        \multicolumn{2}{c}{R-Fidelity} & 
        \multicolumn{2}{c}{F-Fidelity} \\
        \cmidrule(r){3-4} \cmidrule(r){5-6} \cmidrule(r){7-8} \cmidrule(r){9-10}
        & &  w/o  & w/  & w/o  & w/  & w/o  & w/  & w/o  & w/ \\
        % Model & Correlation & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
         \midrule   
        % & \multicolumn{4}{c}{Local Spearman Correlation $\downarrow$} \\ 
        % \hline
        \multirow{3}{*}{\rotatebox[origin=c]{90}{Res.}}
        % \multirow{3}{\rotatebox[origin=c]{90}{Res.}} 
        & MoRF VS GT $\uparrow$ &  \ms{-0.33}{0.08} &\ms{\textbf{1.00}}{0.00} & \ms{{0.94}}{0.06} & \ms{\textbf{1.00}}{0.00} & \ms{0.33}{0.06}  & \ms{\textbf{1.00}}{0.00} & \ms{0.87}{0.06}  & \ms{\textbf{1.00}}{0.00}\\
        & LeRF VS GT $\downarrow$ & \ms{\textbf{-1.00}}{0.00} &\ms{\textbf{-1.00}}{0.00} & \ms{1.00}{0.00} & \ms{0.68}{0.08} & \ms{0.33}{0.06} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00}\\
        & MoRF VS LeRF $\downarrow$ &  \ms{0.33}{0.08} & \ms{\textbf{-1.00}}{0.00} & \ms{0.94}{0.06} &  \ms{-0.68}{0.08}  & \ms{-0.33}{0.06} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-0.87}}{0.06} & \ms{\textbf{-1.00}}{0.00}  \\
        \hline
        \multirow{3}{*}{\rotatebox[origin=c]{90}{ViT}}
        % \multirow{3}{\rotatebox[origin=c]{90}{ViT}} 
        & MoRF VS GT $\uparrow$ &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}    &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} \\
        & LeRF VS GT $\downarrow$ &  \ms{-0.82}{0.02} &  \ms{-0.47}{0.04}  &  \ms{0.83}{0.00} &  \ms{0.87}{0.06}  &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
        & MoRF VS LeRF $\downarrow$ & \ms{-0.82}{0.02} & \ms{-0.47}{0.04} & \ms{0.89}{0.07} & \ms{0.83}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00}\\
        
        % % \makecell*[c]{Global \\ Correlation $\downarrow$ } & \\
        % w/o fine-tune & $0.33\pm0.08$ & $0.94\pm0.06$ & $-0.33\pm0.06$ & $-\textbf{0.87}\pm0.06$ \\
        % w/ fine-tune & $-\textbf{1.00}\pm0.00$ & $-{0.68}\pm0.08$ & $-\textbf{1.00}\pm0.00$ & $-\textbf{1.00}\pm0.00$ \\

        
        % w/o fine-tune & $-0.82\pm0.02$ & $0.89\pm0.07$ & $-\textbf{1.00}\pm0.00$ & $-\textbf{1.00}\pm0.00$ \\
        % w/ fine-tune  & $-0.47\pm0.04$ & $0.83\pm0.00$ & $-\textbf{1.00}\pm0.00$ & $-\textbf{1.00}\pm0.00$ \\
        \bottomrule

        
    \end{tabular}
    }
\end{table*}




==> experiments/his/tinyimagenet-vit-finetune-fid.tex <==
% \begin{table*}[h]
%     \centering
%         \caption{Fidelity results on \tinyimagenet~dataset with finetuned ViT as the model to be explained. The x-axis of the local correlation is the explanation size with hyperparameter top $k$. The global correlation means the rank Spearman correlation of average fidelity. The best performance is marked as bold. For R-Fidelity and F-Fidelity, $\alpha_1=\alpha_2=0.5$. In F-Fidelity, $\beta=0.1$. }
%     \label{tab:exp:tinyimagenet:vit-finetune:fid}
%     \scalebox{1.0}{
%      \begin{tabular}{ccccc}
%         \hline
%         Results  & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
%         \hline   
%         \makecell*[c]{$Fid^+$}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_finetune_vitmodel_ori_interv0.2_gradcam_moRF.png}}
% 	  \end{minipage}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_finetune_vitmodel_road_interv0.2_gradcam_moRF.png}}
% 	  \end{minipage}
        
%         & 
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_finetune_vitmodel_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_moRF.png}}
% 	  \end{minipage}

%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_finetune_vitmodel_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_moRF.png}}
% 	  \end{minipage}        \\

%         \makecell*[c]{$Fid^-$ }
%          &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_finetune_vitmodel_ori_interv0.2_gradcam_leRF.png}}
% 	  \end{minipage}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_finetune_vitmodel_road_interv0.2_gradcam_leRF.png}}
% 	  \end{minipage}
        
%         & 
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_finetune_vitmodel_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_leRF.png}}
% 	  \end{minipage}

%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_finetune_vitmodel_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_leRF.png}}
% 	  \end{minipage}        \\
            
%          \hline
        
%     \end{tabular}
%     }
% \end{table*}

\begin{table*}[h]
    \centering
        \caption{Fidelity results on \tinyimagenet~dataset with fine-tuned ViT as the model to be explained. The x-axis of the local correlation is the explanation size with hyperparameter top $k$. For R-Fidelity and F-Fidelity, $\alpha_1=\alpha_2=0.5$. In F-Fidelity, $\beta=0.1$. }
        % The global correlation means the rank Spearman correlation of average fidelity. The best performance is marked as bold. 
    \label{tab:exp:tinyimagenet:vit-finetuned:fid}
    \scalebox{1.0}{
     \begin{tabular}{ccccc}
        \hline
        Method  & {$Fid^+$}  & {$Fid^-$ } & \makecell*[c]{Local Spearman \\ Correlation }  \\ %R-Fidelity  &  {F-Fidelity} \\
        \hline   
        % \makecell*[c]{$Fid^+$}
        Fidelity &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_finetune_vitmodel_ori_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_finetune_vitmodel_ori_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        
        & 
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_finetune_vitmodel_ori_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage} \\

        % \makecell*[c]{$Fid^-$ }
         ROAD &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_finetune_vitmodel_road_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_finetune_vitmodel_road_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        & 
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_finetune_vitmodel_road_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage} \\

        
         R-Fidelity &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_finetune_vitmodel_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_finetune_vitmodel_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        & 
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_finetune_vitmodel_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage} \\

         F-Fidelity &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_finetune_vitmodel_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_finetune_vitmodel_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        & 
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_finetune_vitmodel_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage} \\
            
         \hline
        
    \end{tabular}
    }
\end{table*}



==> experiments/his/tinyimagenet-vit-finetune.tex <==
\begin{table*}[h]
    \centering
    \caption{Rank Spearman correlation results on \tinyimagenet~dataset with finetuned ViT as the model to be explained. The x-axis of the local correlation is the explanation size with hyperparameter top $k$. The global correlation means the rank Spearman correlation of average fidelity. The best performance is marked as bold. For R-Fidelity and F-Fidelity, $\alpha_1=\alpha_2=0.5$. In F-Fidelity, $\beta=0.1$. }
\label{tab:exp:tinyimagenet:vit-finetune}
    \scalebox{1.0}{
     \begin{tabular}{ccccc}
        \hline
        Results  & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
        \hline   
        \makecell*[c]{Local \\ Correlation $\downarrow$ }
        &
        \begin{minipage}[b]{0.18\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_finetune_vitmodel_ori_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.18\columnwidth}
		\centering
                \vspace{2pt}
    		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_finetune_vitmodel_road_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage}
        
        & 
        \begin{minipage}[b]{0.18\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_finetune_vitmodel_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage}

        &
        \begin{minipage}[b]{0.18\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_finetune_vitmodel_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage}        \\

        \makecell*[c]{Global \\ Correlation $\downarrow$ }
         & $-0.47\pm0.04$ & $0.83\pm0.00$ & $-\textbf{1.00}\pm0.00$ & $-\textbf{1.00}\pm0.00$ \\
        \hline

    \end{tabular}
    }
\end{table*}

==> experiments/his/tinyimagenet-vit-ori-fid.tex <==
% \begin{table*}[h]
%     \centering
%         \caption{Fidelity results on \tinyimagenet~dataset with ViT as the model to be explained. The x-axis of the local correlation is the explanation size with hyperparameter top $k$. The global correlation means the rank Spearman correlation of average fidelity. The best performance is marked as bold. For R-Fidelity and F-Fidelity, $\alpha_1=\alpha_2=0.5$. In F-Fidelity, $\beta=0.1$. }
%     \label{tab:exp:tinyimagenet:vit:fid}
%     \scalebox{1.0}{
%      \begin{tabular}{ccccc}
%         \hline
%         Results  & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
%         \hline   
%         \makecell*[c]{$Fid^+$}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_ori_vitmodel_ori_interv0.2_gradcam_moRF.png}}
% 	  \end{minipage}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_ori_vitmodel_road_interv0.2_gradcam_moRF.png}}
% 	  \end{minipage}
        
%         & 
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_ori_vitmodel_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_moRF.png}}
% 	  \end{minipage}

%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_ori_vitmodel_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_moRF.png}}
% 	  \end{minipage}        \\

%         \makecell*[c]{$Fid^-$ }
%          &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_ori_vitmodel_ori_interv0.2_gradcam_leRF.png}}
% 	  \end{minipage}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_ori_vitmodel_road_interv0.2_gradcam_leRF.png}}
% 	  \end{minipage}
        
%         & 
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_ori_vitmodel_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_leRF.png}}
% 	  \end{minipage}

%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_ori_vitmodel_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_leRF.png}}
% 	  \end{minipage}        \\
            
%          \hline
        
%     \end{tabular}
%     }
% \end{table*}


\begin{table*}[h]
    \centering
        \caption{Fidelity results on \tinyimagenet~dataset with ViT as the model to be explained. The x-axis of the local correlation is the explanation size with hyperparameter top $k$. For R-Fidelity and F-Fidelity, $\alpha_1=\alpha_2=0.5$. In F-Fidelity, $\beta=0.1$. }
        % The global correlation means the rank Spearman correlation of average fidelity. The best performance is marked as bold. 
    \label{tab:exp:tinyimagenet:vit:fid}
    \scalebox{1.0}{
     \begin{tabular}{ccccc}
        \hline
        Method  & {$Fid^+$}  & {$Fid^-$ } & \makecell*[c]{Local Spearman \\ Correlation }  \\ %R-Fidelity  &  {F-Fidelity} \\
        \hline   
        % \makecell*[c]{$Fid^+$}
        Fidelity &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_ori_vitmodel_ori_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_ori_vitmodel_ori_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        
        & 
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_ori_vitmodel_ori_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage} \\

        % \makecell*[c]{$Fid^-$ }
         ROAD &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_ori_vitmodel_road_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_ori_vitmodel_road_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        & 
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_ori_vitmodel_road_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage} \\

        
         R-Fidelity &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_ori_vitmodel_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_ori_vitmodel_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        & 
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_ori_vitmodel_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage} \\

         F-Fidelity &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_ori_vitmodel_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_moRF.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_ori_vitmodel_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_leRF.png}}
	  \end{minipage}
        & 
        \begin{minipage}[b]{0.25\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_ori_vitmodel_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage} \\
            
         \hline
        
    \end{tabular}
    }
\end{table*}


==> experiments/his/tinyimagenet-vit-ori.tex <==
% \begin{table*}[h]
%     \centering
%         \caption{Rank Spearman correlation results on \tinyimagenet~dataset with ViT as the model to be explained. The x-axis of the local correlation is the explanation size with hyperparameter top $k$. The global correlation means the rank Spearman correlation of average fidelity. The best performance is marked as bold. For R-Fidelity and F-Fidelity, $\alpha_1=\alpha_2=0.5$. In F-Fidelity, $\beta=0.1$. }
%     \label{tab:exp:tinyimagenet:vit}
%     \scalebox{1.0}{
%      \begin{tabular}{ccccc}
%         \hline
%         Results  & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
%         \hline   
%         \makecell*[c]{Local \\ Correlation $\downarrow$ }
%         &
%         \begin{minipage}[b]{0.18\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_ori_vitmodel_ori_interv0.2_gradcam_SpearmanCoeff.png}}
% 	  \end{minipage}
%         &
%         \begin{minipage}[b]{0.18\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_ori_vitmodel_road_interv0.2_gradcam_SpearmanCoeff.png}}
% 	  \end{minipage}
        
%         & 
%         \begin{minipage}[b]{0.18\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_ori_vitmodel_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_SpearmanCoeff.png}}
% 	  \end{minipage}

%         &
%         \begin{minipage}[b]{0.18\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/image_ori_vitmodel_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_SpearmanCoeff.png}}
% 	  \end{minipage}        \\

%         \makecell*[c]{Global \\ Correlation $\downarrow$ }
%          & $-0.82\pm0.02$ & $0.89\pm0.07$ & $\textbf{-1.00}\pm0.00$ & $\textbf{-1.00}\pm0.00$ \\
%         \hline

        
%     \end{tabular}
%     }
% \end{table*}

\begin{table*}[h]
    \centering
        \caption{Rank Spearman correlation results on \tinyimagenet~dataset with ViT as the model to be explained. The x-axis of the local correlation is the explanation size with hyperparameter top $k$. The global correlation means the rank Spearman correlation of average fidelity. The best performance is marked as bold. For R-Fidelity and F-Fidelity, $\alpha_1=\alpha_2=0.5$. In F-Fidelity, $\beta=0.1$. }
    \label{tab:exp:tinyimagenet:vit}
    \scalebox{1.0}{
     \begin{tabular}{ccccc}
        \hline
          & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
        \hline   
        \makecell*[c]{Local \quad \\Spearman \quad \\ Correlation $\downarrow$ }
        &
        \begin{minipage}[b]{0.18\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/merge/image_finetune_vitmodel_ori_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage}
        &
        \begin{minipage}[b]{0.18\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/merge/image_finetune_vitmodel_road_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage}
        
        & 
        \begin{minipage}[b]{0.18\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/merge/image_finetune_vitmodel_ours_MoRF0.50_LeRF0.50_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage}

        &
        \begin{minipage}[b]{0.18\columnwidth}
		\centering
                \vspace{2pt}
		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/tinyimagenet/merge/image_finetune_vitmodel_ours_MoRF0.50_LeRF0.50_threshold0.10_interv0.2_gradcam_SpearmanCoeff.png}}
	  \end{minipage}        \\

        \\
        \hline
        \multicolumn{5}{c}{Global Spearman Correlation $\downarrow$} \\ 
        \hline
        
        % \makecell*[c]{Global \\ Correlation $\downarrow$ }
        w/o fine-tune & $-0.82\pm0.02$ & $0.89\pm0.07$ & $-\textbf{1.00}\pm0.00$ & $-\textbf{1.00}\pm0.00$ \\
        w/ fine-tune  & $-0.47\pm0.04$ & $0.83\pm0.00$ & $-\textbf{1.00}\pm0.00$ & $-\textbf{1.00}\pm0.00$ \\
        \hline

        
    \end{tabular}
    }
\end{table*}

==> experiments/image/Spearman_correlation_local.tex <==


\begin{table*}[h]
    \centering
    \caption{Local Spearman rank correlation results on \cfar~dataset. We report the total number of top-1 ranks at each sparsity between $5\%$ to $95\%$. The best performance is marked as bold.}
    \label{tab:exp:cfar:local:correlation_rank}
    \scalebox{0.85}{
     \begin{tabular}{ccccccccc}
        \toprule
        Model &
        Top-1 Ranks &
        Fidelity &
        ROAR & 
        R-Fidelity & 
        F-Fidelity \\
        \midrule   
        \multirow{3}{*}{\rotatebox[origin=c]{90}{Res.}} 
        & MoRF vs GT & 0  & 0  & 17  & \textbf{19}\\
        & LeRF vs GT & 14 & 16 & \textbf{19}  & \textbf{19}\\
        & MoRF vs LeRF & 0  & 0  & 17  & \textbf{19}\\
        \hline
        \multirow{3}{*}{\rotatebox[origin=c]{90}{ViT}} 
        & MoRF vs GT & 2   & 1   & 18  & \textbf{19}\\
        & LeRF vs GT & 16  & 16  & \textbf{19}  & \textbf{19}\\
        & MoRF vs LeRF & 1   & 1   & 18  & \textbf{19}\\
        \bottomrule
    \end{tabular}
    }
\end{table*}



\begin{table*}[h]
    \centering
        \caption{Local Spearman rank correlation results on \tinyimagenet~dataset. We report the total number of top-1 ranks at each sparsity between $5\%$ to $95\%$. The best performance is marked as bold. Other settings are the same as Table~\ref{tab:exp:tinyimagenet:global:correlation}}
    \label{tab:exp:cfar:local:correlation_rank}
    \scalebox{0.75}{
     \begin{tabular}{cccccccccc}
        \toprule
        \multirow{2}{*}{Model} &
        \multirow{2}{*}{Top-1 Ranks } &
        \multicolumn{2}{c}{Fidelity} &
        \multicolumn{1}{c}{ROAR} & 
        \multicolumn{2}{c}{R-Fidelity} & 
        \multicolumn{2}{c}{F-Fidelity} \\
        \cmidrule(r){3-4} \cmidrule(r){5-5} \cmidrule(r){6-7} \cmidrule(r){8-9}
        & &  origin  & fine-tune   & retrain  & origin  & fine-tune   & origin  & fine-tune  \\
         \midrule   
        % & \multicolumn{4}{c}{Local Spearman Correlation $\downarrow$} \\ 
        % \hline
        \multirow{3}{*}{\rotatebox[origin=c]{90}{Res.}}
        % \multirow{3}{\rotatebox[origin=c]{90}{Res.}} 
        & MoRF VS GT & 0 & 0 & 0 & 16 & \textbf{19} & 18 & 17\\
        & LeRF VS GT & 18 & 17 & 17 & \textbf{19} & \textbf{19} & \textbf{19} & \textbf{19}\\
        & MoRF VS LeRF & 0 & 0 & 0 & 16 & \textbf{19} & 18 & 17\\
        \hline
        \multirow{3}{*}{\rotatebox[origin=c]{90}{ViT}}
        % \multirow{3}{\rotatebox[origin=c]{90}{ViT}}  \ms{\textbf{1.00}}{0.00}
        & MoRF VS GT  & 0 & 0 & 0 & \textbf{19} & \textbf{19} & 18 & 16 \\
        & LeRF VS GT  & \textbf{19} & \textbf{19} & \textbf{19} & \textbf{19} & \textbf{19} & \textbf{19} & \textbf{19}\\
        & MoRF VS LeRF & 0 & 0 & 0 & \textbf{19} & \textbf{19} & 18 & 16\\
        \bottomrule
    \end{tabular}
    }
\end{table*}


==> experiments/image/spearman_correlation_global.tex <==
\begin{table*}[h]
    \centering
    \caption{Global Spearman rank correlation results on \cfar~dataset which compares the average fidelity of different explanation sizes between $5\%$ to $95\%$. The best performance is marked as bold \ds{bold the number}. }
    \label{tab:exp:cfar:global:correlation}
    \scalebox{0.99}{
     \begin{tabular}{ccccccccc}
        \toprule
        Model &
        Correlation &
        Fidelity &
        ROAR &
        R-Fidelity & 
        F-Fidelity \\
        \midrule   
        \multirow{3}{*}{\rotatebox[origin=c]{90}{Res.}} 
        & MoRF vs GT $\downarrow$ &  \ms{-0.68}{0.08}  &   \ms{-0.66}{0.00}   &\ms{-1.00}{0.00}  &  \ms{-1.00}{0.00}\\
        & LeRF vs GT $\uparrow$ & \ms{1.00}{0.00}      &     \ms{1.00}{0.00}   &\ms{1.00}{0.00}  &   \ms{1.00}{0.00}\\
        & MoRF vs LeRF $\downarrow$ & \ms{-0.68}{0.08} &    \ms{-0.66}{0.00}  &\ms{-1.00}{0.00}  &  \ms{-1.00}{0.00}\\
        \hline
        \multirow{3}{*}{\rotatebox[origin=c]{90}{ViT}} 
        & MoRF vs GT $\downarrow$ &  \ms{-0.94}{0.00}   &     \ms{-0.94}{0.00} &  \ms{-1.00}{0.00} &     \ms{-1.00}{0.00}\\
        & LeRF vs GT $\uparrow$  &    \ms{1.00}{0.00}   &   \ms{1.00}{0.00}  &  \ms{1.00}{0.00}  &    \ms{1.00}{0.00}\\
        & MoRF vs LeRF $\downarrow$ &  \ms{-0.94}{0.08}   &    \ms{-0.94}{0.00} &  \ms{-1.00}{0.00} &     \ms{-1.00}{0.00}\\
        \bottomrule
    \end{tabular}
    }
\end{table*}

\begin{table*}[h]
    \centering
        \caption{Global Spearman rank correlation results on \tinyimagenet~dataset which compares the average fidelity of different explanation size between $5\%$ to $95\%$. The best performance is marked as bold. }
    \label{tab:exp:tinyimagenet:global:correlation}
    \scalebox{0.75}{
     \begin{tabular}{ccccccccccc}
        \toprule
        \multirow{2}{*}{Model} &
        \multirow{2}{*}{Correlation} &
        \multicolumn{2}{c}{Fidelity} &
        \multicolumn{1}{c}{ROAR} &
        \multicolumn{2}{c}{R-Fidelity} & 
        \multicolumn{2}{c}{F-Fidelity} \\
        \cmidrule(r){3-4} \cmidrule(r){5-5} \cmidrule(r){6-7} \cmidrule(r){8-9}
        & &  origin  & fine-tune   & retrain  & origin  & fine-tune   & origin  & fine-tune  \\
        
        % Model & Correlation & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
         \midrule   
        % & \multicolumn{4}{c}{Local Spearman Correlation $\downarrow$} \\ 
        % \hline
        \multirow{3}{*}{\rotatebox[origin=c]{90}{Res.}}
        % \multirow{3}{\rotatebox[origin=c]{90}{Res.}}  \ms{1.00}{0.00}
        & MoRF VS GT $\downarrow$   & \ms{-0.69}{0.07}  & \ms{-0.83}{0.00} & \ms{-0.83}{0.00} & \ms{-1.00}{0.00} & \ms{-1.00}{0.00} & \ms{-1.00}{0.00} & \ms{-1.00}{0.00}\\
        & LeRF VS GT $\uparrow$     & \ms{1.00}{0.00}   & \ms{1.00}{0.00}  & \ms{1.00}{0.00}  & \ms{1.00}{0.00}  & \ms{1.00}{0.00} & \ms{1.00}{0.00} & \ms{1.00}{0.00}\\
        & MoRF VS LeRF $\downarrow$ & \ms{-0.69}{0.07}  & \ms{-0.83}{0.00} & \ms{-0.83}{0.00} & \ms{-1.00}{0.00} & \ms{-1.00}{0.00} & \ms{-1.00}{0.00} & \ms{-1.00}{0.00}\\
        \hline
        \multirow{3}{*}{\rotatebox[origin=c]{90}{ViT}}
        % \multirow{3}{\rotatebox[origin=c]{90}{ViT}}  \ms{\textbf{1.00}}{0.00}
        & MoRF VS GT $\downarrow$   & \ms{-0.82}{0.02}  & \ms{-0.73}{0.08}  & \ms{-0.83}{0.00} & \ms{-1.00}{0.00} & \ms{-1.00}{0.00} & \ms{-1.00}{0.00} & \ms{-1.00}{0.00}\\
        & LeRF VS GT $\uparrow$     & \ms{1.00}{0.00}   & \ms{1.00}{0.00}   & \ms{1.00}{0.00} & \ms{1.00}{0.00}  & \ms{1.00}{0.00} & \ms{1.00}{0.00} & \ms{1.00}{0.00}\\
        & MoRF VS LeRF $\downarrow$ & \ms{-0.82}{0.02}  & \ms{-0.73}{0.08}  & \ms{-0.83}{0.00} & \ms{-1.00}{0.00} & \ms{-1.00}{0.00} & \ms{-1.00}{0.00} & \ms{-1.00}{0.00}\\
        
        \bottomrule
    \end{tabular}
    }
\end{table*}

==> experiments/lstm_local_correlation.tex <==
\begin{table*}[h]
    \centering
        \caption{Local Spearman rank correlation results on PAM and Boiler dataset. We report the total number of top-1 ranks at each sparsity between $5\%$ to $95\%$. The best performance is marked as bold.}
    \label{tab:exp:cfar:local:correlation_rank}
    \scalebox{0.85}{
     \begin{tabular}{cccccccccc}
        \toprule
        \multirow{2}{*}{Model} &
        \multirow{2}{*}{Top-1 Ranks } &
        \multicolumn{2}{c}{Fidelity} &
        \multicolumn{1}{c}{ROAR} &
        \multicolumn{2}{c}{R-Fidelity} & 
        \multicolumn{2}{c}{F-Fidelity} \\
        \cmidrule(r){3-4} \cmidrule(r){5-5} \cmidrule(r){6-7} \cmidrule(r){8-9} 
        & &  origin  & fine-tune  & retrain & origin  & fine-tune  & origin  & fine-tune   \\
         \midrule   
        \multirow{3}{*}{\rotatebox[origin=c]{90}{PAM}}
        & MoRF VS GT  & 13 & 14 & 13 & \textbf{19} & 18 & 17 & 16 \\
        & LeRF VS GT & 6 & 2 & 2 & 16 & \textbf{17} & 16 & 16\\
        & MoRF VS LeRF & 6 & 2 & 2 & \textbf{16} & \textbf{16} & 15 & 14\\
        \hline
        \multirow{3}{*}{\rotatebox[origin=c]{90}{Boiler}}
        & MoRF VS GT  & 0 & 2 & 1 & \textbf{14} & 5 & 11 & 9\\
        & LeRF VS GT  & 4 & 0 & 1 & 5 & \textbf{9} & 4 & 7\\
        & MoRF VS LeRF & 0 & 0 & 0 & 2 & \textbf{16} & 8 & 7\\
        \bottomrule
    \end{tabular}
    }
\end{table*}



==> experiments/sparsity/sparsity.tex <==
\begin{figure}[h]
  \centering
    \subfigure[$\gamma=0.1,\alpha^+ = 0.5$]{\includegraphics[width=0.23\textwidth]{experiments/sparsity/finetune_size0.10_F-Fidelity_alpha0.50_MoRF.png} \hspace{-0.1em}\label{fig:exp:ablation:sparsity10}  }
    \subfigure[$\gamma = 0.15,\alpha^+ = 0.5$]{\includegraphics[width=0.23\textwidth]{experiments/sparsity/finetune_size0.15_F-Fidelity_alpha0.50_MoRF.png} \hspace{-0.1em}\label{fig:exp:ablation:sparsity15}}
    \subfigure[$\gamma = 0.2, \alpha^+ = 0.5$]{\includegraphics[width=0.23\textwidth]{experiments/sparsity/finetune_size0.20_F-Fidelity_alpha0.50_MoRF.png} \hspace{-0.1em}\label{fig:exp:ablation:sparsity20}} 
    \subfigure[$\gamma = 0.25, \alpha^+ = 0.5$]{\includegraphics[width=0.23\textwidth]{experiments/sparsity/finetune_size0.25_F-Fidelity_alpha0.50_MoRF.png} \hspace{-0.1em}\label{fig:exp:ablation:sparsity25}} 
    
    \caption{The relationship between ground truth explanation size $\gamma$ and $FFid^+$ in \ffid.
    %We observe that when the x-axis reaches explanation size, there exists a flat area that indicates the ground truth explanation size. 
    }
    \label{fig:exp:ablation:sparsity}
        \vspace{-0.3cm}
\end{figure}

==> experiments/table_accuracy.tex <==
\begin{table*}[h]
  \centering
    \caption{The accuracy of the models to be explained in the image classification task.}
  \label{exp:tab:image:acc}
  \scalebox{1.00}{
  \begin{tabular}{ccccccc}
  \toprule
         &  \multicolumn{3}{c}{ResNet} &  \multicolumn{3}{c}{ViT} \\
         \cmidrule(r){2-4} \cmidrule(r){5-7}
         Dataset &  origin &  retrain & fine-tune & origin & retrain & fine-tune \\
    \midrule
    \cfar~ &0.7323 & 0.7001 & 0.7310 & 0.5025 & 0.5071 &0.4691 \\   
    \tinyimagenet~ & 0.5585 & 0.5600 & 0.5476  & 0.4255 &0.4262 & 0.3825\\ 
    \bottomrule
  \end{tabular}
}
\end{table*}



\begin{table*}[h]
  \centering
    \caption{The accuracy of the models to be explained in the time series classification task.}
  \label{exp:tab:timeseries:acc}
  \scalebox{1.00}{
  \begin{tabular}{ccccccc}
  \toprule
         &  \multicolumn{3}{c}{LSTM} &  \multicolumn{3}{c}{CNN} \\
         \cmidrule(r){2-4} \cmidrule(r){5-7}
         Dataset &  origin & retrain & fine-tune & origin & retrain & fine-tune \\
    \midrule
    PAM     &0.8989 & 0.8446 & 0.8839 & 0.9433  & 0.9583  & 0.9533 \\   
    Boiler  &0.8014 &0.7889 & 0.7722 & 0.8222  & 0.8264  & 0.8639 \\ 
    \bottomrule
  \end{tabular}
}
\end{table*}


\begin{table*}[h]
  \centering
    \caption{The agreement between the original model and fine-tuned/ROAR model on dataset Cifar-100 and {\tinyimagenet}.}
  \label{exp:tab:timeseries:acc}
  \scalebox{1.00}{
  \begin{tabular}{ccccc}
  \toprule
         &  \multicolumn{2}{c}{Resnet} &  \multicolumn{2}{c}{ViT} \\
         \cmidrule(r){2-3} \cmidrule(r){4-5}
         Dataset & retrain & fine-tune & retrain & fine-tune \\
    \midrule
    Cifar-100        &0.6627 & 0.6619 & 0.4944 & 0.4859 \\   
    {\tinyimagenet}  &0.1223 &0.1263  & 0.4391 & 0.4249 \\ 
    \bottomrule
  \end{tabular}
}
\end{table*}








==> experiments/timagenet/gradcam/resnet_correlation_detail.tex <==
\begin{table*}[h]
    \centering
    \caption{Local Spearman rank correlation results on \tinyimagenet~dataset with ResNet as the model to be explained.}
    \label{tab:exp:tinyimagenet:resnet:local:combined}
    \scalebox{0.6}{
    \begin{tabular}{c|cccc|cccc|cccc}
        \toprule
        & \multicolumn{4}{c|}{MoRF vs GT} & \multicolumn{4}{c|}{LeRF vs GT} & \multicolumn{4}{c}{MoRF vs LeRF} \\
        Sparsity & Fidelity & ROAR & R-Fidelity & F-Fidelity & Fidelity & ROAR & R-Fidelity & F-Fidelity & Fidelity & ROAR & R-Fidelity & F-Fidelity \\
        \midrule
        $5\%$  & \ms{-0.99}{0.01} & \ms{0.76}{0.08} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.02} & \ms{0.94}{0.05} & \ms{-0.64}{0.14}& \ms{0.52}{0.25} & \ms{-0.96}{0.03} & \ms{0.83}{0.11} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00}\\
        $10\%$ & \ms{-0.98}{0.02} & \ms{0.64}{0.02} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{0.97}{0.02} & \ms{0.99}{0.01} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.97}{0.04} & \ms{0.65}{0.01} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00}\\
        $15\%$ & \ms{\textbf{-1.00}}{0.00} & \ms{0.63}{0.03} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{0.98}{0.01} & \ms{0.98}{0.02} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.99}{0.01} & \ms{0.67}{0.09} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00}\\
        $20\%$ & \ms{-0.85}{0.05} & \ms{0.62}{0.03} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{0.99}{0.01} & \ms{0.98}{0.02} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.84}{0.05} & \ms{0.64}{0.04} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00}\\
        $25\%$ & \ms{-0.79}{0.07} & \ms{0.62}{0.02} & \ms{-0.98}{0.02} & \ms{\textbf{-1.00}}{0.00} & \ms{0.99}{0.00} & \ms{0.95}{0.02} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.79}{0.07} & \ms{0.73}{0.08} & \ms{-0.98}{0.02} & \ms{\textbf{-1.00}}{0.00}\\
        $30\%$ & \ms{-0.74}{0.08} & \ms{0.65}{0.07} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.74}{0.08} & \ms{0.65}{0.07} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00}\\
        $35\%$ & \ms{-0.67}{0.08} & \ms{0.61}{0.02} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.67}{0.08} & \ms{0.61}{0.02} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00}\\
        $40\%$ & \ms{-0.62}{0.02} & \ms{0.55}{0.12} & \ms{-0.98}{0.02} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.62}{0.02} & \ms{0.55}{0.12} & \ms{-0.98}{0.02} & \ms{\textbf{-1.00}}{0.00}\\
        $45\%$ & \ms{-0.66}{0.06} & \ms{0.53}{0.04} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{0.98}{0.02} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.66}{0.06} & \ms{0.56}{0.11} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00}\\
        $50\%$ & \ms{-0.62}{0.02} & \ms{0.68}{0.06} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.61}{0.02} & \ms{0.68}{0.06} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00}\\
        $55\%$ & \ms{-0.42}{0.08} & \ms{0.85}{0.08} & \ms{-0.96}{0.03} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.42}{0.08} & \ms{0.85}{0.07} & \ms{-0.96}{0.03} & \ms{\textbf{-1.00}}{0.00}\\
        $60\%$ & \ms{-0.33}{0.30} & \ms{0.80}{0.14} & \ms{-0.95}{0.02} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.33}{0.30} & \ms{0.80}{0.14} & \ms{-0.95}{0.02} & \ms{\textbf{-1.00}}{0.00}\\
        $65\%$ & \ms{0.18}{0.30}  & \ms{0.86}{0.13} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{0.18}{0.30}  & \ms{0.86}{0.13} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00}\\
        $70\%$ & \ms{0.48}{0.29}  & \ms{0.63}{0.38} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{0.48}{0.29}  & \ms{0.63}{0.38} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00}\\
        $75\%$ & \ms{0.46}{0.36}  & \ms{0.40}{0.14} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{0.46}{0.36}  & \ms{0.40}{0.14} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00}\\
        $80\%$ & \ms{0.53}{0.28}  & \ms{0.07}{0.13} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{0.54}{0.28}  & \ms{0.07}{0.13} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00}\\
        $85\%$ & \ms{-0.19}{0.21} & \ms{-0.04}{0.47}& \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.18}{0.21} & \ms{-0.04}{0.48} & \ms{\textbf{-1.00}}{0.00}& \ms{\textbf{-1.00}}{0.00}\\
        $90\%$ & \ms{-0.05}{0.24} & \ms{-0.31}{0.50}& \ms{\textbf{-1.00}}{0.02} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.05}{0.24} & \ms{-0.31}{0.50} & \ms{\textbf{-1.00}}{0.00}& \ms{\textbf{-1.00}}{0.00}\\
        $95\%$ & \ms{-0.74}{0.18} & \ms{0.68}{0.27} & \ms{\textbf{-0.98}}{0.00} & \ms{\textbf{-0.98}}{0.03} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.74}{0.19} & \ms{0.68}{0.27} & \ms{\textbf{-0.98}}{0.02} & \ms{\textbf{-0.98}}{0.03}\\
        \midrule
        Avg. Rank & 3.05 & 3.84 & 1.21 & \textbf{1.00} & 1.47 & 1.58 & 1.58 & \textbf{1.11} & 3.16 & 3.84 & 1.21 & \textbf{1.00} \\
        \bottomrule
    \end{tabular}
    }
\end{table*}

% \begin{table*}[h]
%     \centering
%     \caption{"MoRF VS GT" Local Spearman rank correlation results on \tinyimagenet~dataset with ResNet as the model to be explained.}
%     \label{tab:exp:tinyimagenet:resnet:local:morf_rank}
%     % beta = 1.0
%     \scalebox{0.75}{
%     \begin{tabular}{ccccc}
%         \toprule
%         Sparsity & Fidelity & ROAR & R-Fidelity & F-Fidelity \\
%         \midrule
%         $5\%$  & \ms{-0.87}{0.05} & \ms{-0.81}{0.03} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
%         $10\%$ & \ms{-0.65}{0.03} & \ms{-0.81}{0.03} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $15\%$ & \ms{-0.83}{0.00} & \ms{-0.87}{0.06} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $20\%$ & \ms{-0.83}{0.00} & \ms{-0.87}{0.06} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $25\%$ & \ms{-0.83}{0.00} & \ms{-0.92}{0.05} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $30\%$ & \ms{-0.83}{0.00} & \ms{-0.83}{0.00} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $35\%$ & \ms{-0.73}{0.08} & \ms{-0.83}{0.00} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $40\%$ & \ms{-0.69}{0.07} & \ms{-0.79}{0.07} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $45\%$ & \ms{-0.66}{0.00} & \ms{-0.68}{0.08} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $50\%$ & \ms{-0.66}{0.00} & \ms{-0.65}{0.01} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $55\%$ & \ms{-0.44}{0.03} & \ms{-0.66}{0.00} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $60\%$ & \ms{-0.16}{0.11} & \ms{-0.42}{0.02} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $65\%$ & \ms{-0.07}{0.10} & \ms{-0.34}{0.13} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $70\%$ & \ms{0.14}{0.07}  & \ms{-0.17}{0.11} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $75\%$ & \ms{0.36}{0.10}  & \ms{-0.12}{0.03} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $80\%$ & \ms{0.58}{0.30}  & \ms{0.02}{0.14}  & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $85\%$ & \ms{0.62}{0.35}  & \ms{-0.09}{0.34} & \ms{-0.99}{0.02}          & \ms{\textbf{-1.00}}{0.00} \\
%         $90\%$ & \ms{-0.49}{0.28} & \ms{0.05}{0.29}  & \ms{-0.99}{0.02}          & \ms{\textbf{-1.00}}{0.00} \\
%         $95\%$ & \ms{-0.26}{0.23} & \ms{0.22}{0.35}  & \ms{-0.87}{0.25}          & \ms{\textbf{-1.00}}{0.00} \\
%         \midrule
%         Avg. Rank & 6.26 & 5.95 & 1.42 & \textbf{1.00} \\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table*}

% \begin{table*}[h]
%     \centering
%     \caption{``LeRF VS GT'' Local Spearman rank correlation results on \tinyimagenet~dataset with ResNet as the model to be explained.}
%     \label{tab:exp:tinyimagenet:resnet:local:lerf_rank}
%     \scalebox{0.75}{
%     \begin{tabular}{ccccc}
%         \toprule
%         Sparsity & Fidelity & ROAR & R-Fidelity & F-Fidelity \\
%         \midrule
%         $5\%$  & \ms{\textbf{1.00}}{0.00} & \ms{0.96}{0.02} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $10\%$ & \ms{0.99}{0.02}          & \ms{0.98}{0.03} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $15\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $20\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $25\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $30\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $35\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $40\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $45\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $50\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $55\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $60\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $65\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $70\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $75\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $80\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $85\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $90\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $95\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         \midrule
%         Avg. Rank & 1.21 & 1.63 & \textbf{1.00} & \textbf{1.00} \\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table*}


% \begin{table*}[h]
%     \centering
%     \caption{``MoRF VS LeRF'' Local Spearman rank correlation results on \tinyimagenet~dataset with ResNet as the model to be explained.}
%     \label{tab:exp:tinyimagenet:resnet:local:morf_lerf}
%     \scalebox{0.75}{
%     \begin{tabular}{ccccc}
%         \toprule
%         Sparsity & Fidelity & ROAR & R-Fidelity & F-Fidelity \\
%         \midrule
%         $5\%$  & \ms{-0.87}{0.05} & \ms{-0.77}{0.04} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
%         $10\%$ & \ms{-0.63}{0.03} & \ms{-0.78}{0.02} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $15\%$ & \ms{-0.83}{0.00} & \ms{-0.87}{0.06} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $20\%$ & \ms{-0.83}{0.00} & \ms{-0.87}{0.06} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $25\%$ & \ms{-0.83}{0.00} & \ms{-0.92}{0.05} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $30\%$ & \ms{-0.83}{0.00} & \ms{-0.83}{0.00} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $35\%$ & \ms{-0.73}{0.08} & \ms{-0.83}{0.00} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $40\%$ & \ms{-0.69}{0.07} & \ms{-0.79}{0.07} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $45\%$ & \ms{-0.66}{0.00} & \ms{-0.68}{0.08} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $50\%$ & \ms{-0.66}{0.00} & \ms{-0.65}{0.08} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $55\%$ & \ms{-0.44}{0.03} & \ms{-0.66}{0.00} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $60\%$ & \ms{-0.16}{0.11} & \ms{-0.42}{0.02} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $65\%$ & \ms{-0.07}{0.10} & \ms{-0.34}{0.13} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $70\%$ & \ms{0.14}{0.07}  & \ms{-0.17}{0.11} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $75\%$ & \ms{0.37}{0.10}  & \ms{-0.12}{0.03} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $80\%$ & \ms{0.58}{0.30}  & \ms{0.02}{0.14}  & \ms{\textbf{-1.00}}{0.00}   & \ms{\textbf{-1.00}}{0.00} \\
%         $85\%$ & \ms{0.62}{0.35}  & \ms{-0.09}{0.34} & \ms{-0.99}{0.02}  & \ms{\textbf{-1.00}}{0.00} \\
%         $90\%$ & \ms{-0.49}{0.28} & \ms{0.05}{0.29}  & \ms{-0.99}{0.02}  & \ms{-0.99}{0.02} \\
%         $95\%$ & \ms{-0.26}{0.23} & \ms{0.22}{0.35}  & \ms{-0.87}{0.25}  & \ms{-0.97}{0.07} \\
%         \midrule
%         Avg. Rank & 6.21 & 5.42 & 1.42 & \textbf{1.00} \\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table*}


% % \begin{table*}[h]
% %     \centering
% %         \caption{``MoRF VS GT'' Local Spearman rank correlation results on \tinyimagenet~dataset with Resnet as the model to be explained.}
% %     \label{tab:exp:tinyimagenet:resnet:local:morf_rank}
% %     \scalebox{0.75}{
% %      \begin{tabular}{ccccccccc}
% %         \toprule
% %         &
% %         \multicolumn{2}{c}{Fidelity} &
% %         \multicolumn{1}{c}{ROAR} &
% %         \multicolumn{2}{c}{R-Fidelity} & 
% %         \multicolumn{2}{c}{F-Fidelity} \\
% %         \cmidrule(r){2-3} \cmidrule(r){4-4} \cmidrule(r){5-6} \cmidrule(r){7-8} 
% %         Sparsity &  origin  & fine-tune  & retrain  & origin  & fine-tune  & origin  & fine-tune \\
% %         % Model & Correlation & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
% %          \midrule   
% %         % & \multicolumn{4}{c}{Local Spearman Correlation $\downarrow$} \\ 
% %         % \hline
% %         % \multirow{3}{\rotatebox[origin=c]{90}{ViT}}  \ms{\textbf{1.00}}{0.00}
% %         $5\%$ &  \ms{-0.87}{0.05}&  \ms{-0.94}{0.00} &  \ms{-0.81}{0.03} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         10\% &  \ms{-0.65}{0.03} &  \ms{-0.92}{0.05} &  \ms{-0.81}{0.03} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         15\% &  \ms{-0.83}{0.00} &  \ms{-0.84}{0.03} &  \ms{-0.87}{0.06} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         20\% &  \ms{-0.83}{0.00} &  \ms{-0.83}{0.00} &  \ms{-0.87}{0.06} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         25\% &  \ms{-0.83}{0.00} &  \ms{-0.83}{0.00} &  \ms{-0.92}{0.05} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
        
% %         30\% &  \ms{-0.83}{0.00} &  \ms{-0.83}{0.00} &  \ms{-0.83}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         35\% &  \ms{-0.73}{0.08} &  \ms{-0.79}{0.07} &  \ms{-0.83}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         40\% &  \ms{-0.69}{0.07} &  \ms{-0.68}{0.08} &  \ms{-0.79}{0.07} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         45\% &  \ms{-0.66}{0.00} &  \ms{-0.63}{0.03} &  \ms{-0.68}{0.08} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         50\% &  \ms{-0.66}{0.00} &  \ms{-0.65}{0.02} &  \ms{-0.65}{0.01} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         55\% &  \ms{-0.44}{0.03} &  \ms{-0.44}{0.09} &  \ms{-0.66}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
        
% %         60\% &  \ms{-0.16}{0.11} &  \ms{-0.37}{0.07} &  \ms{-0.42}{0.02} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         65\% &  \ms{-0.07}{0.10} &  \ms{-0.23}{0.22} &  \ms{-0.34}{0.13} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         70\% &  \ms{0.14}{0.07} &  \ms{-0.12}{0.19} &  \ms{-0.17}{0.11}  &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         75\% &  \ms{0.36}{0.10} &  \ms{-0.05}{0.09} &  \ms{-0.12}{0.03}  &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         80\% &  \ms{0.58}{0.30} &  \ms{-0.04}{0.50} &  \ms{0.02}{0.14}   &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         85\% &  \ms{0.62}{0.35} &  \ms{-0.02}{0.40} &  \ms{-0.09}{0.34}  &  \ms{-0.99}{0.02} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
        
% %         90\% &  \ms{-0.49}{0.28} &  \ms{-0.28}{0.32} &  \ms{0.05}{0.29}  &  \ms{-0.99}{0.02} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{-0.99}{0.02}\\
% %         95\% &  \ms{-0.26}{0.23} &  \ms{0.50}{0.37} &  \ms{0.22}{0.35}   &  \ms{-0.87}{0.25} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{-0.99}{0.02}  &  \ms{-0.97}{0.07}\\
% %         \midrule   
% %         Avg. Rank & 6.26 & 5.95 & 5.42 & 1.42 & \textbf{1.00} & 1.05 & 1.21\\
% %         \bottomrule
% %     \end{tabular}
% %     }
% % \end{table*}

% % \begin{table*}[h]
% %     \centering
% %         \caption{``LeRF VS GT'' Local Spearman rank correlation results on \tinyimagenet~dataset with Resnet as the model to be explained.}
% %     \label{tab:exp:tinyimagenet:resnet:local:lerf_rank}
% %     \scalebox{0.75}{
% %      \begin{tabular}{ccccccccc}
% %         \toprule
% %         &
% %         \multicolumn{2}{c}{Fidelity} &
% %         \multicolumn{1}{c}{ROAR} &
% %         \multicolumn{2}{c}{R-Fidelity} & 
% %         \multicolumn{2}{c}{F-Fidelity} \\
% %         \cmidrule(r){2-3} \cmidrule(r){4-4} \cmidrule(r){5-6} \cmidrule(r){7-8} 
% %         Sparsity &  origin  & fine-tune  & retrain  & origin  & fine-tune  & origin  & fine-tune \\
% %         % Model & Correlation & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
% %          \midrule   
% %         % & \multicolumn{4}{c}{Local Spearman Correlation $\downarrow$} \\ 
% %         % \hline
% %         % \multirow{3}{\rotatebox[origin=c]{90}{ViT}}  \ms{\textbf{1.00}}{0.00}
% %         $5\%$ & \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{0.96}{0.02} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00} \\
% %         10\% &  \ms{0.99}{0.02} &  \ms{0.99}{0.02} &  \ms{0.98}{0.03} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}\\
% %         15\% &  \ms{\textbf{1.00}}{0.00} &  \ms{0.99}{0.02} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}\\
% %         20\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}\\
% %         25\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}\\
        
% %         30\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}\\
% %         35\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}\\
% %         40\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}\\
% %         45\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}\\
% %         50\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}\\
% %         55\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}\\
        
% %         60\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}\\
% %         65\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}\\
% %         70\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}\\
% %         75\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}\\
% %         80\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}\\
% %         85\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}\\
        
% %         90\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}\\
% %         95\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}\\
% %         \midrule   
% %         Avg. Rank & 1.21 & 1.53 & 1.63 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00}\\
% %         \bottomrule
% %     \end{tabular}
% %     }
% % \end{table*}


% % \begin{table*}[h]
% %     \centering
% %         \caption{``MoRF VS LeRF'' Local Spearman rank correlation results on \tinyimagenet~dataset  with Resnet as the model to be explained.}
% %     \label{tab:exp:tinyimagenet:resnet:local:morf_lerf}
% %     \scalebox{0.75}{
% %      \begin{tabular}{ccccccccc}
% %         \toprule
% %         &
% %         \multicolumn{2}{c}{Fidelity} &
% %         \multicolumn{1}{c}{ROAR} &
% %         \multicolumn{2}{c}{R-Fidelity} & 
% %         \multicolumn{2}{c}{F-Fidelity} \\
% %         \cmidrule(r){2-3} \cmidrule(r){4-4} \cmidrule(r){5-6} \cmidrule(r){7-8} 
% %         Sparsity &  origin  & fine-tune  & retrain  & origin  & fine-tune  & origin  & fine-tune \\
% %         % Model & Correlation & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
% %          \midrule   
% %         % & \multicolumn{4}{c}{Local Spearman Correlation $\downarrow$} \\ 
% %         % \hline
% %         % \multirow{3}{\rotatebox[origin=c]{90}{ViT}}  \ms{\textbf{1.00}}{0.00}
% %        $5\%$ &  \ms{-0.87}{0.05} &  \ms{-0.94}{0.00} &  \ms{-0.77}{0.04} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         10\% &  \ms{-0.63}{0.03} &  \ms{-0.91}{0.05} &  \ms{-0.78}{0.02} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  \\
% %         15\% &  \ms{-0.83}{0.00} &  \ms{-0.83}{0.03} &  \ms{-0.87}{0.06} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         20\% &  \ms{-0.83}{0.00} &  \ms{-0.83}{0.00} &  \ms{-0.87}{0.06} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         25\% &  \ms{-0.83}{0.00} &  \ms{-0.83}{0.00} &  \ms{-0.92}{0.05} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
        
% %         30\% &  \ms{-0.83}{0.00} &  \ms{-0.83}{0.00} &  \ms{-0.83}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         35\% &  \ms{-0.73}{0.08} &  \ms{-0.79}{0.07} &  \ms{-0.83}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         40\% &  \ms{-0.69}{0.07} &  \ms{-0.68}{0.08} &  \ms{-0.79}{0.07} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         45\% &  \ms{-0.66}{0.00} &  \ms{-0.63}{0.03} &  \ms{-0.68}{0.08} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         50\% &  \ms{-0.66}{0.00} &  \ms{-0.65}{0.02} &  \ms{-0.65}{0.08} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         55\% &  \ms{-0.44}{0.03} &  \ms{-0.44}{0.09} &  \ms{-0.66}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
        
% %         60\% &  \ms{-0.16}{0.11} &  \ms{-0.37}{0.07} &  \ms{-0.42}{0.02} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         65\% &  \ms{-0.07}{0.10} &  \ms{-0.23}{0.22} &  \ms{-0.34}{0.13} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         70\% &  \ms{0.14}{0.07} &  \ms{-0.12}{0.19} &  \ms{-0.17}{0.11} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         75\% &  \ms{0.37}{0.10} &  \ms{-0.05}{0.09} &  \ms{-0.12}{0.03} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         80\% &  \ms{0.58}{0.30} &  \ms{-0.04}{0.50} &  \ms{0.02}{0.14} &  \ms{\textbf{-1.00}}{0.00}   &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         85\% &  \ms{0.62}{0.35} &  \ms{-0.02}{0.40} &  \ms{-0.09}{0.34} &  \ms{-0.99}{0.02}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
        
% %         90\% &  \ms{-0.49}{0.28} &  \ms{-0.28}{0.33} &  \ms{0.05}{0.29} &  \ms{-0.99}{0.02}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{-0.99}{0.02}\\
% %         95\% &  \ms{-0.26}{0.23} &  \ms{0.50}{0.37} &  \ms{0.22}{0.35} &  \ms{-0.87}{0.25}   &  \ms{\textbf{-1.00}}{0.00}  &  \ms{-0.99}{0.02}  &  \ms{-0.97}{0.07}\\
% %         \midrule   
% %         Avg. Rank & 6.21 & 5.95 & 5.42 & 1.42 & \textbf{1.00} & 1.05 & 1.21\\
% %         \bottomrule
% %     \end{tabular}
% %     }
% % \end{table*}



==> experiments/timagenet/gradcam/resnet_fid_images.tex <==
\begin{table*}[h]
    \centering
        \caption{Fidelity results on \tinyimagenet~dataset2 with Resnet as the model to be explained.}
    \label{tab:exp:timagenet:resnet:fid}
    \scalebox{1.0}{
     \begin{tabular}{ccccc}
        \toprule
        & Fidelity & ROAR & R-Fidelity & F-Fidelity \\
        \midrule
        $Fid^+$
        &
        \begin{minipage}[b]{0.20\columnwidth}
        \centering
                \vspace{2pt}
        \raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/timagenet/gradcam/resnet/image_ori_resnet-9-explanations_ori_interv0.2_moRF.png}}
        \end{minipage}
        &
        \begin{minipage}[b]{0.20\columnwidth}
        \centering
                \vspace{2pt}
        \raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/timagenet/gradcam/resnet/image_ori_resnet-9-explanations_roar_interv0.2_moRF.png}}
        \end{minipage}
        &
        \begin{minipage}[b]{0.20\columnwidth}
        \centering
                \vspace{2pt}
        \raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/timagenet/gradcam/resnet/image_ori_resnet-9-explanations_rfid_interv0.2_moRF.png}}
        \end{minipage}
        &
        \begin{minipage}[b]{0.20\columnwidth}
        \centering
                \vspace{2pt}
        \raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/timagenet/gradcam/resnet/image_finetune_resnet-9-finetune-explanations_ffid_interv0.2_moRF.png}}
        \end{minipage}
        \\

        $Fid^-$
        &
        \begin{minipage}[b]{0.20\columnwidth}
        \centering
                \vspace{2pt}
        \raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/timagenet/gradcam/resnet/image_ori_resnet-9-explanations_ori_interv0.2_leRF.png}}
        \end{minipage}
        &
        \begin{minipage}[b]{0.20\columnwidth}
            \centering
            \vspace{2pt}
            \raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/timagenet/gradcam/resnet/image_ori_resnet-9-explanations_roar_interv0.2_leRF.png}}
        \end{minipage}
        &
        % R-Fidelity, Fid^-, origin
        \begin{minipage}[b]{0.20\columnwidth}
            \centering
            \vspace{2pt}
            \raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/timagenet/gradcam/resnet/image_ori_resnet-9-explanations_rfid_interv0.2_leRF.png}}
        \end{minipage}
    &
        \begin{minipage}[b]{0.20\columnwidth}
            \centering
            \vspace{2pt}
            \raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/timagenet/gradcam/resnet/image_finetune_resnet-9-finetune-explanations_ffid_interv0.2_leRF.png}}
        \end{minipage}
        \\
        \bottomrule
    \end{tabular}
    }
\end{table*}















% \begin{table*}[h]
%     \centering
%         \caption{Fidelity results on \tinyimagenet~dataset with Resnet as the model to be explained. }
%     \label{tab:exp:timagenet:resnet:fid}
%     \scalebox{1.0}{
%      \begin{tabular}{ccccc}
%         \toprule
%          & \multicolumn{2}{c}{$Fid^+$} & \multicolumn{2}{c}{$Fid^-$} \\ 
%         \cmidrule(r){2-3} \cmidrule(r){4-5} 
%         Methods &  origin  & retrain/fine-tune  & origin & retrain/fine-tune \\ 
        
%         \midrule 
%         \rotatebox[origin=c]{90}{Fidelity}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/timagenet/resnet/image_ori_resnet-9-explanations_ori_interv0.2_moRF.png}}
% 	  \end{minipage}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/timagenet/resnet/image_finetune_resnet-9-finetune-explanations_ori_interv0.2_moRF.png}}
% 	  \end{minipage}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/timagenet/resnet/image_ori_resnet-9-explanations_ori_interv0.2_leRF.png}}
% 	  \end{minipage}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/timagenet/resnet/image_finetune_resnet-9-finetune-explanations_ori_interv0.2_leRF.png}}
% 	  \end{minipage}
%         \\

%         \rotatebox[origin=c]{90}{ROAR}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/timagenet/resnet/image_ori_resnet-9-explanations_ori_interv0.2_moRF.png}}
% 	  \end{minipage}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/timagenet/resnet/image_ori_resnet-9-explanations_roar_interv0.2_moRF.png}}
% 	  \end{minipage}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/timagenet/resnet/image_ori_resnet-9-explanations_ori_interv0.2_leRF.png}}
% 	  \end{minipage}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/timagenet/resnet/image_ori_resnet-9-explanations_roar_interv0.2_leRF.png}}
% 	  \end{minipage}
%         \\

        
%         \rotatebox[origin=c]{90}{R-Fidelity}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/timagenet/resnet/image_ori_resnet-9-explanations_rfid_interv0.2_moRF.png}}
% 	  \end{minipage}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/timagenet/resnet/image_finetune_resnet-9-finetune-explanations_rfid_interv0.2_moRF.png}}
% 	  \end{minipage}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/timagenet/resnet/image_ori_resnet-9-explanations_rfid_interv0.2_leRF.png}}
% 	  \end{minipage}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/timagenet/resnet/image_finetune_resnet-9-finetune-explanations_rfid_interv0.2_leRF.png}}
% 	  \end{minipage}
%         \\

%         \rotatebox[origin=c]{90}{F-Fidelity}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/timagenet/resnet/image_ori_resnet-9-explanations_ffid_interv0.2_moRF.png}}
% 	  \end{minipage}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/timagenet/resnet/image_finetune_resnet-9-finetune-explanations_ffid_interv0.2_moRF.png}}
% 	  \end{minipage}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/timagenet/resnet/image_ori_resnet-9-explanations_ffid_interv0.2_leRF.png}}
% 	  \end{minipage}
%         &
%         \begin{minipage}[b]{0.20\columnwidth}
% 		\centering
%                 \vspace{2pt}
% 		\raisebox{-.5\height}{\includegraphics[width=\linewidth]{experiments/timagenet/resnet/image_finetune_resnet-9-finetune-explanations_ffid_interv0.2_leRF.png}}
% 	  \end{minipage}
%         \\

%         \bottomrule
        
%     \end{tabular}
%     }
% \end{table*}




==> experiments/timagenet/resnet_correlation_detail.tex <==
\begin{table*}[h]
    \centering
    \caption{Micro Spearman rank correlation results on \tinyimagenet~dataset with ResNet as the model to be explained.}
    \label{tab:exp:tinyimagenet:resnet:local:combined}
    \scalebox{0.6}{
    \begin{tabular}{c|cccc|cccc|cccc}
        \toprule
        & \multicolumn{4}{c|}{MoRF vs GT} & \multicolumn{4}{c|}{LeRF vs GT} & \multicolumn{4}{c}{MoRF vs LeRF} \\
        Sparsity & Fidelity & ROAR & R-Fidelity & F-Fidelity & Fidelity & ROAR & R-Fidelity & F-Fidelity & Fidelity & ROAR & R-Fidelity & F-Fidelity \\
        \midrule
        $5\%$  & \ms{-0.87}{0.05} & \ms{-0.81}{0.03} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{0.96}{0.02} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.87}{0.05} & \ms{-0.77}{0.04} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $10\%$ & \ms{-0.65}{0.03} & \ms{-0.81}{0.03} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} & \ms{0.99}{0.02}          & \ms{0.98}{0.03} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.63}{0.03} & \ms{-0.78}{0.02} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
        $15\%$ & \ms{-0.83}{0.00} & \ms{-0.87}{0.06} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.83}{0.00} & \ms{-0.87}{0.06} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
        $20\%$ & \ms{-0.83}{0.00} & \ms{-0.87}{0.06} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.83}{0.00} & \ms{-0.87}{0.06} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
        $25\%$ & \ms{-0.83}{0.00} & \ms{-0.92}{0.05} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.83}{0.00} & \ms{-0.92}{0.05} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
        $30\%$ & \ms{-0.83}{0.00} & \ms{-0.83}{0.00} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.83}{0.00} & \ms{-0.83}{0.00} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
        $35\%$ & \ms{-0.73}{0.08} & \ms{-0.83}{0.00} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.73}{0.08} & \ms{-0.83}{0.00} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
        $40\%$ & \ms{-0.69}{0.07} & \ms{-0.79}{0.07} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.69}{0.07} & \ms{-0.79}{0.07} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
        $45\%$ & \ms{-0.66}{0.00} & \ms{-0.68}{0.08} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.66}{0.00} & \ms{-0.68}{0.08} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
        $50\%$ & \ms{-0.66}{0.00} & \ms{-0.65}{0.01} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}   & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.66}{0.00} & \ms{-0.65}{0.08} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
        $55\%$ & \ms{-0.44}{0.03} & \ms{-0.66}{0.00} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}   & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} & \ms{-0.44}{0.03} & \ms{-0.66}{0.00} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
        $60\%$ & \ms{-0.16}{0.11} & \ms{-0.42}{0.02} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}   & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} & \ms{-0.16}{0.11} & \ms{-0.42}{0.02} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
        $65\%$ & \ms{-0.07}{0.10} & \ms{-0.34}{0.13} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00}& \ms{\textbf{1.00}}{0.00}   & \ms{\textbf{1.00}}{0.00}   & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} & \ms{-0.07}{0.10} & \ms{-0.34}{0.13} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $70\%$ & \ms{0.14}{0.07}  & \ms{-0.17}{0.11} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00}& \ms{\textbf{1.00}}{0.00}   & \ms{\textbf{1.00}}{0.00}   & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} & \ms{0.14}{0.07}  & \ms{-0.17}{0.11} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $75\%$ & \ms{0.36}{0.10}  & \ms{-0.12}{0.03} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00}& \ms{\textbf{1.00}}{0.00}   & \ms{\textbf{1.00}}{0.00}   & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} & \ms{0.37}{0.10}  & \ms{-0.12}{0.03} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $80\%$ & \ms{0.58}{0.30}  & \ms{0.02}{0.14}  & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00}& \ms{\textbf{1.00}}{0.00}   & \ms{\textbf{1.00}}{0.00}   & \ms{\textbf{1.00}}{0.00}   & \ms{\textbf{1.00}}{0.00} & \ms{0.58}{0.30}  & \ms{0.02}{0.14}  & \ms{\textbf{-1.00}}{0.00}   & \ms{\textbf{-1.00}}{0.00} \\
        $85\%$ & \ms{0.62}{0.35}  & \ms{-0.09}{0.34} & \ms{-0.99}{0.02}          & \ms{\textbf{-1.00}}{0.00}& \ms{\textbf{1.00}}{0.00}   & \ms{\textbf{1.00}}{0.00}   & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} & \ms{0.62}{0.35}  & \ms{-0.09}{0.34} & \ms{-0.99}{0.02}  & \ms{\textbf{-1.00}}{0.00} \\
        $90\%$ & \ms{-0.49}{0.28} & \ms{0.05}{0.29}  & \ms{-0.99}{0.02}          & \ms{\textbf{-1.00}}{0.00}& \ms{\textbf{1.00}}{0.00}   & \ms{\textbf{1.00}}{0.00}   & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} & \ms{-0.49}{0.28} & \ms{0.05}{0.29}  & \ms{-0.99}{0.02}  & \ms{-0.99}{0.02} \\
        $95\%$ & \ms{-0.26}{0.23} & \ms{0.22}{0.35}  & \ms{-0.87}{0.25}          & \ms{\textbf{-1.00}}{0.00}& \ms{\textbf{1.00}}{0.00}   & \ms{\textbf{1.00}}{0.00}   & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00} & \ms{-0.26}{0.23} & \ms{0.22}{0.35}  & \ms{-0.87}{0.25}  & \ms{-0.97}{0.07} \\
        \midrule
        Avg. Rank & 2.89 & 2.37 & 1.16 & \textbf{1.00} & 1.05 & 1.16 & \textbf{1.00} & \textbf{1.00} & 2.84 & 2.32 & 1.11 & \textbf{1.00} \\
        \bottomrule
    \end{tabular}
    }
\end{table*}

% \begin{table*}[h]
%     \centering
%     \caption{"MoRF VS GT" Local Spearman rank correlation results on \tinyimagenet~dataset with ResNet as the model to be explained.}
%     \label{tab:exp:tinyimagenet:resnet:local:morf_rank}
%     % beta = 1.0
%     \scalebox{0.75}{
%     \begin{tabular}{ccccc}
%         \toprule
%         Sparsity & Fidelity & ROAR & R-Fidelity & F-Fidelity \\
%         \midrule
%         $5\%$  & \ms{-0.87}{0.05} & \ms{-0.81}{0.03} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
%         $10\%$ & \ms{-0.65}{0.03} & \ms{-0.81}{0.03} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $15\%$ & \ms{-0.83}{0.00} & \ms{-0.87}{0.06} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $20\%$ & \ms{-0.83}{0.00} & \ms{-0.87}{0.06} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $25\%$ & \ms{-0.83}{0.00} & \ms{-0.92}{0.05} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $30\%$ & \ms{-0.83}{0.00} & \ms{-0.83}{0.00} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $35\%$ & \ms{-0.73}{0.08} & \ms{-0.83}{0.00} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $40\%$ & \ms{-0.69}{0.07} & \ms{-0.79}{0.07} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $45\%$ & \ms{-0.66}{0.00} & \ms{-0.68}{0.08} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $50\%$ & \ms{-0.66}{0.00} & \ms{-0.65}{0.01} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $55\%$ & \ms{-0.44}{0.03} & \ms{-0.66}{0.00} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $60\%$ & \ms{-0.16}{0.11} & \ms{-0.42}{0.02} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $65\%$ & \ms{-0.07}{0.10} & \ms{-0.34}{0.13} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $70\%$ & \ms{0.14}{0.07}  & \ms{-0.17}{0.11} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $75\%$ & \ms{0.36}{0.10}  & \ms{-0.12}{0.03} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $80\%$ & \ms{0.58}{0.30}  & \ms{0.02}{0.14}  & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $85\%$ & \ms{0.62}{0.35}  & \ms{-0.09}{0.34} & \ms{-0.99}{0.02}          & \ms{\textbf{-1.00}}{0.00} \\
%         $90\%$ & \ms{-0.49}{0.28} & \ms{0.05}{0.29}  & \ms{-0.99}{0.02}          & \ms{\textbf{-1.00}}{0.00} \\
%         $95\%$ & \ms{-0.26}{0.23} & \ms{0.22}{0.35}  & \ms{-0.87}{0.25}          & \ms{\textbf{-1.00}}{0.00} \\
%         \midrule
%         Avg. Rank & 6.26 & 5.95 & 1.42 & \textbf{1.00} \\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table*}

% \begin{table*}[h]
%     \centering
%     \caption{``LeRF VS GT'' Local Spearman rank correlation results on \tinyimagenet~dataset with ResNet as the model to be explained.}
%     \label{tab:exp:tinyimagenet:resnet:local:lerf_rank}
%     \scalebox{0.75}{
%     \begin{tabular}{ccccc}
%         \toprule
%         Sparsity & Fidelity & ROAR & R-Fidelity & F-Fidelity \\
%         \midrule
%         $5\%$  & \ms{\textbf{1.00}}{0.00} & \ms{0.96}{0.02} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $10\%$ & \ms{0.99}{0.02}          & \ms{0.98}{0.03} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $15\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $20\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $25\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $30\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $35\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $40\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $45\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $50\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $55\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $60\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $65\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $70\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $75\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $80\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $85\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $90\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         $95\%$ & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} \\
%         \midrule
%         Avg. Rank & 1.21 & 1.63 & \textbf{1.00} & \textbf{1.00} \\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table*}


% \begin{table*}[h]
%     \centering
%     \caption{``MoRF VS LeRF'' Local Spearman rank correlation results on \tinyimagenet~dataset with ResNet as the model to be explained.}
%     \label{tab:exp:tinyimagenet:resnet:local:morf_lerf}
%     \scalebox{0.75}{
%     \begin{tabular}{ccccc}
%         \toprule
%         Sparsity & Fidelity & ROAR & R-Fidelity & F-Fidelity \\
%         \midrule
%         $5\%$  & \ms{-0.87}{0.05} & \ms{-0.77}{0.04} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
%         $10\%$ & \ms{-0.63}{0.03} & \ms{-0.78}{0.02} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $15\%$ & \ms{-0.83}{0.00} & \ms{-0.87}{0.06} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $20\%$ & \ms{-0.83}{0.00} & \ms{-0.87}{0.06} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $25\%$ & \ms{-0.83}{0.00} & \ms{-0.92}{0.05} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $30\%$ & \ms{-0.83}{0.00} & \ms{-0.83}{0.00} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $35\%$ & \ms{-0.73}{0.08} & \ms{-0.83}{0.00} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $40\%$ & \ms{-0.69}{0.07} & \ms{-0.79}{0.07} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $45\%$ & \ms{-0.66}{0.00} & \ms{-0.68}{0.08} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $50\%$ & \ms{-0.66}{0.00} & \ms{-0.65}{0.08} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $55\%$ & \ms{-0.44}{0.03} & \ms{-0.66}{0.00} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $60\%$ & \ms{-0.16}{0.11} & \ms{-0.42}{0.02} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $65\%$ & \ms{-0.07}{0.10} & \ms{-0.34}{0.13} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $70\%$ & \ms{0.14}{0.07}  & \ms{-0.17}{0.11} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $75\%$ & \ms{0.37}{0.10}  & \ms{-0.12}{0.03} & \ms{\textbf{-1.00}}{0.00}  & \ms{\textbf{-1.00}}{0.00} \\
%         $80\%$ & \ms{0.58}{0.30}  & \ms{0.02}{0.14}  & \ms{\textbf{-1.00}}{0.00}   & \ms{\textbf{-1.00}}{0.00} \\
%         $85\%$ & \ms{0.62}{0.35}  & \ms{-0.09}{0.34} & \ms{-0.99}{0.02}  & \ms{\textbf{-1.00}}{0.00} \\
%         $90\%$ & \ms{-0.49}{0.28} & \ms{0.05}{0.29}  & \ms{-0.99}{0.02}  & \ms{-0.99}{0.02} \\
%         $95\%$ & \ms{-0.26}{0.23} & \ms{0.22}{0.35}  & \ms{-0.87}{0.25}  & \ms{-0.97}{0.07} \\
%         \midrule
%         Avg. Rank & 6.21 & 5.42 & 1.42 & \textbf{1.00} \\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table*}


% % \begin{table*}[h]
% %     \centering
% %         \caption{``MoRF VS GT'' Local Spearman rank correlation results on \tinyimagenet~dataset with Resnet as the model to be explained.}
% %     \label{tab:exp:tinyimagenet:resnet:local:morf_rank}
% %     \scalebox{0.75}{
% %      \begin{tabular}{ccccccccc}
% %         \toprule
% %         &
% %         \multicolumn{2}{c}{Fidelity} &
% %         \multicolumn{1}{c}{ROAR} &
% %         \multicolumn{2}{c}{R-Fidelity} & 
% %         \multicolumn{2}{c}{F-Fidelity} \\
% %         \cmidrule(r){2-3} \cmidrule(r){4-4} \cmidrule(r){5-6} \cmidrule(r){7-8} 
% %         Sparsity &  origin  & fine-tune  & retrain  & origin  & fine-tune  & origin  & fine-tune \\
% %         % Model & Correlation & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
% %          \midrule   
% %         % & \multicolumn{4}{c}{Local Spearman Correlation $\downarrow$} \\ 
% %         % \hline
% %         % \multirow{3}{\rotatebox[origin=c]{90}{ViT}}  \ms{\textbf{1.00}}{0.00}
% %         $5\%$ &  \ms{-0.87}{0.05}&  \ms{-0.94}{0.00} &  \ms{-0.81}{0.03} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         10\% &  \ms{-0.65}{0.03} &  \ms{-0.92}{0.05} &  \ms{-0.81}{0.03} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         15\% &  \ms{-0.83}{0.00} &  \ms{-0.84}{0.03} &  \ms{-0.87}{0.06} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         20\% &  \ms{-0.83}{0.00} &  \ms{-0.83}{0.00} &  \ms{-0.87}{0.06} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         25\% &  \ms{-0.83}{0.00} &  \ms{-0.83}{0.00} &  \ms{-0.92}{0.05} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
        
% %         30\% &  \ms{-0.83}{0.00} &  \ms{-0.83}{0.00} &  \ms{-0.83}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         35\% &  \ms{-0.73}{0.08} &  \ms{-0.79}{0.07} &  \ms{-0.83}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         40\% &  \ms{-0.69}{0.07} &  \ms{-0.68}{0.08} &  \ms{-0.79}{0.07} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         45\% &  \ms{-0.66}{0.00} &  \ms{-0.63}{0.03} &  \ms{-0.68}{0.08} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         50\% &  \ms{-0.66}{0.00} &  \ms{-0.65}{0.02} &  \ms{-0.65}{0.01} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         55\% &  \ms{-0.44}{0.03} &  \ms{-0.44}{0.09} &  \ms{-0.66}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
        
% %         60\% &  \ms{-0.16}{0.11} &  \ms{-0.37}{0.07} &  \ms{-0.42}{0.02} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         65\% &  \ms{-0.07}{0.10} &  \ms{-0.23}{0.22} &  \ms{-0.34}{0.13} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         70\% &  \ms{0.14}{0.07} &  \ms{-0.12}{0.19} &  \ms{-0.17}{0.11}  &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         75\% &  \ms{0.36}{0.10} &  \ms{-0.05}{0.09} &  \ms{-0.12}{0.03}  &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         80\% &  \ms{0.58}{0.30} &  \ms{-0.04}{0.50} &  \ms{0.02}{0.14}   &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         85\% &  \ms{0.62}{0.35} &  \ms{-0.02}{0.40} &  \ms{-0.09}{0.34}  &  \ms{-0.99}{0.02} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
        
% %         90\% &  \ms{-0.49}{0.28} &  \ms{-0.28}{0.32} &  \ms{0.05}{0.29}  &  \ms{-0.99}{0.02} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{-0.99}{0.02}\\
% %         95\% &  \ms{-0.26}{0.23} &  \ms{0.50}{0.37} &  \ms{0.22}{0.35}   &  \ms{-0.87}{0.25} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{-0.99}{0.02}  &  \ms{-0.97}{0.07}\\
% %         \midrule   
% %         Avg. Rank & 6.26 & 5.95 & 5.42 & 1.42 & \textbf{1.00} & 1.05 & 1.21\\
% %         \bottomrule
% %     \end{tabular}
% %     }
% % \end{table*}

% % \begin{table*}[h]
% %     \centering
% %         \caption{``LeRF VS GT'' Local Spearman rank correlation results on \tinyimagenet~dataset with Resnet as the model to be explained.}
% %     \label{tab:exp:tinyimagenet:resnet:local:lerf_rank}
% %     \scalebox{0.75}{
% %      \begin{tabular}{ccccccccc}
% %         \toprule
% %         &
% %         \multicolumn{2}{c}{Fidelity} &
% %         \multicolumn{1}{c}{ROAR} &
% %         \multicolumn{2}{c}{R-Fidelity} & 
% %         \multicolumn{2}{c}{F-Fidelity} \\
% %         \cmidrule(r){2-3} \cmidrule(r){4-4} \cmidrule(r){5-6} \cmidrule(r){7-8} 
% %         Sparsity &  origin  & fine-tune  & retrain  & origin  & fine-tune  & origin  & fine-tune \\
% %         % Model & Correlation & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
% %          \midrule   
% %         % & \multicolumn{4}{c}{Local Spearman Correlation $\downarrow$} \\ 
% %         % \hline
% %         % \multirow{3}{\rotatebox[origin=c]{90}{ViT}}  \ms{\textbf{1.00}}{0.00}
% %         $5\%$ & \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{0.96}{0.02} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00} \\
% %         10\% &  \ms{0.99}{0.02} &  \ms{0.99}{0.02} &  \ms{0.98}{0.03} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}\\
% %         15\% &  \ms{\textbf{1.00}}{0.00} &  \ms{0.99}{0.02} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}\\
% %         20\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}\\
% %         25\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}\\
        
% %         30\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}\\
% %         35\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}\\
% %         40\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}\\
% %         45\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}\\
% %         50\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}\\
% %         55\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}\\
        
% %         60\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}\\
% %         65\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}\\
% %         70\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}\\
% %         75\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}\\
% %         80\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}\\
% %         85\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}\\
        
% %         90\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}\\
% %         95\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}  &  \ms{\textbf{1.00}}{0.00}\\
% %         \midrule   
% %         Avg. Rank & 1.21 & 1.53 & 1.63 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00}\\
% %         \bottomrule
% %     \end{tabular}
% %     }
% % \end{table*}


% % \begin{table*}[h]
% %     \centering
% %         \caption{``MoRF VS LeRF'' Local Spearman rank correlation results on \tinyimagenet~dataset  with Resnet as the model to be explained.}
% %     \label{tab:exp:tinyimagenet:resnet:local:morf_lerf}
% %     \scalebox{0.75}{
% %      \begin{tabular}{ccccccccc}
% %         \toprule
% %         &
% %         \multicolumn{2}{c}{Fidelity} &
% %         \multicolumn{1}{c}{ROAR} &
% %         \multicolumn{2}{c}{R-Fidelity} & 
% %         \multicolumn{2}{c}{F-Fidelity} \\
% %         \cmidrule(r){2-3} \cmidrule(r){4-4} \cmidrule(r){5-6} \cmidrule(r){7-8} 
% %         Sparsity &  origin  & fine-tune  & retrain  & origin  & fine-tune  & origin  & fine-tune \\
% %         % Model & Correlation & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
% %          \midrule   
% %         % & \multicolumn{4}{c}{Local Spearman Correlation $\downarrow$} \\ 
% %         % \hline
% %         % \multirow{3}{\rotatebox[origin=c]{90}{ViT}}  \ms{\textbf{1.00}}{0.00}
% %        $5\%$ &  \ms{-0.87}{0.05} &  \ms{-0.94}{0.00} &  \ms{-0.77}{0.04} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         10\% &  \ms{-0.63}{0.03} &  \ms{-0.91}{0.05} &  \ms{-0.78}{0.02} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  \\
% %         15\% &  \ms{-0.83}{0.00} &  \ms{-0.83}{0.03} &  \ms{-0.87}{0.06} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         20\% &  \ms{-0.83}{0.00} &  \ms{-0.83}{0.00} &  \ms{-0.87}{0.06} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         25\% &  \ms{-0.83}{0.00} &  \ms{-0.83}{0.00} &  \ms{-0.92}{0.05} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
        
% %         30\% &  \ms{-0.83}{0.00} &  \ms{-0.83}{0.00} &  \ms{-0.83}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         35\% &  \ms{-0.73}{0.08} &  \ms{-0.79}{0.07} &  \ms{-0.83}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         40\% &  \ms{-0.69}{0.07} &  \ms{-0.68}{0.08} &  \ms{-0.79}{0.07} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         45\% &  \ms{-0.66}{0.00} &  \ms{-0.63}{0.03} &  \ms{-0.68}{0.08} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         50\% &  \ms{-0.66}{0.00} &  \ms{-0.65}{0.02} &  \ms{-0.65}{0.08} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         55\% &  \ms{-0.44}{0.03} &  \ms{-0.44}{0.09} &  \ms{-0.66}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
        
% %         60\% &  \ms{-0.16}{0.11} &  \ms{-0.37}{0.07} &  \ms{-0.42}{0.02} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         65\% &  \ms{-0.07}{0.10} &  \ms{-0.23}{0.22} &  \ms{-0.34}{0.13} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         70\% &  \ms{0.14}{0.07} &  \ms{-0.12}{0.19} &  \ms{-0.17}{0.11} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         75\% &  \ms{0.37}{0.10} &  \ms{-0.05}{0.09} &  \ms{-0.12}{0.03} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         80\% &  \ms{0.58}{0.30} &  \ms{-0.04}{0.50} &  \ms{0.02}{0.14} &  \ms{\textbf{-1.00}}{0.00}   &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
% %         85\% &  \ms{0.62}{0.35} &  \ms{-0.02}{0.40} &  \ms{-0.09}{0.34} &  \ms{-0.99}{0.02}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}\\
        
% %         90\% &  \ms{-0.49}{0.28} &  \ms{-0.28}{0.33} &  \ms{0.05}{0.29} &  \ms{-0.99}{0.02}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00}  &  \ms{-0.99}{0.02}\\
% %         95\% &  \ms{-0.26}{0.23} &  \ms{0.50}{0.37} &  \ms{0.22}{0.35} &  \ms{-0.87}{0.25}   &  \ms{\textbf{-1.00}}{0.00}  &  \ms{-0.99}{0.02}  &  \ms{-0.97}{0.07}\\
% %         \midrule   
% %         Avg. Rank & 6.21 & 5.95 & 5.42 & 1.42 & \textbf{1.00} & 1.05 & 1.21\\
% %         \bottomrule
% %     \end{tabular}
% %     }
% % \end{table*}



==> experiments/timagenet/spearman_correlation_local.tex <==
% \begin{table*}[h]
%     \centering
%         \caption{Global Spearman rank correlation results on {\tinyimagenet} dataset with ViT. }
%     \label{tab:exp:tinyimagenet:vit:correlation}
%     \scalebox{0.75}{
%      \begin{tabular}{cccccc|cccc}
%         \toprule
%         \multirow{2}{*}{} &
%         \multirow{2}{*}{Correlation} &
%         \multicolumn{4}{c}{SG-SQ} &
%         \multicolumn{4}{c}{GradCam} \\
%         \cmidrule(r){3-6} \cmidrule(r){7-10}
%         & & 
%         Fidelity &
%         ROAR &
%         R-Fidelity & 
%         F-Fidelity & Fidelity &
%         ROAR &
%         R-Fidelity & 
%         F-Fidelity\\
%          \midrule   
%         \multirow{3}{*}{\rotatebox[origin=c]{90}{\shortstack{Macro \\ Corr.}}}
%         & MoRF vs GT $\downarrow$ & \ms{-0.82}{0.02}  & \ms{-0.83}{0.00} & \ms{-1.00}{0.00} & \ms{-1.00}{0.00} & ... & ... & ... & ...\\
%         & LeRF vs GT $\uparrow$    & \ms{1.00}{0.00}   & \ms{1.00}{0.00}  & \ms{1.00}{0.00} & \ms{1.00}{0.00} & ... & ... & ... & ... \\
%         & MoRF vs LeRF $\downarrow$ & \ms{-0.82}{0.02}  & \ms{-0.83}{0.00} & \ms{-1.00}{0.00} & \ms{-1.00}{0.00} & ... & ... & ... & ... \\
%         \midrule
%         \multirow{3}{*}{\rotatebox[origin=c]{90}{\shortstack{Micro \\ Corr.}}}
%         & MoRF vs GT $\downarrow$ & \\
%         & LeRF vs GT $\uparrow$   & \\
%         & MoRF vs LeRF $\downarrow$&\\
%         \midrule
%         \multirow{3}{*}{\rotatebox[origin=c]{90}{\shortstack{Micro \\ Rank}}}
%         & MoRF vs GT $\downarrow$ & \\
%         & LeRF vs GT  $\downarrow$& \\
%         & MoRF vs LeRF$\downarrow$& \\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table*}



% \begin{table*}[h]
%     \centering
%         \caption{Local Spearman rank correlation results on \tinyimagenet~dataset. We report the total number of top-1 ranks at each sparsity between $5\%$ to $95\%$. The best performance is marked as bold. Other settings are the same as Table~\ref{tab:exp:tinyimagenet:global:correlation}.}
%     \label{tab:exp:tinyimagenet:local:correlation_rank}
%     \scalebox{0.75}{
%      \begin{tabular}{cccccc|cccc}
%         \toprule
%         \multirow{2}{*}{Backbone} &
%         \multirow{2}{*}{Top-1 Ranks} &
%         \multicolumn{4}{c}{SG-SQ} &
%         \multicolumn{4}{c}{GradCam} \\
%         \cmidrule(r){3-6} \cmidrule(r){7-10}
%         & & 
%         Fidelity &
%         ROAR &
%         R-Fidelity & 
%         F-Fidelity &
%         Fidelity &
%         ROAR &
%         R-Fidelity & 
%         F-Fidelity \\
%          \midrule   
%         \multirow{3}{*}{\rotatebox[origin=c]{90}{Res.}}
%         & MoRF vs GT & 0 & 0 & 16 & \textbf{19} & ... & ... & ... & ... \\
%         & LeRF vs GT & 18 & 17 & \textbf{19} & \textbf{19} & ... & ... & ... & ... \\
%         & MoRF vs LeRF & 0 & 0 & 16 & \textbf{19} & ... & ... & ... & ... \\
%         \hline
%         \multirow{3}{*}{\rotatebox[origin=c]{90}{ViT}}
%         & MoRF vs GT  & 0 & 0 & \textbf{19} & \textbf{19} & ... & ... & ... & ... \\
%         & LeRF vs GT  & \textbf{19} & \textbf{19} & \textbf{19} & \textbf{19} & ... & ... & ... & ... \\
%         & MoRF vs LeRF & 0 & 0 & \textbf{19} & \textbf{19} & ... & ... & ... & ... \\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table*}


% \begin{table*}[h]
%     \centering
%         \caption{Local Spearman rank correlation results on \tinyimagenet~dataset. We report the total number of top-1 ranks at each sparsity between $5\%$ to $95\%$. The best performance is marked as bold. Other settings are the same as Table~\ref{tab:exp:tinyimagenet:global:correlation}}
%     \label{tab:exp:cfar:local:correlation_rank}
%     \scalebox{0.75}{
%      \begin{tabular}{cccccccccc}
%         \toprule
%         \multirow{2}{*}{Model} &
%         \multirow{2}{*}{Top-1 Ranks } &
%         \multicolumn{2}{c}{Fidelity} &
%         \multicolumn{1}{c}{ROAR} & 
%         \multicolumn{2}{c}{R-Fidelity} & 
%         \multicolumn{2}{c}{F-Fidelity} \\
%         \cmidrule(r){3-4} \cmidrule(r){5-5} \cmidrule(r){6-7} \cmidrule(r){8-9}
%         & &  origin  & fine-tune   & retrain  & origin  & fine-tune   & origin  & fine-tune  \\
%          \midrule   
%         % & \multicolumn{4}{c}{Local Spearman Correlation $\downarrow$} \\ 
%         % \hline
%         \multirow{3}{*}{\rotatebox[origin=c]{90}{Res.}}
%         % \multirow{3}{\rotatebox[origin=c]{90}{Res.}} 
%         & MoRF VS GT & 0 & 0 & 0 & 16 & \textbf{19} & 18 & 17\\
%         & LeRF VS GT & 18 & 17 & 17 & \textbf{19} & \textbf{19} & \textbf{19} & \textbf{19}\\
%         & MoRF VS LeRF & 0 & 0 & 0 & 16 & \textbf{19} & 18 & 17\\
%         \hline
%         \multirow{3}{*}{\rotatebox[origin=c]{90}{ViT}}
%         % \multirow{3}{\rotatebox[origin=c]{90}{ViT}}  \ms{\textbf{1.00}}{0.00}
%         & MoRF VS GT  & 0 & 0 & 0 & \textbf{19} & \textbf{19} & 18 & 16 \\
%         & LeRF VS GT  & \textbf{19} & \textbf{19} & \textbf{19} & \textbf{19} & \textbf{19} & \textbf{19} & \textbf{19}\\
%         & MoRF VS LeRF & 0 & 0 & 0 & \textbf{19} & \textbf{19} & 18 & 16\\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table*}



==> experiments/timagenet/vit_correlation_detail.tex <==
\begin{table*}[h]
    \centering
    \caption{Micro Spearman rank correlation results on \tinyimagenet~dataset with ViT as the model to be explained.}
    \label{tab:exp:tinyimagenet:vit:local:combined}
    \scalebox{0.6}{
     \begin{tabular}{c|cccc|cccc|cccc}
        \toprule
        & \multicolumn{4}{c|}{MoRF vs GT} & \multicolumn{4}{c|}{LeRF vs GT} & \multicolumn{4}{c}{MoRF vs LeRF} \\
        Sparsity & Fidelity & ROAR & R-Fidelity & F-Fidelity & Fidelity & ROAR & R-Fidelity & F-Fidelity & Fidelity & ROAR & R-Fidelity & F-Fidelity \\
        \midrule   
        $5\%$ & \ms{-0.83}{0.00} & \ms{-0.81}{0.03} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.83}{0.00} & \ms{-0.81}{0.03} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $10\%$ & \ms{-0.83}{0.00} & \ms{-0.79}{0.03} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.83}{0.00} & \ms{-0.79}{0.03} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $15\%$ & \ms{-0.82}{0.02} & \ms{-0.63}{0.03} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.82}{0.02} & \ms{-0.63}{0.03} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $20\%$ & \ms{-0.76}{0.06} & \ms{-0.61}{0.02} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.76}{0.06} & \ms{-0.61}{0.02} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $25\%$ & \ms{-0.74}{0.07} & \ms{-0.65}{0.02} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.74}{0.07} & \ms{-0.65}{0.02} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $30\%$ & \ms{-0.83}{0.00} & \ms{-0.67}{0.08} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.83}{0.00} & \ms{-0.67}{0.08} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $35\%$ & \ms{-0.81}{0.03} & \ms{-0.71}{0.10} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.81}{0.03} & \ms{-0.71}{0.10} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $40\%$ & \ms{-0.84}{0.06} & \ms{-0.83}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.84}{0.06} & \ms{-0.83}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $45\%$ & \ms{-0.83}{0.00} & \ms{-0.83}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.83}{0.00} & \ms{-0.83}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $50\%$ & \ms{-0.83}{0.00} & \ms{-0.83}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.83}{0.00} & \ms{-0.83}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $55\%$ & \ms{-0.90}{0.06} & \ms{-0.87}{0.06} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.90}{0.06} & \ms{-0.87}{0.06} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $60\%$ & \ms{-0.90}{0.06} & \ms{-0.92}{0.05} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.90}{0.06} & \ms{-0.92}{0.05} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $65\%$ & \ms{-0.80}{0.03} & \ms{-0.78}{0.09} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.80}{0.03} & \ms{-0.78}{0.09} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $70\%$ & \ms{-0.94}{0.04} & \ms{-0.70}{0.06} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.94}{0.04} & \ms{-0.70}{0.06} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $75\%$ & \ms{-0.79}{0.11} & \ms{-0.75}{0.09} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.79}{0.11} & \ms{-0.75}{0.09} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $80\%$ & \ms{-0.72}{0.15} & \ms{-0.95}{0.25} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.72}{0.15} & \ms{-0.95}{0.25} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $85\%$ & \ms{-0.65}{0.24} & \ms{-0.66}{0.21} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.65}{0.24} & \ms{-0.66}{0.21} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $90\%$ & \ms{-0.48}{0.24} & \ms{-0.71}{0.17} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{\textbf{1.00}}{0.00} & \ms{-0.48}{0.24} & \ms{-0.71}{0.17} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        $95\%$ & \ms{0.32}{0.21} & \ms{-0.70}{0.09} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}  & \ms{\textbf{1.00}}{0.00}   & \ms{\textbf{1.00}}{0.00} & \ms{0.32}{0.21}  & \ms{-0.70}{0.09} & \ms{\textbf{-1.00}}{0.00} & \ms{\textbf{-1.00}}{0.00} \\
        \midrule   
        Avg. Rank & 2.26 & 2.63 & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & 2.26 & 2.63 & \textbf{1.00} & \textbf{1.00} \\
        \bottomrule
    \end{tabular}
    }
\end{table*}

% \begin{table*}[h]
%     \centering
%     \caption{``MoRF VS GT'' Local Spearman rank correlation results on \tinyimagenet~dataset with ViT as the model to be explained.}
%     \label{tab:exp:tinyimagenet:vit:local:morf_rank}
%     \scalebox{0.75}{
%      \begin{tabular}{ccccc}
%         \toprule
%         Sparsity &
%         Fidelity &
%         ROAR &
%         R-Fidelity & 
%         F-Fidelity \\
%         \midrule   
%         $5\%$ & \ms{-0.83}{0.00} &  \ms{-0.81}{0.03} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} \\
%         10\% &  \ms{-0.83}{0.00} &  \ms{-0.79}{0.03} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} \\
%         15\% &  \ms{-0.82}{0.02} &  \ms{-0.63}{0.03} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} \\
%         20\% &  \ms{-0.76}{0.06} &  \ms{-0.61}{0.02} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} \\
%         25\% &  \ms{-0.74}{0.07} &  \ms{-0.65}{0.02} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} \\
%         30\% &  \ms{-0.83}{0.00} &  \ms{-0.67}{0.08} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} \\
%         35\% &  \ms{-0.81}{0.03} &  \ms{-0.71}{0.10} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} \\
%         40\% &  \ms{-0.84}{0.06} &  \ms{-0.83}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} \\
%         45\% &  \ms{-0.83}{0.00} &  \ms{-0.83}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} \\
%         50\% &  \ms{-0.83}{0.00} &  \ms{-0.83}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} \\
%         55\% &  \ms{-0.90}{0.06} &  \ms{-0.87}{0.06} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} \\
%         60\% &  \ms{-0.90}{0.06} &  \ms{-0.92}{0.05} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} \\
%         65\% &  \ms{-0.80}{0.03} &  \ms{-0.78}{0.09} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} \\
%         70\% & \ms{-0.94}{0.04} &  \ms{-0.70}{0.06} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} \\
%         75\% & \ms{-0.79}{0.11} &  \ms{-0.75}{0.09} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} \\
%         80\% & \ms{-0.72}{0.15} &  \ms{-0.95}{0.25} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} \\
%         85\% & \ms{-0.65}{0.24} &  \ms{-0.66}{0.21} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} \\
%         90\% &  \ms{-0.48}{0.24} &  \ms{-0.71}{0.17} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} \\
%         95\% & \ms{0.32}{0.21} &  \ms{-0.70}{0.09} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} \\ 
%         \midrule   
%         Avg. Rank & 5.37 & 5.95 & \textbf{1.00} & \textbf{1.00} \\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table*}

% \begin{table*}[h]
%     \centering
%     \caption{``LeRF VS GT'' Local Spearman rank correlation results on \tinyimagenet~dataset with ViT as the model to be explained.}
%     \label{tab:exp:tinyimagenet:vit:local:lerf_rank}
%     \scalebox{0.75}{
%      \begin{tabular}{ccccc}
%         \toprule
%         Sparsity &
%         Fidelity &
%         ROAR &
%         R-Fidelity & 
%         F-Fidelity \\
%         \midrule   
%         $5\%$& \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} \\
%         10\% & \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} \\
%         15\% & \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} \\
%         20\% & \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} \\
%         25\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} \\
%         30\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} \\
%         35\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} \\
%         40\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} \\
%         45\% &\ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} \\
%         50\% &\ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} \\
%         55\% &\ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} \\
%         60\% & \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} \\
%         65\% & \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} \\
%         70\% & \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} \\
%         75\% & \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} \\
%         80\% & \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} \\
%         85\% & \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} \\
%         90\% & \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} \\
%         95\% & \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} \\
%         \midrule   
%         Avg. Rank & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} \\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table*}


% \begin{table*}[h]
%     \centering
%     \caption{``MoRF VS LeRF'' Local Spearman rank correlation results on \tinyimagenet~dataset with ViT as the model to be explained.}
%     \label{tab:exp:tinyimagenet:vit:local:morf_lerf}
%     \scalebox{0.75}{
%      \begin{tabular}{ccccc}
%         \toprule
%         Sparsity &
%         Fidelity &
%         ROAR &
%         R-Fidelity & 
%         F-Fidelity \\
%         \midrule   
%         $5\%$ &  \ms{-0.83}{0.00} &  \ms{-0.81}{0.03} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} \\
%         10\% &  \ms{-0.83}{0.00} &  \ms{-0.79}{0.03} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} \\
%         15\% &  \ms{-0.82}{0.02} &  \ms{-0.63}{0.03} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} \\
%         20\% &  \ms{-0.76}{0.06} &  \ms{-0.61}{0.02} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} \\
%         25\% &  \ms{-0.74}{0.07} &  \ms{-0.65}{0.02} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} \\
%         30\% &  \ms{-0.83}{0.00} &  \ms{-0.67}{0.08} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} \\
%         35\% &  \ms{-0.81}{0.03} &  \ms{-0.71}{0.10} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} \\
%         40\% &  \ms{-0.84}{0.06} &  \ms{-0.83}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} \\
%         45\% &  \ms{-0.83}{0.00} &  \ms{-0.83}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} \\
%         50\% &  \ms{-0.83}{0.00} &  \ms{-0.83}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} \\
%         55\% &  \ms{-0.90}{0.06} &  \ms{-0.87}{0.06} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} \\
%         60\% &  \ms{-0.90}{0.06} &  \ms{-0.92}{0.05} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} \\
%         65\% &  \ms{-0.80}{0.03} &  \ms{-0.78}{0.09} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} \\
%         70\% &  \ms{-0.94}{0.04} &  \ms{-0.70}{0.06} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} \\
%         75\% &  \ms{-0.79}{0.11} &  \ms{-0.75}{0.09} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} \\
%         80\% &  \ms{-0.72}{0.15} &  \ms{-0.95}{0.25} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} \\
%         85\% &  \ms{-0.65}{0.24} &  \ms{-0.66}{0.21} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} \\
%         90\% &  \ms{-0.48}{0.24} &  \ms{-0.71}{0.17} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} \\
%         95\% &  \ms{0.32}{0.21}  &  \ms{-0.70}{0.09} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} \\
%         \midrule   
%         Avg. Rank & 5.42 & 6.05 & \textbf{1.00} & \textbf{1.00} \\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table*}

% \begin{table*}[h]
%     \centering
%         \caption{``MoRF VS GT'' Local Spearman rank correlation results on \tinyimagenet~dataset with ViT as the model to be explained.}
%     \label{tab:exp:tinyimagenet:vit:local:morf_rank}
%     \scalebox{0.75}{
%      \begin{tabular}{ccccccccc}
%         \toprule
%         &
%         \multicolumn{2}{c}{Fidelity} &
%         \multicolumn{1}{c}{ROAR} &
%         \multicolumn{2}{c}{R-Fidelity} & 
%         \multicolumn{2}{c}{F-Fidelity} \\
%         \cmidrule(r){2-3} \cmidrule(r){4-4} \cmidrule(r){5-6} \cmidrule(r){7-8} 
%         Sparsity &  origin  & fine-tune  & retrain  & origin  & fine-tune  & origin  & fine-tune \\
%         % Model & Correlation & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
%          \midrule   
%         % & \multicolumn{4}{c}{Local Spearman Correlation $\downarrow$} \\ 
%         % \hline
%         % \multirow{3}{\rotatebox[origin=c]{90}{ViT}}  \ms{\textbf{1.00}}{0.00}
%         $5\%$ & \ms{-0.83}{0.00} &  \ms{-0.89}{0.06} &  \ms{-0.81}{0.03} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         10\% &  \ms{-0.83}{0.00} &  \ms{-0.73}{0.08} &  \ms{-0.79}{0.03} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         15\% &  \ms{-0.82}{0.02} &  \ms{-0.70}{0.08} &  \ms{-0.63}{0.03} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         20\% &  \ms{-0.76}{0.06} &  \ms{-0.62}{0.03} &  \ms{-0.61}{0.02} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         25\% &  \ms{-0.74}{0.07} &  \ms{-0.65}{0.07} &  \ms{-0.65}{0.02} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
        
%         30\% &  \ms{-0.83}{0.00} &  \ms{-0.75}{0.08} &  \ms{-0.67}{0.08} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         35\% &  \ms{-0.81}{0.03} &  \ms{-0.67}{0.06} &  \ms{-0.71}{0.10} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         40\% &  \ms{-0.84}{0.06} &  \ms{-0.73}{0.08} &  \ms{-0.83}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         45\% &  \ms{-0.83}{0.00} &  \ms{-0.72}{0.02} &  \ms{-0.83}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         50\% &  \ms{-0.83}{0.00} &  \ms{-0.79}{0.03} &  \ms{-0.83}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         55\% &  \ms{-0.90}{0.06} &  \ms{-0.82}{0.02} &  \ms{-0.87}{0.06} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
        
%         60\% &  \ms{-0.90}{0.06} &  \ms{-0.81}{0.03} &  \ms{-0.92}{0.05} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         65\% &  \ms{-0.80}{0.03} &  \ms{-0.85}{0.06} &  \ms{-0.78}{0.09} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         70\% & \ms{-0.94}{0.04} &  \ms{-0.76}{0.08} &  \ms{-0.70}{0.06} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         75\% & \ms{-0.79}{0.11} &  \ms{-0.39}{0.10} &  \ms{-0.75}{0.09} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         80\% & \ms{-0.72}{0.15} &  \ms{-0.06}{0.13} &  \ms{-0.95}{0.25} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         85\% & \ms{-0.65}{0.24} &  \ms{0.37}{0.19}  &  \ms{-0.66}{0.21} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{-0.97}{0.03}\\
        
%         90\% &  \ms{-0.48}{0.24} &  \ms{0.75}{0.11} &  \ms{-0.71}{0.17} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{-0.90}{0.06}\\
%         95\% & \ms{0.32}{0.21} &  \ms{0.67}{0.18}   &  \ms{-0.70}{0.09} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{-0.99}{0.02} &  \ms{-0.71}{0.14}\\ 
%         \midrule   
%         Avg. Rank & 5.37 & 6.53 & 5.95 & \textbf{1.00} & \textbf{1.00} & 1.11 & 1.47\\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table*}


% \begin{table*}[h]
%     \centering
%         \caption{``LeRF VS GT'' Local Spearman rank correlation results on \tinyimagenet~dataset with ViT as the model to be explained.}
%     \label{tab:exp:tinyimagenet:vit:local:lerf_rank}
%     \scalebox{0.75}{
%      \begin{tabular}{ccccccccc}
%         \toprule
%         &
%         \multicolumn{2}{c}{Fidelity} &
%         \multicolumn{1}{c}{ROAR} &
%         \multicolumn{2}{c}{R-Fidelity} & 
%         \multicolumn{2}{c}{F-Fidelity} \\
%         \cmidrule(r){2-3} \cmidrule(r){4-4} \cmidrule(r){5-6} \cmidrule(r){7-8} 
%         Sparsity &  origin  & fine-tune  & retrain  & origin  & fine-tune  & origin  & fine-tune \\
%         % Model & Correlation & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
%          \midrule   
%         % & \multicolumn{4}{c}{Local Spearman Correlation $\downarrow$} \\ 
%         % \hline
%         % \multirow{3}{\rotatebox[origin=c]{90}{ViT}}  \ms{\textbf{1.00}}{0.00}
%         $5\%$& \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         10\% & \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         15\% & \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         20\% & \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         25\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
        
%         30\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         35\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         40\% &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         45\% &\ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         50\% &\ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         55\% &\ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
        
%         60\% & \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         65\% & \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         70\% & \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         75\% & \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         80\% & \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         85\% & \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
        
%         90\% & \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         95\% & \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00} &  \ms{\textbf{1.00}}{0.00}\\
%         \midrule   
%         Avg. Rank & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00}\\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table*}



% \begin{table*}[h]
%     \centering
%         \caption{``MoRF VS LeRF'' Local Spearman rank correlation results on \tinyimagenet~dataset  with ViT as the model to be explained.}
%     \label{tab:exp:tinyimagenet:vit:local:morf_lerf}
%     \scalebox{0.75}{
%      \begin{tabular}{ccccccccc}
%         \toprule
%         &
%         \multicolumn{2}{c}{Fidelity} &
%         \multicolumn{1}{c}{ROAR} &
%         \multicolumn{2}{c}{R-Fidelity} & 
%         \multicolumn{2}{c}{F-Fidelity} \\
%         \cmidrule(r){2-3} \cmidrule(r){4-4} \cmidrule(r){5-6} \cmidrule(r){7-8} 
%         Sparsity &  origin  & fine-tune  & retrain  & origin  & fine-tune  & origin  & fine-tune \\
%         % Model & Correlation & Fidelity  & ROAD & R-Fidelity  &  {F-Fidelity} \\
%          \midrule   
%         % & \multicolumn{4}{c}{Local Spearman Correlation $\downarrow$} \\ 
%         % \hline
%         % \multirow{3}{\rotatebox[origin=c]{90}{ViT}}  \ms{\textbf{1.00}}{0.00}
%        $5\%$ &  \ms{-0.83}{0.00} &  \ms{-0.89}{0.06} &  \ms{-0.81}{0.03} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         10\% &  \ms{-0.83}{0.00} &  \ms{-0.73}{0.08} &  \ms{-0.79}{0.03} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         15\% &  \ms{-0.82}{0.02} &  \ms{-0.70}{0.08} &  \ms{-0.63}{0.03} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         20\% &  \ms{-0.76}{0.06} &  \ms{-0.62}{0.03} &  \ms{-0.61}{0.02} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         25\% &  \ms{-0.74}{0.07} &  \ms{-0.65}{0.07} &  \ms{-0.65}{0.02} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
        
%         30\% &  \ms{-0.83}{0.00} &  \ms{-0.75}{0.08} &  \ms{-0.67}{0.08} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         35\% &  \ms{-0.81}{0.03} &  \ms{-0.67}{0.06} &  \ms{-0.71}{0.10} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         40\% &  \ms{-0.84}{0.06} &  \ms{-0.73}{0.08} &  \ms{-0.83}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         45\% &  \ms{-0.83}{0.00} &  \ms{-0.72}{0.02} &  \ms{-0.83}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         50\% &  \ms{-0.83}{0.00} &  \ms{-0.79}{0.03} &  \ms{-0.83}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         55\% &  \ms{-0.90}{0.06} &  \ms{-0.82}{0.02} &  \ms{-0.87}{0.06} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
        
%         60\% &  \ms{-0.90}{0.06} &  \ms{-0.81}{0.03} &  \ms{-0.92}{0.05} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         65\% &  \ms{-0.80}{0.03} &  \ms{-0.85}{0.06} &  \ms{-0.78}{0.09} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         70\% &  \ms{-0.94}{0.04} &  \ms{-0.76}{0.08} &  \ms{-0.70}{0.06} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         75\% &  \ms{-0.79}{0.11} &  \ms{-0.39}{0.10} &  \ms{-0.75}{0.09} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         80\% &  \ms{-0.72}{0.15} &  \ms{-0.06}{0.13} &  \ms{-0.95}{0.25} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00}\\
%         85\% &  \ms{-0.65}{0.24} &  \ms{0.37}{0.19} &  \ms{-0.66}{0.21} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{-0.97}{0.03}\\
        
%         90\% &  \ms{-0.48}{0.24} &  \ms{0.75}{0.11} &  \ms{-0.71}{0.17} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00} &  \ms{\textbf{-1.00}}{0.00} &  \ms{-0.90}{0.06}\\
%         95\% &  \ms{0.32}{0.21}  &  \ms{0.67}{0.18} &  \ms{-0.70}{0.09} &  \ms{\textbf{-1.00}}{0.00}  &  \ms{\textbf{-1.00}}{0.00} &  \ms{-0.99}{0.02} &  \ms{-0.71}{0.14}\\
%         \midrule   
%         Avg. Rank & 5.42 & 6.42 & 6.05 & \textbf{1.00} & \textbf{1.00} & 1.11 & 1.47\\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table*}



==> note.tex <==
When using stochastic and uniformly applied data augmentation, such as random pixel removal, the underlying assumption is that the augmentation introduces variations that mimic the natural distribution of input data, thereby improving generalization without distorting the model's understanding of the data distribution. Theoretical insights supporting this claim stem from several aspects of data augmentation and its effects on model learning.

1. Stochastic Augmentation Regularizes Learning
Theoretical Insight: Stochastic data augmentation acts as an implicit regularizer in machine learning, analogous to techniques like dropout or weight decay. By presenting the model with diverse views of the input data, augmentation discourages overfitting to specific features or patterns in the training set.
Mathematical Argument: Let 
��
(
��
;
��
)
L(θ;x) be the loss function of the model parameterized by 
��
θ. When applying augmentation 
��
(
��
)
A(x), the effective loss becomes an expectation over augmented inputs:
��
��
��
��
(
��
;
��
)
=
��
��
[
��
(
��
;
��
(
��
)
)
]
.
L 
aug
​
 (θ;x)=E 
A
​
 [L(θ;A(x))].
The averaging effect over the augmentation distribution reduces sensitivity to specific input patterns and promotes smoother decision boundaries.
2. Uniform Distribution Preserves Input Characteristics
Theoretical Insight: If the augmentation is uniformly applied (e.g., random pixel removal), all pixels have an equal probability of being removed, ensuring that no specific region of the input is disproportionately emphasized or ignored. This uniformity minimizes the introduction of biases toward specific patterns in the input data.
Practical Implication: Uniform random pixel removal maintains the core structure of the image, ensuring that the perturbed images remain representative of the original data distribution.
3. Invariant Representation Learning
Theoretical Insight: Data augmentation encourages the model to learn invariant representations. For instance, random pixel removal forces the model to focus on global and structural patterns in the data rather than over-relying on specific pixel-level features.
Support from Invariance Theory: Techniques like Mixup, Cutout, and random erasing, which are conceptually similar to random pixel removal, have been shown to improve robustness and generalization by promoting invariance to specific perturbations.
4. Generalization Bounds and Stability
Theoretical Insight: Stochastic augmentation can improve the generalization bounds of a model by effectively increasing the size of the training data space. This results in a smaller empirical Rademacher complexity or VC-dimension, metrics often used to measure the model’s capacity and potential to generalize.
Key Papers:
Zhang et al. (2017): Demonstrate that augmentation improves model generalization by acting as a form of dataset expansion.
Chen et al. (2020): Analyze how data augmentation leads to flatter loss landscapes, which are empirically correlated with better generalization performance.
5. Robustness to Perturbations
Theoretical Insight: Random pixel removal introduces a controlled level of noise into the data. Learning to classify correctly in the presence of such noise encourages the model to form decision boundaries that are robust to small input perturbations.
Connection to Adversarial Training: While adversarial training actively seeks to generate challenging perturbations, random augmentation passively introduces perturbations. Both approaches enhance robustness by ensuring the decision boundary is less sensitive to small variations in input.
6. Relationship to Manifold Learning
Theoretical Insight: Data augmentation can be viewed as a form of manifold learning. By perturbing inputs in ways that retain semantic meaning, the augmented data samples populate the data manifold more densely. This allows the model to better approximate the underlying structure of the data distribution.
Support from Augmentation Literature: Random pixel removal implicitly assumes that the perturbed inputs remain on or near the true data manifold. Studies have shown that models trained with augmented data tend to interpolate better between data points, leading to smoother and more reliable decision boundaries.
